Wi-Fringe: Leveraging Text Semantics in WiFi CSI-Based Device-Free Named Gesture Recognition

The lack of adequate training data is one of the major hurdles in WiFi-based activity recognition systems. In this paper, we propose Wi-Fringe, which is a WiFi CSI-based device-free human gesture recognition system that recognizes named gestures, i.e., activities and gestures that have a semantically meaningful name in English language, as opposed to arbitrary free-form gestures. Given a list of activities (only their names in English text), along with zero or more training examples (WiFi CSI values) per activity, Wi-Fringe is able to detect all activities at runtime. In other words, a subset of activities that Wi-Fringe detects do not require any training examples at all.

==> 01_introduction.tex <==
%\newpage
\section{Introduction}
\label{sec:intro}

\parlabel{Batteryless Systems. } The Internet of Things (IoT) promises to make our lives efficient, productive, enjoyable, and healthier by making everyday objects capable of sensing, computation, and communication. Many of these so-called IoT devices are powered by limited-capacity batteries---which makes them mobile, small, and lightweight. Batteries, however, require periodic maintenance (e.g.,  replacement and recharging) which is an inconvenience at a large scale. To address this practical problem, batteryless IoT devices have been proposed, which harvest energy from ambient sources, e.g., solar, thermal, kinetic, and RF to power up. These devices, in principle, last forever---as long as the energy harvesting conditions are met. They typically consist of low-power sensors, microcontrollers, and energy-harvesting and management circuitry, and their applications are in many deploy-and-forget scenarios, e.g., wildlife monitoring, remote surveillance, environment and infrastructure monitoring, wearables, and implantables.

\parlabel{Time-Aware Inference. } Many IoT applications require timely feedbacks. For instance, in an acoustic monitoring system, audio events need to be detected and reported as fast as possible to initiate prompt actions. Similarly, an air-quality monitoring system needs to identify the increase of a certain air component on time for taking proper actions. Likewise, shared resources, such as gym-equipment and shared bikes in a campus, can be monitored in real-time to detect misuses or malfunctions, and to inform the authority about the incidence on time. While a batteryless system is desirable in these real-time sensing and event detection applications, the unpredictability of the harvested energy, combined with the complexity of on-device event detection tasks, complicates timely execution of machine learning-based event detection tasks on batteryless systems. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.35\textwidth]{fig/intermittencd_deadlinemiss.pdf}
            \vspace{-1em}
    \caption{(a) With constant power both deadlines are met. (b) With intermittent power, task $\tau_2$ misses deadline. (c) When, execution of the whole task is not necessary, both tasks can be scheduled successfully.}
        \label{fig:intermittent_deadmiss}
        \vspace{-1em}
\end{figure}

\parlabel{Prior Work on Timeliness. } Prior works on time-aware batteryless computing systems can be broadly categorized into two types. The first category focuses on \emph{time-keeping}, i.e., maintaining a reliable system clock~\cite{rahmati2012tardis, hester2016persistent} even when the power is out. The sporadic nature of an energy harvesting system forces it to run intermittently by going through alternating episodes of power ON and OFF phases which disrupts the continuity of the system clock. By exploiting the rate of decay of an internal capacitor and the content of the SRAM, these systems enable time-keeping during the absence of power. The second category proposes runtime systems that consider the temporal aspect of data across power failures~\cite{hester2017timely, buettner2011dewdrop, zhu2012deos, yildirim2018ink}. For instance, ~\cite{hester2017timely} discards data after a predefined interval and thus saves energy by not processing stale data, and ~\cite{yildirim2018ink, buettner2011dewdrop,zhu2012deos} propose energy-aware runtime systems to increase the chances of task completion. However, none of these consider the utility of data or exploit the property of inference tasks to plan real-time deadline-aware execution of tasks.  

\parlabel{Real-Time Intermittent Computing. } Scheduling time-aware machine learning tasks on a batteryless computing system is an extremely challenging feat. The two main sources of challenges are the \emph{intermittent power supply} and the \emph{computational demand for executing machine learning tasks}. These two challenges have been studied extensively in non-real-time settings. For instance, ~\cite{ransford2012mementos, mirhoseini2013automated,balsamo2015hibernus, balsamo2016hibernus++,maeng2017alpaca, colin2016chain, maeng2018adaptive} enable seamless execution of non-real-time tasks on intermittently powered systems by proposing techniques that save and restore the program states across power failures. ~\cite{gobieskiintermittent, gobieski2019intelligence, nirjon2018lifelong, bashima2019ondevice} propose lightweight and compressed deep neural network inference for on-device machine learning on batteryless systems. However, none of these works consider the timing constraints of the machine learning tasks. In a real-time setting, simply applying these two types of solutions in conjunction with an existing real-time scheduling algorithm does not quite solve the problem at hand, which is illustrated in Figure~\ref{fig:intermittent_deadmiss}. We consider two tasks, $\tau_1$ and $\tau_2$, released at time 0 and 25, respectively. Their deadlines are 45 and 56, and both have an execution time of 28. In Figure~\ref{fig:intermittent_deadmiss}(a), we observe that under the earliest deadline first (EDF) scheduling, both tasks meet the deadlines when the power is uninterrupted. But when power is intermittent, Figure~\ref{fig:intermittent_deadmiss}(b) shows that task $\tau_2$ misses its deadline.

\parlabel{Observations. } The goal of this paper is to overcome the aforementioned challenges. Towards this end, we study the energy harvesting pattern and the accuracy-execution trade-off of compressed deep neural networks (DNNs) that are executable on small systems~\cite{gobieski2019intelligence}. From these studies, we make two observations: 

$\bullet$ First, energy generated by a harvester is \emph{bursty}, and therefore, its energy harvesting pattern can be modeled using a stochastic framework over a short duration. Here, burstiness indicates that energy generation is maintained during a short period. 

$\bullet$ Second, since deeper layers of a DNN extract fine-grained and more detailed features of the input, for a given accuracy, the amount of DNN computation required for an input data is dependent on the quality of data itself. 

\parlabel{The \Sys~Approach. } By exploiting these above two observations, we design an \emph{imprecise computing}~\cite{shih1992line, liu1991algorithms}, online scheduling algorithm that considers both the intermittent nature of the power supply and the accuracy-execution trade-off of the DNN model. This design allows us to increase both accuracy and timeliness of DNN execution in intermittent systems. For example, in Figure~\ref{fig:intermittent_deadmiss}(c), when a full execution of the task is not necessary, i.e., tasks are \emph{imprecise}, both tasks can meet the deadline.

%Deep neural network (DNN) refers to neural networks with more than three layers including input and output layers. The DNNs considered in this paper, are small and compressed networks with at most 64,000 fixed-point parameters.}     

Our work complements previous work on time-keeping~\cite{rahmati2012tardis, hester2016persistent} and intermittent execution of non-real-time tasks~\cite{gobieskiintermittent, gobieski2019intelligence, ransford2012mementos, mirhoseini2013automated,balsamo2015hibernus, balsamo2016hibernus++,maeng2017alpaca, colin2016chain, maeng2018adaptive}. We extend the state-of-the-art intermittent DNN execution framework, called SONIC ~\cite{gobieski2019intelligence}, by implementing a runtime framework that supports intelligent scheduling of real-time DNN tasks. To enable time-aware adaptive deep learning in intermittently powered systems, we make three key technical contributions:   

%, and considers that time-keeping can be achieved with~\cite{rahmati2012tardis, hester2016persistent}. Both time-keeping and intermittent execution in batteryless system is out of the scope of this paper. Like ~\cite{yildirim2018ink,hester2017timely} this paper keeps time with a real-time clock for the ease of implementation as described in Section~\ref{sec:setup}.

%\bnote{Unlike battery-powered systems where usability is tied to battery-life, a batteryless system, which lasts forever, loses its worth when the code dies. Death of the code refers to outdated parameters which is unable to model the current environment. Therefore, evolving with the environment in such a system is necessary. The computational and memory constraints of batteryless systems and the unavailability of labeled data obstruct complicated adaptation techniques (e.g., back propagation). To address this challenge, we consider a semi-supervised learning (semi-supervised K-means) that updates previously trained model with the incoming data stream. }


$\bullet$ First, we devise a metric, i.e., the $\eta$-factor, to model the predictability of an energy harvester's source. This metric indicates the probability of a harvester maintaining its current state over a short period in time. The introduction of $\eta$-factor abstracts away the unpredictability of an energy harvesting source and enables development of scheduling algorithms that can make informed decisions based on predicted energy over a short period in the future. 

$\bullet$ Second, we redesign the DNN construction and training algorithms to enable early termination of a DNN task based on the quality of the input data. To enable this, we propose a \emph{layer-aware loss function} to improve the accuracy of a clustering-based, semi-supervised inference algorithm that uses DNN layer outputs as the representation of the input examples.

$\bullet$ Third, we propose an imprecise computing-based, online, scheduling algorithm that improves the timeliness of DNN inference tasks running on energy harvesting systems. This algorithm leverages the $\eta$-factor of the energy source, along with the properties of the input data to adapt the execution of real-time DNN tasks. 

\parlabel{Main Results. } We implement the system on a TI MSP430FR5994 and evaluate its performance using two datasets: MNIST~\cite{lecun1998mnist} and ESC-10~\cite{piczak2015environmental}, as well as in real-world acoustic event detection experiments. We achieve 9.45\% - 3.19\% higher accuracy than the baseline DNN algorithms for MCUs and achieve 14\% reduction in execution time. The proposed scheduling algorithm successfully schedules 33\%-12\% more tasks than traditional scheduling algorithms. 

%non-real-time systems. 


% \rnote{mention impmentaion and application and results to complete the intro.,}

%as well as the utility-execution trade-off where the utility can be application dependent. 

%$\bullet$ We introduce a combination of pre-trained DNN model and semi-supervised learning algorithm. We also utilize the dependency of required network depth on data and propose early termination of a deep neural network. We also propose a light-weight utility for this system and tie our scheduling algorithm with DNN models.

%$\bullet$ To maximize the early termination accuracy, we propose a layer-aware loss function which considers loss across each layer of the network. We also propose an approximate adaptation of the deeper layers of networks for the data which terminates the network early. To our knowledge, we are the first to consider layer-aware loss function. 


==> 02_motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\parlabel{On-Device Learning.} Resource-constrained sensing and inference systems enjoy the benefit of machine learning in two ways -- either they send raw or partially processed sensor readings to a remote server for inference, or they do everything on device. While most low-power IoT systems largely use the former method~\cite{de2018paws, shao2018marble, choudhurysuper, chandrasekaran2016seus, xia2019improving}, in recent years, we see an increasing trend in on-device machine learning on embedded systems ~\cite{google_federated_learning, OVIC, ravi2017projectionnet, google_projectionnet}. This can partly be attributed to the limitations of server-based systems -- which are generally energy-demanding, slow, less reliable, and privacy invasive. The other reason behind this increasing trend is the advancement in hardware and software technologies~\cite{qualcommOnDevice, qualcommOnDeviceSlide,EdgeTPU,appleAI, QualcommNPS,google_federated_learning,appleAI} that are enabling powerful machine learning features into small and low-power systems.     


%Artificial Intelligence is the ability to automate intellectual tasks usually performed by humans~\cite{chollet2017deep}. Similar to a human, a system learns from experience to exhibit intellect where experience comes as large datasets. Most machine learning operations execute in the cloud/server and have several drawbacks, e.g., latency, privacy, and reliability~\cite{nirjon2018lifelong, bashima2019ondevice}.

%On-device learning addresses these short-comings with the need for more optimized operation. It achieves \emph{lower latency} than cloud-based solutions by saving the round-trip to the server. It increases \emph{reliability} as communication with a server is still tricky in several parts of the world due to the bad or no network signal. Besides, limited communication \emph{saves energy} by reducing the usage of power hungry network modules. Low-power networks (e.g., backscatter) has lower data-rate, which results in the prolonged transmission period. On-device learning saves scarce and limited \emph{network bandwidth} resource. Finally, on-device learning \emph{preserves privacy} and thus avoids security hazards. For example, last year sensitive information of 31 million Android users was leaked due to the hacking of a popular keyboard~\cite{keyboardBreach}. To enable on-device learning in current smartphones, special purpose hardware~\cite{qualcommOnDevice, qualcommOnDeviceSlide,EdgeTPU,appleAI} and software~\cite{QualcommNPS,google_federated_learning,appleAI} have been introduced.


%Today's low power computing devices commonly offload the majority of computations~\cite{de2018paws, shao2018marble, choudhurysuper, chandrasekaran2016seus, xia2019improving}. With the exponential growth of the internet of things (IoT)~\cite{iotgrowth}, this design is causing stress on the limited bandwidth. The power consumption for communication (23,000mJ) costs 360$\times$ higher than local inference (198mJ) on a MNIST~\cite{lecun1998mnist} input~\cite{gobieski2019intelligence}. Therefore sending the result rather than the raw data is more efficient~\cite{gobieski2019intelligence, islam2018glimpse}. 

\parlabel{Learning on Batteryless Systems.} Previous works have addressed the need for computation including inference of deep neural network on energy harvested devices ~\cite{gobieskiintermittent, gobieski2019intelligence, ransford2012mementos, colin2016chain, maeng2017alpaca}. However, the necessity of updating the models and timeliness is yet to be explored. As no two scenarios or people are genuinely similar, the need to have a customized model is inevitable. Besides, the models of a forever executing batteryless system become outdated with time. To address the same issue, on-device learning (including training) is introduced~\cite{google_federated_learning}, which improves accuracy and provides a personalized system that ensures privacy, lower latency, and reliability.
Moreover, most batteryless systems are deployed at unreachable places (e.g., deep jungles, calamity-prone areas) where the traditional power source is absent and replacing a battery is unrealistic. It is also not feasible to collect data and update the model on-site in such cases. With time, such devices observe a massive amount of information which is likely to be wasted due to the inefficiency of data transmission. To fully utilize the potential of batteryless devices, training the models is needed. However, the small footprint of batteryless devices works against the extra computational and energy load enforced by training models and the unavailability of labeled data obstruct complicated adaptation techniques (e.g., back propagation). Light-weight semi-supervised learning algorithms needs to be considered to evolve previously trained models with the incoming data stream. 

\parlabel{Deep Inference. }
Due to its non-linear and parametric model, Deep Neural Network (DNN) exhibits better performance than other traditional models, e.g., Support Vector Machine  (SVM). Here, DNN refers to neural networks with more than one hidden layer. Sending the inference result instead of the raw data is more energy efficient and high accuracy is essential to maintain the system's usability. ~\cite{gobieski2019intelligence} shows that inference accuracy determines the end-to-end system performance. 

\parlabel{Time-Aware Inference. }
The higher accuracy of DNN is achieved using more rigorous computations that result in higher execution and response time.  For a usable system, the response time needs to be tolerable~\cite{zhu2012deos, moser2006lazy, moser2007real}. High delay of a system hampers its usability despite accuracy. Though some works have addressed real-time requirements for batteryless sensor nodes, the accuracy of the system itself has not been considered yet. Precision and responsiveness both are crucial for the usability of a learning system and are contradictory to each other. The goal is to find the sweet spot where the highest accuracy can be achieved with acceptable delay. Such a time-aware application includes event detection and  monitoring wildlife, natural calamities, wearable, implantable, infrastructure, and buildings. To illustrate, an acoustic event detector at home enables home activating monitoring, intruder detection, and elderly monitoring. Similarly, gym-equipment and shared bike usage can be monitored using kinetic energy harvesting systems which can inform the authority about the required maintenance of the system. 

==> 03_pre_study.tex <==
\section{System Modeling}
\label{sec:model}
In this section, we study and model the energy harvesting pattern of energy harvesters and the accuracy-execution trade-off of deep neural networks. 

\subsection{Modeling Energy Harvesting Pattern}
\label{sec:energy_study}

\parlabel{Energy Events.} 
Transiently powered systems operate intermittently because energy is not always available to harvest and, even when energy is available, buffering sufficient energy to perform adequate work takes time. In most cases, the pattern of this intermittency is stochastic and thus modeling this patter is not straight forward. To schedule the workload of an intermittently operating system at run-time, we decide whether to start execution of a task or not at a time instant. This decision heavily depends on the availability of harvestable energy. To model the availability of energy, we define \emph{energy event} which expresses the availability of sufficient energy during a period. Energy event represents a successful generation of at least K Joules of energy in total during T time slot. Here, K and T are system dependent. In order to better understand the property of energy events, we observe the phenomenons causing energy events. For example, in a piezo-electric harvester, taking a minimal number of steps that generates at least K Joule of energy during T time slot is considered equivalent to the occurrence of an energy event. Similarly, we consider a minimal number of packet transmissions per time slot and minimum intensity of solar per time slot as energy events for RF and solar harvesters, respectively.

\parlabel{Properties of Energy Events.}
We study energy event patterns of three commonly used harvesters -- piezo-electric harvester, solar harvester, and RF harvester from datasets ~\cite{meyer2016daily, ipdataset}. These datasets contain the number of steps taken during every 5-minute time-slot for 61 days, harvested solar energy measurements for three days and outbound packet transmission rate by an RF transmitter for 30 days. This study reveals two interesting observation about the pattern of energy events -- (1) energy events occur in bursts where burstiness is the intermittent increases and decreases in activity or frequency of an event~\cite{akbarpour2018diffusion}, (2) a probabilistic relation exists among the consecutive energy events during a short period. In other words, the occurrence of an energy event increases the probability of the next energy event during a short period. To illustrate, when a person starts walking, the probability of continuing the walk is high within the first few time slots and it decreases with time. Likewise, when a person is sitting, the probability of remain seated is high immediately, but decreases after a while. 

\parlabel{Conditional Energy Event. }
We define \emph{conditional energy event (CEE)} that represents the conditional probability of an energy event occurrence based on the occurrence/absence of previous consecutive energy events. CEE(N) is the probability that an energy event will occur given immediately preceding N consecutive energy events occurred (for $N >0$) or not occurred (for $N < 0$). The following equation expresses CEE.
\begin{equation}
\resizebox{0.43 \textwidth}{!}{
    $CEE(N) = 
        \begin{cases}
        $p$($occurrence $|$ N consecutive occurrence$),& $if $ N > 0 \\
        $p$($occurrence $|$ N consecutive non-occurrence$) ,& $if $ N < 0
        \end{cases}$
}
\end{equation}
To illustrate CEE(10) = 90\%  implies that the next energy event will occur with 90\% probability if 10 immediately preceding consecutive energy event occurred. Similarly, CEE(-15) = 5\% indicates the probability of an energy event at the current time slot is 5\%, given that there were no energy events in the last 15 slots.)
\begin{figure}[!htb]
    \centering
    \vspace{-.2in}
    \subfloat[KW=0, \Factor=1]{\includegraphics[width=.24\textwidth]{plot/Ideal_CEE.pdf}}
    \subfloat[KW=0.17, \Factor=0.65]{\includegraphics[width=.24\textwidth]{plot/step_CEE_1.pdf}}
    
    \subfloat[KW=0.06, \Factor=0.84]{\includegraphics[width=.24\textwidth]{plot/solar_CEE_1.pdf}}
    \subfloat[KW=0.11, \Factor=0.76]{\includegraphics[width=.24\textwidth]{plot/RF_CEE_1.pdf}}
    \caption{(a)CEE for persistent power source. (b) CEE for piezo-electric harvester. (c) CEE for solar harvester. (d) CEE for RF harvester. We use N=20 for calculating KW and \Factor. 
    }
    \label{fig:assumption_proof}
\end{figure}

The CEE of a system powered by a persistently power supply or an ideal harvester that has no intermittence looks like Figure ~\ref{fig:assumption_proof}(a). Figure ~\ref{fig:assumption_proof}(b-d) shows the CEE of three energy harvested systems. From these figures, we observe that for a small value of N these systems demonstrate similarity with the ideal correlative harvester. We measure the similarity of CEE of a harvested system with persistent powered or ideal harvested system using Kantorovich-Wasserstein (KW) distance~\cite{ramdas2017wasserstein}. Through out this paper, we use KW to express the Kantorovich-Wasserstein distance between the CEE a system (H) and the CEE of persistently powered system (P) as given in Equation~\ref{eq:kw}.  We also observe that for a large $|$N$|$ the CEE drops significantly because when the interval time between the first and current event increases their probabilistic relation decreases. For example, a person is walking for a long time has a high probability of stopping.
\begin{equation}
    KW(H, P) = \int_{-\infty}^{+\infty} |CDF(H) - CDF(P)|
\label{eq:kw}
\end{equation}

\parlabel{\Factor~Factor. }
To quantify the predictability of a harvester, we take inspiration from ~\cite{srinivasan2008beta} and define a predictability metric \Factor. Despite being informative, distance alone is not sufficient to measure predictability. Because distance does not address the imbalance between the number of elements in CEE with positive and negative N values. To address this, we quantify \Factor~ as the distance of the harvester (H) from a persistently powered system compared to the distance of the random harvester from a persistently powered system with same energy event rate. Random harvester (R) refers to harvesters where energy events are completely independent. \Factor~ is expressed as follows. 
\begin{equation}
    \eta = \frac{KW(R, P) - KW(H, P)}{KW(R, P)}
\end{equation} 

\Factor~$=1$ indicates that the power is persistent, while \Factor~$=0$ indicates energy events are totally random. This metric is also depends on the number of consecutive energy events. As CEE(N) is close to zero for high $|$N$|$, we consider small $|$N$|$ throughout the paper.
Figure~\ref{fig:assumption_proof}(b-d) shows the KW and \Factor~ where $|$N$|$ is 20. 

\Factor~ not only varies across different harvesters but also changes for a specific harvester. For transiently powered devices this change over time depends on different parameters, e.g., change of human weight, change of seasons or locations, the distance between RF transmitter and receiver. However, due to the infrequency of these changes, they can be ignored.



\subsection{Modeling Deep Neural Network}
\label{sec:study_dnn}
In order to execute machine learning tasks (e.g., deep neural network (DNN) inference with convolution and fully connected layers) in a resource-constrained batteryless system, we need to minimize memory and computation costs. To achieve this goal, we study several attributes that are unique to deep learning processes. 

\parlabel{Significance of Depth.} DNN have layered structures where the input of the first layer is from an external source, e.g., sensors. The output of a layer is fed as the input of the next layer, and it goes on until the end of the network. The total number of layers in a DNN is called \emph{depth}. A shallow neural network, e.g. first perceptrons are composed of one input layer, at most one hidden layer and one output layer. A neural network having more than three layers (including input and output) qualifies as "deep" neural network. Increased number of layers and neurons both contribute to more complicated calculation resulting in higher accuracy~\cite{he2016deep}. However, a shallow network requires width exponential to that of a deeper network to achieve similar accuracy.  Therefore, the performance of a neural network depends on not only the number of parameters but also depth. For example, VGGNet has 16 layers with ~140M parameters, while ResNet beats it with 152 layers but only ~2M parameters. 
\begin{figure}[!htb]
    \centering
    \vspace{-0.19in}
    \includegraphics[width=0.45\textwidth]{fig/face5.pdf}
    \vspace{-0.19in}
    \caption{Example of deep learning learns layers of features.}
    \vspace{-0.16in}
    \label{fig:depth_example}
\end{figure}

The depth of a DNN is significant because at each layer nodes train on a distinct set of features based on the output of the previous layer. The complexity and abstraction of features increase with the depth of layers, and it is known as the feature hierarchy. Deep learning can extract features from data without human intervention. This automatic feature extraction is known as representation learning. 
To understand the effect of the depth of a DNN, let us consider a face detector in Figure~\ref{fig:depth_example}(a). The first layer of this deep learning based face detector learns basic features, e.g., edges. In the next layer, a collection of edges, e.g., nose, is learned.  A deeper layer learns a higher level feature, e.g., face abstraction.
\begin{figure}[!htb]
    \centering
    \vspace{-0.25in}
    \subfloat{\includegraphics[width=.4\textwidth]{plot/layer_class.pdf}}
    \vspace{-0.22in}
    \caption{Hard data requires complex representation to achieve similar accuracy.}
    \label{fig:exit_motivation1}
\end{figure}
\vspace{-0.22in}

\parlabel{Required Depth.} To decrease the execution time we observe the fact that depth is highly \emph{data-dependent}~\cite{bolukbasi2017adaptive}. If target classes are profoundly distinctive, then simple features can be used to distinguish them. For example, in Figure~\ref{fig:exit_motivation1}, audio of cat and water (easy data) are very distinguishable; thus a single layer CNN achieves 93\% classification accuracy. On the other hand, similar classes, e.g., train and helicopter (hard data) needs more complex representations to be distinct and thus require five layers of CNN to achieve 81\% accuracy. \emph{Representation learning} uses deep neural network to extract features from raw data. By executing only necessary layers based on the complexity of data we can achieve similar accuracy with decreased execution time. We consider execution of each data sample as a task and introduce the requirement of depth as a imprecise task model~\cite{shih1992line, liu1991algorithms, canon2018scheduling}. Each imprecise task consists of two portions -- mandatory and optional. Mandatory portion of a task is necessary to achieve required accuracy while executing optional portions further improves the performance. We consider the required depth for a data sample as mandatory portion and rest as optional.

\parlabel{DNNs for Ultra-Low-Power Systems.}
Fitting neural networks in resource-constrained energy harvesting systems is a challenge especially due to limited memory capacity. Most commonly used processors in existing intermittent systems are TI MSP430 low-power microcontrollers~\cite{colin2018reconfigurable, hester2016amulet, gobieski2019intelligence,hester2015tragedy,hester2017flicker} that include 1-4KB of SRAM and 32-256KB of FRAM. Therefore, only small compressed networks are suitable for these systems. Compressed networks mentioned in Table~\ref{tab:network} and previous work~\cite{gobieski2019intelligence} have 48,136-10,411 parameters. For 16-bit fixed point data type these parameter requires 96.3-20KB of memory. On the other hand, same networks require 943.66-180KB of memory without compression. Such networks can be executed in batteryless systems only after compression. However, larger networks  e.g., Resnet (image) and EnvNet (audio) requires 5MB and 94MB of memory which is not suitable for small memory footprint devices even after compression.

We execute MNIST(compressed) in TI MSP430 to estimate the size of code and other variables in the FRAM. We observed that instructions and other parameters (including a buffer to perform matrix operations) require around 128KB of memory. Though the increasing number of parameters increases the buffer size, for simplicity we ignore it. The remaining memory can be used for storing approximately 64,000 16 bit fixed point parameters. A deep neural network that requires less than 64,000 parameters can execute in a microcontroller having 256KB of FRAM. The number of hidden layers and the number of neurons at each layer depend on the number of input and output~\cite{heaton2011programming}. Therefore, very large dataset e.g., Imagenet is not suitable for such systems. These conditions are sufficient for executing 4-6 layer networks depending on the network configuration~\cite{gobieski2019intelligence}.


% HAR = 14,754 -- 524,616 
% OkG = 48,136 -- 330,896
% MNIST = 13,645 -- 475,500
% ESC-10 = 10,411 -- 65,936


%  An MSP430 with 256 KB of memory, for 28$\times$28 input and 10 outputs can support either -- (1) 4 fully connected(FC) hidden layers having an average of 64 neurons at each layer,  or (2) 2 convolution hidden layers where average filter size is 5$\times$5, and number of filters are 24 on average followed by 2 fully connected hidden layers having an average 64 neurons at each layer. }

This paper considers two networks summarized in Table~\ref{tab:network}. MNIST~\cite{lecun1998mnist} represents the image-based application, and ESC-10~\cite{piczak2015dataset} represents audio applications. We use two known techniques -- rank decomposition or separation~\cite{bhattacharya2016sparsification, chollet2017xception, xue2013restructuring, de2000multilinear, de2000best, tucker1966some} and pruning~\cite{han2015deep, nabhan1994toward} to compress each layer of the networks. Note that, our semi-supervised models avoid the last layers for inference.

% \rnote{Add a table comparing the traditional DNN's size and accuracy with compressed DNN's size and accuracy.}

\begin{table}[!thb]
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}cccc@{}}
\toprule
Dataset                & Layer & \begin{tabular}[c]{@{}c@{}}Uncompressed\\ Size\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Compressed\\ Size\end{tabular} \\ \midrule
\multirow{4}{*}{MNIST} & Convolution  & 20$\times$1$\times$5$\times$5                                                                                                               & 3$\times$1D Convolution                                                 \\ 
                       & Convolution  & 100$\times$20$\times$5$\times$5                                                                                                     & 1253                                                      \\ 
                       & Fully Connected    & 200$\times$1600                                                                                                     & 5456                                                      \\ 
                       & Fully Connected    & 500$\times$200                                                                                                       & 1892                                                      \\
                       & Fully Connected    & 10$\times$500                                                                                                     & --                                                      \\
                       \midrule
\multirow{4}{*}{ESC-10} & Convolution  & 16$\times$1$\times$5$\times$5                                                                                                            & 3$\times$1D Conv                                                 \\ 
                       & Convolution  & 32$\times$16$\times$5$\times$5                                                                                                     & 1280                                                      \\ 
                       & Convolution    & 64$\times$32$\times$5$\times$5                                                                                                 & 5068                                                      \\ 
                       & Fully Connected    & 96$\times$256                                                                                                      & 2703                                                      \\
                       & Fully Connected    & 10$\times$96                                                                                                  & --                                                      \\ \bottomrule
\end{tabular}
}
\caption{Networks considered in this paper.}
\vspace{-.3in}
\label{tab:network}
\end{table}

==> 04_overview.tex <==
\section{\Sys~System Design}
\label{sec:overview}

\Sys~is a system architecture that executes semi-supervised deep learning with timing constraints in an intermittently powered system. It uses a deep neural network to extract complex features from data samples, where the deep neural network is pre-trained on a high-end device. \Sys~adapts to new unlabeled incoming data by using semi-supervised models, e.g., seed-based k-means~\cite{basu2002semi}. In seed-based k-means, initial centroids are defined from labeled data in training phase and at runtime the unlabel data update these centroids. \Sys~ relies on imprecise computing to maximize the number of samples meeting timing constraints in a batteryless platform. 

\Sys~aims to achieve three goals simultaneously -- (1) minimize classification error, (2) maximize the number of samples meeting time constraints, and (3) minimize energy waste. \Sys~addresses this by terminating the deep feature extraction network early when necessary and scheduling the samples with a special online scheduling algorithm for batteryless system that considers time, classification error and availability of energy simultaneously. 
\begin{figure}[!thb]
    \centering
    \vspace{-.5em}
    \includegraphics[width=.48\textwidth]{fig/flow_chart.pdf}
    \caption{\Sys~system architecture.}
    \vspace{-.2in}
    \label{fig:sys}
\end{figure}

\subsection{System Components}
\Sys~consists of five major components -- task generator, energy manager, agile DNN model, scheduler and adaptive models. 

$\bullet$ \textit{Task Generator. } 
\Sys~ gathers data from sensors (e.g. microphone, camera) and considers each data sample as a task. A task includes inference of agile DNN model and semi-supervised learning using adaptive model with adaptation for a data sample. To sense, it takes advantage of the analog to digital converter (ADC) and direct memory access (DMA) which writes sensor data to non-volatile memory without occupying the CPU. Each task (data sample) is pushed in the \emph{task queue} upon arrival. Each task contains two portions -- mandatory and optional. Only tasks in the task-queue are considered for execution and a task leaves the queue at the end of execution or at deadline.

$\bullet$ \textit{Energy Manager. }
The energy manager monitors the status of the energy storage (e.g. capacitor) and the energy harvesting rate. To measure the energy harvesting rate it relies on the system operating voltage and the voltage across the capacitor. These parameters are fed to the scheduler that determines whether to execute a task depending on these parameters. When energy is less than a minimum threshold ($E_{man}$), power failure occurs and nothing gets executed. We use SONIC~\cite{gobieski2019intelligence} to handle intermittent execution of tasks in this system.

$\bullet$ \textit{Agile DNN Model. }
Agile DNN model is a pre-trained feature extraction deep neural network. This deep neural network is trained with labeled data to extract the features from data for semi-supervised learning. This network is trained in a high-end device (e.g. server or GPU). We compress the trained network using rank decomposition and separation to fit in memory-constrained systems. To achieve better classification/ clustering accuracy in the earlier layer of the network, we propose a layer-aware loss function. The goal of this loss function is to extract distinctive features in the early stages of the network if possible. 

$\bullet$ \textit{Adaptive Models. } 
Adaptive models are a set of seed-based k-means models. These models classify the sensor data by using the features extracted from the Agile DNN models. To select only useful features and to decrease the model size, these models use features with highest Chi-squared stats. Adaptive models are incrementally updated to evolve with new data and adapt to dynamic environment. These models are utilized to determine confidence of accuracy (utility) to exit the DNN layers.

$\bullet$ \textit{Scheduler. }
The scheduler decides which task to process and partitions the task based on utility. This utility decides if the data sample requires further processing for more confident decision making. The scheduler uses this mandatory and optional segments, achieved confidence (utility) and energy status from the energy manager to decide which data sample to process. 
When a function of current energy of the system ($E_{curr}$) and \Factor~ is less than a threshold ($E_{opt}$), \Sys~ becomes conservative in its choice for execution and considers only mandatory portions of tasks. The high probability for low energy harvesting and possible power failure in the near future leads to this decision. Otherwise \Sys~ considers both mandatory and optional portions for execution. 



\begin{table}[!htb]
\begin{tabular}{@{}cccccc@{}}
\toprule
Task & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total\\ Layers\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mandatory\\ Layers\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Optional\\ Layers\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Release\\ Time\end{tabular} & Deadline \\ \midrule
$\tau_1$   & 4            & 1                & 3               & $t_1$           & $t_7$      \\
$\tau_2$    & 4            & 2                & 2               & $t_3$           & $t_9$      \\ \bottomrule

\end{tabular}
\caption{Task Description}
\label{tab:load_des}
\end{table}
\vspace{-.5in}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/example.pdf}
    \vspace{-.15in}
    \caption{Example of execution of \Sys.} 
    \vspace{-.25in}
    \label{fig:example}
\end{figure}
% \vspace{-.25in}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[!htb]
\begin{tabular}{cp{7cm}}
\toprule
Time                 & \multicolumn{1}{c}{Reason of the Action}                            \\ \midrule
$t_0$                  & No task in the system.                                              \\
$t_1$                  & $\tau_1^1$ (the only task) gets scheduled.                          \\
$t_2$                  & Since $E_{curr}$ < $E_{opt}$, optional $\tau_1^2$ is not scheduled.  \\
$t_3$                  & System prioritized $\tau_2^1$ over $\tau_1^2$ (See: Section 5).     \\
$t_4$                  & Since $E_{curr}$ < $E_{man}$ no task is scheduled.                  \\
$t_5$                  & System prioritized mandatory $\tau_2^2$ over optional $\tau_1^2$ .  \\
$t_6$                  & Only optional tasks remain and $E_{curr}$ >$E_{opt}$. The system prioritizes $\tau_1^2$ over $\tau_2^3$ due to its tighter deadline. \\
$t_7$                  & $\tau_2^3$ (the only task) gets scheduled.                          \\
$t_8$                  & $\tau_2^4$ (the only task) gets scheduled.                          \\ \bottomrule
\end{tabular}
\caption{Description of Figure~\ref{fig:example}}
\vspace{-.35in}
\label{tab:example_des}
\end{table}

\subsection{Example Execution}

We describe a simple workload consisting of real-time inference of two examples and demonstrate how \Sys~ executes the workload.
We describe the tasks in Table~\ref{tab:load_des}, where $\tau_i$ refers to task i. Figure~\ref{fig:example} demonstrates execution of task $\tau_1$ and $\tau_2$ along with energy status. Here, $\tau_i^j$ refers to $j^{th}$ layer of task i. Table~\ref{tab:example_des} provides the actions and reasons of the actions taken at each time step. Note that this example uses simplified assumptions (e.g. each layer requires single time unit to execute). The algorithm mentioned in Section 5 handles complexities (e.g., different execution time for each layer, multiple time units per layer, unknown mandatory layer number and, power-failure during layer execution).


==> 05A_scheduler.tex <==
\section{Real-Time Scheduler}
\label{sec:algo_rt}

This section describes a generic real-time task scheduler for intermittently powered systems where each task executes as a chain of sequential subtasks that can be partitioned into mandatory and optional parts. We define the task model and task prioritization metric, and describe the scheduling algorithm.
\begin{figure}[!htb]
    \centering
    \vspace{-.12in}
    \includegraphics{fig/task_model.pdf}
    \vspace{-.7in}
    \caption{Task model for task $\tau_i$}
    \vspace{-.2in}
    \label{fig:task_model}
\end{figure}
\subsection{Task Model}

\parlabel{Define Task.}
We define each data sample entering \Sys~ as an imprecise task\footnote{According to the definitions in the real-time systems community, we should call each data sample a job. However, as each task has only one job in this system, we use task for each data sample for simplicity.}~\cite{shi2009hash, liu1991algorithms}, $\tau$. Data samples enter \Sys~ in a sporadic manner and multiple data samples/tasks can exist at any time point. The $i^{th}$ task is defined at $\tau_i$ where $D_i, e_i^j$ are the deadline of task $\tau_i$ and execution time of $j^{th}$ subtask of task $\tau_i$. The subtasks maintain a strict precedence order. An imprecise task $i$ is divided into two portions -- mandatory and optional. According to the definition of imprecise scheduling, successful execution of the mandatory portion within deadline is considered as schedulable~\cite{shi2009hash, liu1991algorithms}. Figure~\ref{fig:task_model} shows the task model of a task $\tau_i$. Each subtask consists of multiple units that execute atomically in an batteryless system that maintain the precedence order. A unit is similar to a task in task-based intermittent models mentioned in ~\cite{gobieski2019intelligence, gobieskiintermittent, colin2018termination, maeng2017alpaca} that needs to be restarted if there is a power down before it finishes. The scheduler of \Sys~ works with the subtasks and the units are maintained by SONIC~\cite{gobieski2019intelligence}.

\parlabel{Utility and Runtime Task Partitioning.}
The utility is an application specific parameter that indicates the system's goal. For example, in a control system, the completion of a correct control task results in maximum utility.  The utility of a task has a non-decreasing and non-linear correspondence with execution of each subtask. Mandatory portion of a task contains the subtasks which need to be executed to achieve a minimum utility. The rest of the subtasks belong to the optional portion. Unlike traditional imprecise computing ~\cite{shi2009hash, liu1991algorithms} where the number of subtasks in the mandatory portion is a pre-knowledge, the number of subtasks in the mandatory portion of \Sys~ is determined at run-time. We define such imprecise computing model as \textit{Dynamic Imprecise Computing}. 

\parlabel{Preemption and Task Switching.}
Each subtask performs a semantically integrated operation and cannot be preempted by the scheduler. However, the scheduler is allowed to preempt a task at the end of each subtask. This task-model follows the cooperative preemption task model at the subtask level~\cite{musliner1993circa}. Note that, a subtask can be preempted due to a power failure by the energy manager, but this is not related to the scheduler.

\subsection{Scheduling for Persistent Systems}
\label{sec:persistent}
Before we introduce the scheduling algorithm for an intermittently powered system, we discuss the scheduling algorithm for a persistently powered system. We consider that the CPU utilization~\cite{yuan2003energy} can be higher than one because in the intermittent system the power failure virtually blocks the CPU and increases the CPU utilization. As theoretically no scheduler can schedule all the tasks when the CPU utilization greater than one~\cite{yuan2003energy}, our goal is to maximize the number of tasks that can be scheduled.

In order to schedule dynamic imprecise tasks online, we propose a priority function ($\zeta$) which considers both the deadline and the utility of tasks. It also considers the effect of mandatory and optional portions which are crucial for imprecise scheduling. We define the priority function  as following:
\begin{equation}
    \zeta = (1 - \alpha (D_i - t_c)) + (1 - \beta U_i) + \gamma
\end{equation}
Here, $D_i$ and $U_i$ is the deadline and current utility of the task $\tau_i$ respectively. $t_c$ is the current time, and $\alpha$ and $\beta$ are the scaling factors. Finally, $\gamma$ is the \textit{imprecise factor} which defines if a task $\tau_i$ is currently executing a mandatory subtask or an optional one. The following equation expresses the imprecise factor ($\gamma$). 
\begin{equation}
    \gamma = 
    \begin{cases}
    1, & $mandatory portion $ (U_i < U_t)\\
    0, & $optional portion $ (U_i \geq U_t)
    \end{cases}
\end{equation}
Here, $U_t$ is the utility threshold that indicates the end of the mandatory portion. Imprecise factor guarantees the precedence of the mandatory portions before the optional portions. 

\begin{table}[!htb]
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{1}{|c|}{\multirow{2}{*}{Task}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Release \\ Time\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Total\\ Layers\end{tabular}}} & \multicolumn{2}{c|}{Task Set 1}                                                                                 & \multicolumn{2}{c}{Task Set 2}                                                             \\ \cmidrule(l){4-7} 
\multicolumn{1}{|c|}{}                      & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{c|}{}                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mandatory\\ Layers\end{tabular}} & \multicolumn{1}{c|}{Deadline} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mandatory\\ Layers\end{tabular}} & Deadline \\ \cmidrule(r){1-7}
$\tau_1$                                    & 0                                                                                             & 7                                                                                            & 2                                                                               & 45                            & 5                                                                               & 59       \\
$\tau_2$                                    & 25                                                                                            & 7                                                                                            & 4                                                                               & 56                            & 2                                                                               & 69       \\
$\tau_3$                                    & 50                                                                                            & 7                                                                                            & 3                                                                               & 93                            & 1                                                                               & 84       \\ \bottomrule
\end{tabular}
}
\caption{Task Description}
\vspace{-.1in}
\label{tab:load_des_algo}
\end{table}

\begin{figure}[!htb]
    \centering
    \includegraphics{fig/task_algo.pdf}
    \vspace{-.2in}
    \caption{Subtask execution time}
    \label{fig:exec_algo}
\end{figure}

\begin{figure}[!htb]
    \centering
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/EDF_example.pdf}}
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/Priority_example.pdf}}
    % \\
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/EDF_example2.pdf}}
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/Priority_example2.pdf}}
    \includegraphics[]{fig/steady_example.pdf}
    \caption{(a) EDF fails to meet imprecise deadline. (b) Priority function meets imprecise deadline (c) EDF meets deadline with 80\% accuracy (d) Priority function meets deadline with 88.7\% accuracy.}
    \vspace{-.2in}
    \label{fig:schedule_example}
\end{figure}


\parlabel{Example.} 
We consider two sets of three tasks described in Table~\ref{tab:load_des_algo}. We consider accumulated accuracy as utility function. Each task has seven subtasks with execution time shown in Figure~\ref{fig:exec_algo}. 
Figure~\ref{fig:schedule_example}(a-b) shows the execution of tasks from set1 using EDF and priority based scheduling algorithm. In Figure~\ref{fig:schedule_example}(a), EDF fails to schedule the second task; however, priority based scheduler can schedule all three tasks in Figure~\ref{fig:schedule_example}(b). In Figure~\ref{fig:schedule_example}(c-d) we consider tasks from set2. Even though both EDF and priority function succeeds to schedule all the tasks, the accumulated accuracy of the EDF schedule (80\%) is higher than that of priority function schedule (88.7\%). 

\subsection{Scheduling for Intermittent System}
\label{sec:intermittent}
Scheduling in intermittently powered system is challenging due to the occurrence of power failure. In Section~\ref{sec:energy_study}, we introduce a probability of metric $\eta$ to measure predictability of an energy harvester. We use $\eta$ influenced priority function ($\zeta_I$) to schedule an intermittent system. 
\begin{equation}
    \zeta_I = 
    \begin{cases}
    (1 - \alpha (D_i - t_c)) + (1 - \beta U_i) + \gamma, &  \eta E_{curr} \geq E_{opt}\\
    \gamma( (1 - \alpha (D_i - t_c)) + (1 - \beta U_i)), &  \eta E_{curr} < E_{opt}
    \end{cases}
\end{equation}

Here, $E_{curr}$ is the current energy generation rate and $E_{opt}$ is the threshold energy generation rate. For an energy harvester with high \Factor, we leverage the predictability of energy generation and boost the utilization. When the $E_{curr}$ is high, we schedule both mandatory and optional subtasks, opportunely taking advantage of correlated energy event occurrence. Otherwise, the scheduler considers the high probability of energy event non-occurrence and schedules \textit{conservatively}. In this case we only schedule the mandatory subtasks. When \Factor~ is low, the predictability of energy generation is minimal and thus the system schedules conservatively unless the energy generation is very high.

$\zeta_I$ minimizes two types of energy waste in energy harvesting systems~\cite{buettner2011dewdrop}. The first one is running unnecessary tasks which we avoid when $\eta E_{curr} < E_{opt}$. The second wastage occurs by not running tasks when the harvester is getting continuous energy from the source to keep the capacitor charged. We handle this wastage by running optional subtasks when $\eta E_{curr} \geq E_{opt}$.


\subsection{ A Special Case: Scheduling Deterministic Intermittent System.}
\label{sec:intermittent_special}
Deterministic intermittent power source is a special type of intermittent source where energy harvesting pattern is known; e.g., RF harvester with periodic signal transmission. We propose a more simplistic approach for such systems. To schedule in such a system, we pretend this energy intermittence as a hypothetical periodic task (termed \textbf{energy task}) with the highest priority, and it is pre-scheduled offline. This assumption allows us to schedule the tasks with energy constraints taken in to account. Note that we assume that energy task can preempt the conditional-preemptive tasks at any time instance.
\begin{figure}[!htb]
    \centering
    \vspace{-.3in}
    \subfloat{\includegraphics[width=.45\textwidth]{fig/deterministic_EH_example.pdf}}
    \caption{(a) Missed a imprecise deadline of the job by not taking  the deterministic intermittence power into account. (b) Successfully scheduled two tasks by considering deterministic energy pattern as energy tasks.  }
    \vspace{-.1in}
    \label{fig:deterministic_EH_example}
\end{figure}

In Figure~\ref{fig:deterministic_EH_example}, we consider the first two tasks ($\tau_1$ and $\tau_2$) from Figure~\ref{fig:schedule_example}(a-b). We consider a periodic power source with a period of 8 time units. In Figure~\ref{fig:deterministic_EH_example}(a), the system does not consider the energy intermittence and misses the imprecise deadline for $\tau_2$. However, by considering the deterministic power source as energy tasks, the system schedules both tasks successfully.  


==> 05B_agileDNN.tex <==
\section{Agile DNN and Model Adaptation}
In this section, we first describe the task model for semi-supervised learning with deep neural features. Then we describe the construction of agile DNN Model and approximate adaptation of adaptive models. 

\subsection{Agile DNN Task Model}

\parlabel{Define Task. }
We define each data sample entering \Sys~ as a task. The execution of one layer of agile DNN along with corresponding k-means model is defined as a subtask. In a subtask, \Sys~ extracts features of the data sample  from a specific layer of the agile DNN model, use those features to execute a semi-supervised k-means model and update the centroids. 
Figure~\ref{fig:dnn_flow} shows the task model of a task, $\tau_i$. $\tau_i^{k-1}$, $\tau_i^{k}$ and $\tau_i^{k+1}$ are the subtasks of $\tau_i$ that represent the $k-1$, $k$ and $k+1$ layers of the DNN with corresponding semi-supervised k-means clustering, respectively.
\begin{figure}[!htb]
    \centering
    \vspace{-.2in}
    \includegraphics{fig/dnn_flow.pdf}
    \vspace{-.15in}
    \caption{Flow of agile DNN task $\tau_i$ where $k-1$, $k$ and $k+1$ are different DNN layers (subtasks). $U_i^{k-1}$, $U_i^{k}$ and $U_i^{k+1}$ are the utility of $\tau_i$ after execution of $k-1$, $k$ and $k+1$ layers.}
    \vspace{-.18in}
    \label{fig:dnn_flow}
\end{figure}

\parlabel{Early Termination. }
For an energy constraint system, computing accuracy of unlabeled data is expensive. Popular model validation techniques including inter-intra cluster distance measure are computation heavy~\cite{bashima2019ondevice}. Therefore, instead of using accuracy as utility, we propose a light weight utility function. We define the difference between the distances of the data point from two nearest centroids as utility. 
\begin{equation}
    U_i = |d_a - d_b|
\end{equation}
Here, $d_a$ and $d_b$ are the distance of the data sample from the closest and the second closest centroid. The intuition behind this definition is that a data point at similar distances from two centroids is not confident enough regarding which cluster it belongs to. Therefore, more complex representation is required to determine the cluster with confidence. In Figure~\ref{fig:policy}, the distance between the data sample and two nearest centroids, $c_1$ and $c_3$ are $d_1$ and $d_3$ respectively. In Figure~\ref{fig:policy}(a) the difference between $d_1$ and $d_2$ are very small and thus the confidence of the data sample being a member of cluster 3 is low. Therefore more complex representation is needed to provide more confident result and further execution of agile DNN is needed. On the other hand, in Figure~\ref{fig:policy}(b) the difference between $d_1$ and $d_2$ are prominent and thus the data sample belongs to cluster 3 with high confidence. Thus further execution is not needed. 
\begin{figure}[!htb]
    \centering
    \vspace{-.12in}
    \includegraphics[width=0.35\textwidth]{fig/policy.pdf}
    \vspace{-.16in}
    \caption{Early Termination Policy}
    \vspace{-.16in}
    \label{fig:policy}
\end{figure}
Figure~\ref{fig:dnn_flow}, shows the early termination policy and the execution of subtasks. Here, $U_i^{k-1}$, $U_i^{k}$ and $U_i^{k+1}$ are the utility of $\tau_i$ after execution of $k-1$, $k$ and $k+1$ layers. $U_t$ is the threshold utility.


\subsection{Agile DNN Construction}
Our termination policy utilizes the output vector at each layer as learned representation rather than solving a joint optimization problem to perform both classification and clustering at the last layer~\cite{yang2016towards}. To ensure higher utility, we need to learn a representation which maximizes the distance between the representation of different classes and also minimizes the space between the representation of the same class. Contrastive loss function obtain this at the final ~\cite{islam2019soundsemantics}. However, easier samples can be distinguished with simpler representation from previous layers. Thus, we need to achieve distinctive representation in earlier layers.

\parlabel{Layer-Aware Loss Function. }
In order to accomplish this, we propose a layer-aware loss function inspired by the contrastive loss ~\cite{islam2019soundsemantics}. We use a convex combination of contrastive loss at each layer as a loss function that allows the system to have better distinguishable representation at the preceding layer. To ensure distinctive representations at earlier layers, early layers have more weights than the deeper layers. Therefore, easy samples get enough distinguishable representation at an earlier layer of a network mitigating their need to execute all the layers. Note that this loss function is used during the training of the agile DNN model in a traditional deep learning computing system.

The layer-aware loss function, $l$ is represented as follows. 
\begin{align}
\label{eqn:eqlabel}
\begin{split}
     l = \sum_{i=1}^{i=L} \alpha_i \times l_c(W_i, X_i^1, X_i^2, ... , X_i^N); & 
    ~where, \sum_{i=1}^{i=L} \alpha_i = 1
\end{split}
\end{align}
Here, $\alpha_i$ is the convex coefficient at layer $i$. $L$ and $N$ represent the total number of layers  and classes in the network respectively. $W_i$ is the learnable weights of the network at layer $i$. $X_i^1, X_i^2, ... , X_i^N$ are the vectors of each class at layer $i$. $l_c$ is the contrastive loss function and for two classes $X_i^1$ \& $X_i^2$ at layer $i$ it is defined as following. 
\begin{multline}
    l_c(W_i, X_i^1, X_i^2) = (1-Y) \dfrac{1}{2} G_{W_i}(X_i^1)−G_W(X_i^2) \\
    + Y \dfrac{1}{2} max(0, \Delta - G_{W_i}(X_i^1)−G_{W_i}(X_i^2))
\end{multline}
Here, $G_{W_i}(X_i^j)$ is the representation output of a member of class j; where j = 1, 2, .., N; at layer $i$. Coefficient $Y = 0$ if $X^1$ and $X^2$ belong to the same class and $Y = 1$ otherwise. The term $\Delta$ represents the distance margin that is maintained between the representation of different classes.





==> 05C_adaptation.tex <==
\parlabel{Adaptation. }
Due to the prior termination in previous layers, a group of data fails to affect the clustering model with complex representation from deeper layers. It hinders the adaptation of cluster model with more complex features. One solution is to execute the non-linear calculation for each sample to get more complex representation and update the models.  This calculation includes matrix multiplications, addition, and a non-linear function; e.g., RELU activation. However, this execution contradicts to our goal of avoiding unnecessary computations for simple data. This dispute imposes an exciting challenge of updating the centroid of layer $L_{i+k}$ from the centroid of layer $L_i$ with light-weight calculation, where k = 1,2,3, ..., n. Such a challenge never occurred before as this is the first work combining model update with prior termination.

Let $C_j^i$ be a centroid of the clustering model at layer $i$ where $j$ is the number of members in the cluster where $C_{j}^i = \frac{\sum_{k=1}^j X_k^i}{j}$. For the next layer, $i+1$, the centroid is 
\begin{equation}
\label{eq:actual}
    C_{j}^{i+1} = \frac{\sum_{k=1}^j \sigma(W^{i+1} \times X_k^i)}{j}
\end{equation}
Here, $W^{i+1}$ and $B^{i+1}$ are weight and bias for layer $i+1$ respectively. $\sigma$ is the non-linear function; e.g., RELU. This formula requires at least $j$ multiplication. As multiplication is an expensive function, our goal is to avoid using them. Therefore, we approximate Equation~\ref{eq:actual} using the following equation and reduce the number of multiplication by $j-1$. 
\begin{equation}
\label{eq:actual1}
    C_{j}^{i+1} = \frac{\sigma(W^{i+1} \times \sum_{k=1}^j X_k^i)}{j}
\end{equation}
We assume that the non-linear function is RELU activation function. So, $\sigma(x) = max\{0, x\} = \frac{x + |x|}{2}$. After applying the RELU function, we observe that the error, $er$ is 
\begin{equation}
    er^{i+1} = \frac{\sum_{k=1}^j |W^{i+1} \times X_k^i| - |W^{i+1} \times \sum_{k=1}^j X_k^i|}{2j}
\end{equation}



==> 07_evaluation.tex <==
\section{Evaluation}
\begin{figure}[!htb]
     \centering
     \subfloat{
         \includegraphics[width=0.16\textwidth]{fig/MCU.jpg}
     }
     \subfloat{
         \includegraphics[width=0.12\textwidth]{fig/Solar.jpg}
     }
     \subfloat{
         \includegraphics[width=0.16\textwidth]{fig/RF.jpg}
     }
     \vspace{-.1in}
    \caption{\Sys~ experimental setup}
    \label{fig:hardware}
    \vspace{-.18in}
\end{figure}
\subsection{Experimental Setup}
\label{sec:setup}
\parlabel{Computational Device. }
For evaluation we use TI-MSP430FR5994~\cite{msp430} at 16MHz. This micro-controller is equipped with 256KB of FRAM, 8KB of SRAM, 16-channel 12-bit ADC, 6-channel direct memory access (DMA) and a Low Energy Accelerator (LEA). It has an operating voltage range of 1.8V to 3.6V. To program this device we use the Linux distribution and GCC compiler with an ez-FET programmer. \Sys~ uses fixed point calculation and flip-flop buffers to enable DNN execution in MSP430\footnote{The implementation of \Sys~ is available on \href{https://github.com/zygarde-sensys/Zygarde.git}{https://github.com/zygarde-sensys/Zygarde.git}}. 

To train the agile DNN model mentioned in Table~\ref{tab:network} we use an Intel Core i7 PC with RTX2080 GPU. We train the network offline and compress it with rank decomposition or separation ~\cite{bhattacharya2016sparsification, chollet2017xception, xue2013restructuring, de2000multilinear, de2000best, tucker1966some} and pruning~\cite{han2015deep, nabhan1994toward}. We execute this compressed trained network for inference in our target device TI-MSP430FR5994.


\parlabel{Energy Harvester. }
We harvest energy from two ambient sources -- solar and RF. We use a flexible Ethylene Tetrafluoroethylene (ETFE) based solar panel~\cite{solar_panel} that outputs 6V at 1W. We use a LTC3105 step up DC/DC converter with a start up voltage of 250mV~\cite{ltc_3105} to charge the capacitor with the solar panel. A Powercast P2210B~\cite{power_cast} is used to harvest RF energy from  a 3W Power-caster transmitter~\cite{powercase_transmitter}, Figure~\ref{fig:hardware}. For all the experiments with intermittent power we use a 50mF capacitor. For persistently powered experiments we rely on the power supply from the ez-FET of the MSP430 launchpad.

\parlabel{Sensor Peripheral. }
For audio sensor, we use a Electret microphone~\cite{BOB} that draws 3.1mA current and has a start up time of 125ms. We utilize the built in ADC and internal clocks to read data from the microphone. To calculate the FFT we use the LEA and use DMA to write data to the FRAM without occupying the CPU. 

\parlabel{Time Keeping Peripheral. }
Like ~\cite{yildirim2018ink,hester2017timely}, we use a real-time clock, DS3132~\cite{timer} via I2C, for time keeping. This choice is made for the ease of implementations. Note that, we only use this clock during power up for syncing up and maintaining time with the internal clock of the MCU. This real-time clock is easily replaceable with SRAM and capacitor based time-keeping system during power off periods~\cite{rahmati2012tardis, hester2016persistent}. Note that both time-keeping and intermittent execution in batteryless system is out of the scope of this paper.

\parlabel{Libraries. }
We use MSP430 libraries provided by Texas Instrument. For maintaining intermittent execution \Sys~ uses SONIC~\cite{gobieski2019intelligence} and the dependant libraries (e.g. ALPACA~\cite{maeng2017alpaca}) of this project. For training the agile DNN model we use Google's Tensorflow~\cite{45381}. 

\parlabel{Datasets. }
To evaluate our algorithms we use two popular datasets MNIST~\cite{lecun1998mnist} and ESC-10~\cite{piczak2015dataset}. MNIST is a image based dataset which consists of $28 \times 28$ pixel images and 10 classes. ESC-10 consists environmental sounds of 10 classes. Each audio clip is 5s long and has a sampling rate of 44KHz. To accommodate this dataset with our resource constrained device, we take the middle 1s audio and down-sampled it to 8KHz.  

\parlabel{Controlled Energy Source. }
To evaluate the system with different \Factor, we perform controlled experiments with the energy sources. For RF, we vary the distance between the harvester and the transmitter from 1 feet to 5 feet. For solar, we simulate the sun with three dimmable bulbs with varying intensity (5.6 Klx - 35 Klx) as shown in Figure~\ref{fig:hardware}. Note that, for the real-life experiment we use outdoor scenarios and windowed rooms to get the sunlight.  


\subsection{Algorithm Evaluation}

\parlabel{Effect of Layer-Aware Loss Function and Early Termination. }
In this section, we evaluate our proposed layer-aware loss function, early termination and adaptation. We train all models with same hyper-parameters and only use the training dataset. While inference we rely on the testing dataset provided by MNIST and ESC-10 (we use fold 1 only) containing 10,000 and 80 samples respectively. Note that, layer-aware loss function and early termination are applicable for any system, not just intermittently powered ones. Therefore, we do not bring the energy harvesting aspect in this evaluation and perform the evaluation on a persistently powered system. We compare our layer-aware loss function (L) and layer-aware loss function with adaptation (AL) with cross-entropy loss (CE)~\cite{zhang2018generalized} and contrastive loss (C)~\cite{islam2019soundsemantics}. We also consider a network trained with cross-entropy loss which only exits in the last layer similar to the one shown in SONIC~\cite{gobieski2019intelligence}.

\begin{figure}[!htb]
    \centering
    \includegraphics{plot/Early_exit_mnist.pdf}
    \vspace{-.18in}
    \caption{Prior Termination Evaluation MNIST.}
    \label{fig:early_exit_mnist}
\end{figure}
\begin{figure}[!htb]
    \centering
    \includegraphics{plot/Early_exit_esc.pdf}
    \vspace{-.18in}
    \caption{Prior Termination Evaluation ESC-10.}
    \vspace{-.18in}
    \label{fig:early_exit_esc}
\end{figure}
For MNIST dataset in Figure~\ref{fig:early_exit_mnist}, we observe that for cross-entropy loss (CE) with early termination decreases the accuracy along with the execution time. However, with the layer-aware loss(L) we increase the accuracy by 9.45\% from cross-entropy loss (CE) and 3.19\% from contrastive loss (C) while keeping similar execution time. Layer-aware loss function with adaptation (AL) increases the accuracy by 1\% and allows more samples to terminate in the early layers. 

\begin{figure*}[!htb]
    \centering
    \includegraphics{plot/mnist_schedule.pdf}\vspace{-.2in}
    \vspace{-.15in}
    \caption{Realtime Scheduling for Systems with different ($\eta$) on MNIST test dataset.}
    \label{fig:schedule_mnist}
\end{figure*}
\begin{figure*}[!htb]
    \centering
    \includegraphics{plot/esc_schedule.pdf}
    \vspace{-.2in}
    \caption{Realtime Scheduling for Systems with different ($\eta$) on ESC-10 test dataset.}
    \label{fig:schedule_esc}
\end{figure*}

ESC-10 is a complex dataset where previous works achieves 73\% accuracy using models with three convolution layers, data augmentation and, 44KHz sampling rate~\cite{piczak2015environmental}. Our network takes downsampled audio data of 1s duration and achieves 70\% accuracy. 
In Figure~\ref{fig:early_exit_esc}, layer-aware loss function(L) achieves 76.25\% accuracy and decreases the execution time by 1.22 minutes. Note that, layer-aware loss function with approximation (AL) does not show any improvement over layer-aware loss in this scenario because all data samples of several classes exit the network in earlier layers minimizing the need of approximate adaptation for deeper layers. 



\parlabel{Performance of Real-Time Scheduler. }
In this section, we evaluate our proposed scheduling algorithm for dynamic imprecise tasks that is applicable to both persistently (Section~\ref{sec:persistent}) and intermittently (Section~\ref{sec:intermittent}) powered systems for different \Factor. We evaluate the system with two different CPU utilization. 

For MNIST dataset in Figure~\ref{fig:schedule_mnist}, we consider a CPU utilization$\geq1$. Thus even with persistent power we can not schedule all tasks. Without early termination the majority of samples could not be scheduled as they keep on waiting in the queue. But, with early exit 75\% of samples can be scheduled. We consider sporadic tasks with a period of 3 seconds and the deadline is twice the period. According to the definition of imprecise computing, we consider completion of mandatory portion as a successful scheduling~\cite{shih1992line}. For ESC-10 dataset in Figure~\ref{fig:schedule_esc}, we consider that CPU utilization$\leq1$, the period is 0.36 minute and the deadline is twice the period.

We compare our approach with earliest deadline first (EDF) algorithm and a variation of EDF that only executes the mandatory portion (EDF-M). We consider various \Factor~ and use three systems that persistently powered, solar powered and RF powered. We notice that in all the cases \Sys~ can successfully schedule higher number of tasks with higher accuracy. There are two major things to notice in Figure~\ref{fig:schedule_mnist} and Figure~\ref{fig:schedule_esc}.

$\bullet$ When \Factor~ is high \Sys~ increases the number of tasks with correct result by executing some of the optional portion. For a 100\% accurate utility function the performance of ~\Sys~ and EDF-M would be same. 

$\bullet$ For small \Factor~ the performance of \Sys~ and EDF-M is the same because it satisfies the second condition of Equation~6 which only executes mandatory portion. 

$\bullet$ The number of tasks that can be scheduled does not depend only on \Factor~ but also on the harvested energy.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics{plot/eta_runtime_solar.pdf}
%     \caption{Active Execution Time of Realtime Scheduling for systems with different $\eta$ with solar harvester.}
%     \label{fig:persistent_time}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{plot/real_solar.pdf}
    \vspace{-.2in}
    \caption{Real-life evaluation of \Sys~ with solar}
    % \vspace{-.2in}
    \label{fig:real-solar}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{plot/real_rf.pdf}
    \vspace{-.2in}
    \caption{Real-life evaluation of \Sys~ with RF}
    % \vspace{-.2in}
    \label{fig:real-rf}
\end{figure}

\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccllcl@{}}
\toprule
Scenario  & Energy Source & Source Power & Harvester Placement & Additional Cause      & Target Event & \multicolumn{1}{c}{Other Audios}          \\ \midrule
Street           & Solar         & 74 -- 80 Klx    & Pavement    & Vehicle on the closest lane & Car Honk     & Silence, Dog, Human Voice, Car            \\
Shaded Park           & Solar         & 1.8 -- 0.6 Klx    & Under Tree          & People, objects and cloud   & Dog Bark     & Silence, Car, Car Honk, Human Voice       \\
Staircase  & Solar         & 0.5 -- 0.3 Klx    & Edge of the Railing & People and cloud            & Human Voice  & Silence, Car, Car Honk, Dog Bark          \\
Nursery               & RF            & -.48 -- -1.66dB    & On Desk             & Change of distance                  & Baby Cries   & Silence, Human Voice, Washer, Printer     \\
Laundry               & RF            & -.48 -- -1.91dB      & On Counter          & Change of distance                  & Washer       & Silence, Human Voice, Baby Cries, Printer \\
Office                & RF            & -1.59 -- -1.91dB      & On Desk             & Change of distance                  & Printer      & Silence, Human Voice, Baby Cries, Printer \\ \bottomrule
\end{tabular}
}
\caption{Real-life evaluation setup}
\vspace{-.3in}
\label{tab:real_setup}
\end{table*}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics{plot/solar_eta_hi_schedule.pdf}
%     \caption{Realtime Scheduling for Solar Powered System ($\eta$=0.712). 7717 data samples (tasks) entered the system.}
%     \label{fig:persistent_system}
% \end{figure}

\subsection{Real-World Application Evaluation}
 
\parlabel{Experimental Setup.}
In this section, we evaluate your system in an uncontrolled environment. We present an acoustic event detector as the application. We choose six scenarios with seven acoustic events. In three of these scenarios we use a solar harvester and for the rest we use a RF harvester. Table~\ref{tab:real_setup} describes the different scenarios along with the target events. We rely on the natural events for hindrance in power generation for the solar harvested systems. For example in the \emph{street} scenario, the harvester with solar panel is kept on the edge of the pavement. The vehicles (cars, buses) passing through the nearest lane to the pavement is blocking the sun and thus introducing hindrance in energy generation. However, due to the lack of programmable RF harvester or proper setup to harvest from WiFi, we change the distance between RF harvester and transmitter. We use the same setup mentioned in Section~\ref{sec:setup} for the computation and sensing unit. Note that other sound sources were present in all scenarios and we included silence as an event in the classifier for training. 




% \begin{table}[]
% \begin{tabular}{@{}p{1cm}p{.6cm}p{1.3cm}p{1.5cm}p{1.3cm}p{1.5cm}@{}}
% \toprule
% Scenario  & Energy Source & Source \bnote{Power} & Harvester Placement & Hindrance Cause      & Target Event \\ \midrule
% Street           & Solar         & 74-80 Klx    & Pavement    & Vehicle & Car Honk     \\
% Park           & Solar         & 1.8-0.6 Klx    & Under Tree          & People   & Dog Bark     \\
% Staircase            & Solar         & .5-.3 Klx    & Railing & People            & \bnote{Voice}  \\
% Nursery               & RF            & 0.5 ft - 3 ft    & On Desk             & Distance                  & \bnote{Baby Cries}   \\
% Laundry               & RF            & 1 ft - 5 ft      & On Counter          & Distance                  & Washer       \\
% Office                & RF            & 2 ft - 5 ft      & On Desk             & Distance                  & Printer      \\ \bottomrule
% \end{tabular}
% \end{table}


\parlabel{Performance.}
In Figure~\ref{fig:real-solar} shows the voltage across the capacitor along with the operating voltage of the computational unit of the three scenarios where the system is powered by a solar harvester. Note that the voltage across the capacitor and operating voltage is used to measure energy generation rate. The system runs a DNN with a single convolution layer and two fully connected layers. The execution time varies between 1.7 s and 3 s depending on the early exit. Among the 30 events we experienced we have four incorrect detection. We experience three deadline misses even though the detection is accurate. We miss four samples due to intermittence as the system did not have enough energy to be turned on. 

Similar to Figure~\ref{fig:real-solar}, Figure~\ref{fig:real-rf} shows the result for scenarios with RF harvester. We notice two interesting facts with this experiment. The first one is that the MCU experience higher intermittence rate for RF harvester than solar harvester. However, the duration of power off is much higher in solar harvester specially when we do not have the direct sunlight.  



%  need to do as much as possible with msp430
% \begin{itemize}
%     \item In dataset accuracy and time with and without termination policy
%     \item Layer Aware Loss Function $\checkmark$
%     \item Approximate Representation Transformation vs no transformation vs all computation. Accuracy and time. 
%     \item With + Without the algorithm in both powered and powerless systems
%     \item Real-life performance accuracy and #deadline miss
% \end{itemize}
% \subsection{Layer-Aware Loss Function}
% We use audio dataset ESC-50 for evaluating the performance of layer-wise loss function. 
% \\
% In Figure~\ref{fig:cluster_data}, we randomly select classes and observe the number of layers needed for achieving at least 80\% accuracy for clustering. We notice that for various number of clusters, some class combination requires more layers than the previous. To illustrate, cat and toilet flush are very distinguishable sounds and can be clustered with 93\% accuracy using the representation learned from the first layer of the network. On the other hand, train and helicopter both having similarity in audio needs execution of 5 layers to achieve 81.25\% accuracy.
% % Accuracy with and without Layer Adaptation for different dataset (Lenet, Urban Sound 8K, ESC-10, Google Keyword Dataset). (same configuration)/ X-axis runtime, Y-axis accuracy, Shape for different Dataset, Colored chart for the data distribution. 

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.45\textwidth]{plot/layer_class.pdf}
%     \caption{Different combination of classes needs different number of layers to achieve at least 80\% accuracy \textbf{NUMBER OF CLUSTERS}}
%     \label{fig:cluster_data}
% \end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.45\textwidth]{plot/loss_compare.pdf}
%     \caption{Performance comparison of layer-aware loss function, contrastive loss function and regular loss function. \textbf{LAYER-AWARE LOSS}}
%     \label{fig:zygarde_loss}
% \end{figure}

% In Figure~\ref{fig:zygarde_loss}, we compare the performance of our proposed layer-aware loss function, contrastive loss function and regular loss function with Adam optimized commonly used in deep neural network. We train all three systems for same number of epoch and same dataset. As easy data we choose 10 classes from ESC-10 dataset consisting of sneezing, dog barking, clock ticking, crying baby, crowing rooster, rain, sea waves, fire crackling, helicopter and chainsaw. As hard data we choose two classes from each of the five categories of ESC-50 dataset. These classes are -- church bells, clock ticking, frog croaking, baby crying, crickets,  mouse clicking, siren, insects flying, sneezing and water pouring. We observe that for easy data using our layer-aware loss function the system needs to execute four layers to achieve at least 65\% accuracy where as using contrastive loss function and regular loss function it needs to execute five layers. In the scenario of hard data, we can achieve 65\% accuracy after executing six layers using layer-aware loss function. However, the other two loss functions failed to achieve 65\% accuracy even after executing all the six layers. They achieved 61.25\% and 56.25\% accuracy at the final layer using contrastive loss function and regular loss function, respectively. 



% \subsection{Early Exit Policy}
% We use the ESC-Audio dataset.

% \subsection{Representation Transform}
% X axis different layer of different dataset. Y axis error of the transformed data. 

% \subsection{Online Real-time Scheduler}
% In order to verify the usability of the real-time scheduler, we develop a simulated scenario. In this simulation, we have a periodic task with 50 periodic jobs with a representation learner of 10 layers. Each layer execution consists of the time needed for representation learning and clustering. We have a random energy simulator system to simulate the energy harvesting system. 

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=.45\textwidth]{plot/simulation_acc.pdf}
%     \caption{Simulation Accuracy }
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=.45\textwidth]{plot/simulation_en.pdf}
%     \caption{Simulation Energy}
%     \label{fig:my_label}
% \end{figure}


% \bnote{change beta in scheduling to compare quality of inference vs diversity of inference}

% create an simulation to stochasticity of energy harvester
% first half i sregular pattern and second half is irregular pattern
% real timeline over data.

% First audio data comes in and exdecute few layer and execute in hardware
% Early Exit
% Scheduling 
% do the real system first. 
 


==> 0X_related.tex <==
\section{Related Work}
\label{sec:related}

\parlabel{Intermittent Computing. }
Intermittently powered systems experience frequent power failure that resets the software execution and results in repeated execution of the same code and inconsistency in non-volatile memory. Previous works address the progress and memory consistency using software check-pointing~\cite{ransford2012mementos, maeng2018adaptive, hicks2017clank, lucia2015simpler, van2016intermittent, van2016intermittent, jayakumar2014quickrecall, mirhoseini2013automated, bhatti2016efficient}, hardware interruption~\cite{balsamo2015hibernus, balsamo2016hibernus++, mirhoseini2013idetic}, atomic task based model~\cite{maeng2017alpaca, colin2016chain, colin2018termination} and, non-volatile processors(NVP)~\cite{ma2017incidental, ma2015architecture}. Recently ~\cite{gobieskiintermittent, gobieski2019intelligence} proposes a special software system for intermittent execution of deep neural inference combining task atomic task based model with loop continuation. \Sys~ relies on  ~\cite{gobieskiintermittent, gobieski2019intelligence} for intermittent computation of deep neural network.   

\parlabel{Timeliness of Batteryless Systems. }
Prior works on intermittent computing proposes runtime systems that increases the likelihood of a task completion by finding optimum voltage for task execution~\cite{buettner2011dewdrop}, adapting execution rate~\cite{sorber2007eon, dudani2002energy} and discarding stale data~\cite{hester2017timely}. However, none of these works consider the accuracy/utility of the running application or the real-time deadline-aware execution of tasks. 
Some works have addressed scheduling in wireless sensors~\cite{zhu2012deos, moser2006lazy, moser2007real} but none of them consider the higher computation load of intermittent computing systems. ~\cite{yildirim2018ink} proposes a reactive kernel that enables energy aware dynamic execution of multiple threads. Note that they do not consider deep neural tasks or utilize early termination of tasks for increasing schedulability. Unlike \Sys~ which schedules multiple incoming data samples,  ~\cite{yildirim2018ink} schedules kernel threads and can only have one data sample in the system at a time point. 
Other works focuses on maintaining time-keeping through power loss~\cite{rahmati2012tardis, hester2016persistent}. Our work is a complementary of these works and relies on these techniques for time keeping. 

\parlabel{Compression and Partial execution of DNN. }
Recent works have focused on reducing the cost of DNN inference by pruning and splitting models without compromising accuracy~\cite{han2015deep,nabhan1994toward, yao2017deepiot, yao2018rdeepsense, yao2018apdeepsense, yao2018fastdeepiot}. Other works have focused on reduction of floating point and weight precision~\cite{johnson2018rethinking, de2017understanding, han2016eie}, and factorization of computation~\cite{bhattacharya2016sparsification, chollet2017xception, nakkiran2015compressing,szegedy2017inception, szegedy2015going, szegedy2016rethinking, wang2017factorized} to reduce storage and computation cost. The proposed binary networks~\cite{courbariaux2015binaryconnect, hubara2016binarized,rastegari2016xnor, courbariaux2017binarynet} are not suitable for energy harvesting systems due to the higher number parameters needed by such systems~\cite{gobieski2019intelligence}. Even though these works are crucial for enabling DNN execution in batteryless system these can be enhanced by exploiting the fact that in real-life data are usually is a combination of easy examples and difficult examples and the easy examples do not need the full DNN inference~\cite{bolukbasi2017adaptive, figurnov2017spatially, leroux2017cascading}. Unlike prior works that require an additional classifier after each layer, \Sys~ depends on semi-supervised models to reduce computational overhead. ~\cite{bateni2018apnet, zhou2018s} proposes scheduling algorithm for deep neural network in GPU and does not consider the constraints introduced by embedded system and intermittent power supply. 

\parlabel{Modeling Energy Harvesting System. }
~\cite{san2018eh} analytically model the trade-off associated with backing up data to maximize forward propagation. Even though energy harvesting system for a specific energy source has been analyzed and modeled before~\cite{crovetto2014modeling, sharma2018modeling, jia2018modeling}, none of the prior works focus on modeling energy harvesting systems irrespective of energy source. 

\section{Discussion}
After execution an DNN layer, \Sys~ calculates the manhattan distance of the data sample from all $n$ centriods using top $k$ features, where $n$ is the number of clusters. This requires $n\times k$ subtractions, $n\times k$ comparison (to determine absolute value) and $n\times k$ addition. \Sys~ needs $n+1$ comparisons to find the minimum distance and $k$ additions, $k$ multiplications and $k$ divisions to update a centroid. In our implementation, the highest number of $n$ and $k$ are 10 and 50, respectively. The total computation needed after each layer is 10$\times$ smaller than the required multiplication and addition needed for the smallest network layer mentioned in Table~\ref{tab:network}.

\section{Conclusion}
In this paper we propose a generic metric \Factor~ that expresses the stability on an energy harvesting system. We also utilize the fact that real-life data samples are a combination of easy and hard samples and all samples do not require the same amount of computation to achieve similar performance. We propose early termination of deep neural network without compromising much accuracy. To decrease the accuracy loss due to early termination, we propose a layer-aware loss function and achieve 9.45\% - 3.19\% increase in accuracy and 14\% decrease in execution time. We then model such DNN tasks as imprecise tasks and propose a scheduling algorithm that considers time, energy condition, \Factor~ and performance of the system. We evaluate our system with state of the art scheduling algorithms and our algorithm schedules 33\%-12\% more tasks successfully.

==> Tamzeed_ArXIV%20(Copy)/01_introduction.tex <==
%\newpage
\section{Introduction}
\label{sec:intro}

\parlabel{Batteryless Systems. } The Internet of Things (IoT) promises to make our lives efficient, productive, enjoyable, and healthier by making everyday objects capable of sensing, computation, and communication. Many of these so-called IoT devices are powered by limited-capacity batteries---which makes them mobile, small, and lightweight. Batteries, however, require periodic maintenance (e.g.,  replacement and recharging) which is an inconvenience at a large scale. To address this practical problem, batteryless IoT devices have been proposed, which harvest energy from ambient sources, e.g., solar, thermal, kinetic, and RF to power up. These devices, in principle, last forever---as long as the energy harvesting conditions are met. They typically consist of low-power sensors, microcontrollers, and energy-harvesting and management circuitry, and their applications are in many deploy-and-forget scenarios, e.g., wildlife monitoring, remote surveillance, environment and infrastructure monitoring, wearables, and implantables.

\parlabel{Time-Aware Inference. } Many IoT applications require timely feedbacks. For instance, in an acoustic monitoring system, audio events need to be detected and reported as fast as possible to initiate prompt actions. Similarly, an air-quality monitoring system needs to identify the increase of a certain air component on time for taking proper actions. Likewise, shared resources, such as gym-equipment and shared bikes in a campus, can be monitored in real-time to detect misuses or malfunctions, and to inform the authority about the incidence on time. While a batteryless system is desirable in these real-time sensing and event detection applications, the unpredictability of the harvested energy, combined with the complexity of on-device event detection tasks, complicates timely execution of machine learning-based event detection tasks on batteryless systems. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.35\textwidth]{fig/intermittencd_deadlinemiss.pdf}
            \vspace{-1em}
    \caption{(a) With constant power both deadlines are met. (b) With intermittent power, task $\tau_2$ misses deadline. (c) When, execution of the whole task is not necessary, both tasks can be scheduled successfully.}
        \label{fig:intermittent_deadmiss}
        \vspace{-1em}
\end{figure}

\parlabel{Prior Work on Timeliness. } Prior works on time-aware batteryless computing systems can be broadly categorized into two types. The first category focuses on \emph{time-keeping}, i.e., maintaining a reliable system clock~\cite{rahmati2012tardis, hester2016persistent} even when the power is out. The sporadic nature of an energy harvesting system forces it to run intermittently by going through alternating episodes of power ON and OFF phases which disrupts the continuity of the system clock. By exploiting the rate of decay of an internal capacitor and the content of the SRAM, these systems enable time-keeping during the absence of power. The second category proposes runtime systems that consider the temporal aspect of data across power failures~\cite{hester2017timely, buettner2011dewdrop, zhu2012deos, yildirim2018ink}. For instance, ~\cite{hester2017timely} discards data after a predefined interval and thus saves energy by not processing stale data, and ~\cite{yildirim2018ink, buettner2011dewdrop,zhu2012deos} propose energy-aware runtime systems to increase the chances of task completion. However, none of these consider the utility of data or exploit the property of inference tasks to plan real-time deadline-aware execution of tasks.  

\parlabel{Real-Time Intermittent Computing. } Scheduling time-aware machine learning tasks on a batteryless computing system is an extremely challenging feat. The two main sources of challenges are the \emph{intermittent power supply} and the \emph{computational demand for executing machine learning tasks}. These two challenges have been studied extensively in non-real-time settings. For instance, ~\cite{ransford2012mementos, mirhoseini2013automated,balsamo2015hibernus, balsamo2016hibernus++,maeng2017alpaca, colin2016chain, maeng2018adaptive} enable seamless execution of non-real-time tasks on intermittently powered systems by proposing techniques that save and restore the program states across power failures. ~\cite{gobieskiintermittent, gobieski2019intelligence, nirjon2018lifelong, bashima2019ondevice} propose lightweight and compressed deep neural network inference for on-device machine learning on batteryless systems. However, none of these works consider the timing constraints of the machine learning tasks. In a real-time setting, simply applying these two types of solutions in conjunction with an existing real-time scheduling algorithm does not quite solve the problem at hand, which is illustrated in Figure~\ref{fig:intermittent_deadmiss}. We consider two tasks, $\tau_1$ and $\tau_2$, released at time 0 and 25, respectively. Their deadlines are 45 and 56, and both have an execution time of 28. In Figure~\ref{fig:intermittent_deadmiss}(a), we observe that under the earliest deadline first (EDF) scheduling, both tasks meet the deadlines when the power is uninterrupted. But when power is intermittent, Figure~\ref{fig:intermittent_deadmiss}(b) shows that task $\tau_2$ misses its deadline.

\parlabel{Observations. } The goal of this paper is to overcome the aforementioned challenges. Towards this end, we study the energy harvesting pattern and the accuracy-execution trade-off of compressed deep neural networks (DNNs) that are executable on small systems~\cite{gobieski2019intelligence}. From these studies, we make two observations: 

$\bullet$ First, energy generated by a harvester is \emph{bursty}, and therefore, its energy harvesting pattern can be modeled using a stochastic framework over a short duration. Here, burstiness indicates that energy generation is maintained during a short period. 

$\bullet$ Second, since deeper layers of a DNN extract fine-grained and more detailed features of the input, for a given accuracy, the amount of DNN computation required for an input data is dependent on the quality of data itself. 

\parlabel{The \Sys~Approach. } By exploiting these above two observations, we design an \emph{imprecise computing}~\cite{shih1992line, liu1991algorithms}, online scheduling algorithm that considers both the intermittent nature of the power supply and the accuracy-execution trade-off of the DNN model. This design allows us to increase both accuracy and timeliness of DNN execution in intermittent systems. For example, in Figure~\ref{fig:intermittent_deadmiss}(c), when a full execution of the task is not necessary, i.e., tasks are \emph{imprecise}, both tasks can meet the deadline.

%Deep neural network (DNN) refers to neural networks with more than three layers including input and output layers. The DNNs considered in this paper, are small and compressed networks with at most 64,000 fixed-point parameters.}     

Our work complements previous work on time-keeping~\cite{rahmati2012tardis, hester2016persistent} and intermittent execution of non-real-time tasks~\cite{gobieskiintermittent, gobieski2019intelligence, ransford2012mementos, mirhoseini2013automated,balsamo2015hibernus, balsamo2016hibernus++,maeng2017alpaca, colin2016chain, maeng2018adaptive}. We extend the state-of-the-art intermittent DNN execution framework, called SONIC ~\cite{gobieski2019intelligence}, by implementing a runtime framework that supports intelligent scheduling of real-time DNN tasks. To enable time-aware adaptive deep learning in intermittently powered systems, we make three key technical contributions:   

%, and considers that time-keeping can be achieved with~\cite{rahmati2012tardis, hester2016persistent}. Both time-keeping and intermittent execution in batteryless system is out of the scope of this paper. Like ~\cite{yildirim2018ink,hester2017timely} this paper keeps time with a real-time clock for the ease of implementation as described in Section~\ref{sec:setup}.

%\bnote{Unlike battery-powered systems where usability is tied to battery-life, a batteryless system, which lasts forever, loses its worth when the code dies. Death of the code refers to outdated parameters which is unable to model the current environment. Therefore, evolving with the environment in such a system is necessary. The computational and memory constraints of batteryless systems and the unavailability of labeled data obstruct complicated adaptation techniques (e.g., back propagation). To address this challenge, we consider a semi-supervised learning (semi-supervised K-means) that updates previously trained model with the incoming data stream. }


$\bullet$ First, we devise a metric, i.e., the $\eta$-factor, to model the predictability of an energy harvester's source. This metric indicates the probability of a harvester maintaining its current state over a short period in time. The introduction of $\eta$-factor abstracts away the unpredictability of an energy harvesting source and enables development of scheduling algorithms that can make informed decisions based on predicted energy over a short period in the future. 

$\bullet$ Second, we redesign the DNN construction and training algorithms to enable early termination of a DNN task based on the quality of the input data. To enable this, we propose a \emph{layer-aware loss function} to improve the accuracy of a clustering-based, semi-supervised inference algorithm that uses DNN layer outputs as the representation of the input examples.

$\bullet$ Third, we propose an imprecise computing-based, online, scheduling algorithm that improves the timeliness of DNN inference tasks running on energy harvesting systems. This algorithm leverages the $\eta$-factor of the energy source, along with the properties of the input data to adapt the execution of real-time DNN tasks. 

\parlabel{Main Results. } We implement the system on a TI MSP430FR5994 and evaluate its performance using two datasets: MNIST~\cite{lecun1998mnist} and ESC-10~\cite{piczak2015environmental}, as well as in real-world acoustic event detection experiments. We achieve 9.45\% - 3.19\% higher accuracy than the baseline DNN algorithms for MCUs and achieve 14\% reduction in execution time. The proposed scheduling algorithm successfully schedules 33\%-12\% more tasks than traditional scheduling algorithms. 

%non-real-time systems. 


% \rnote{mention impmentaion and application and results to complete the intro.,}

%as well as the utility-execution trade-off where the utility can be application dependent. 

%$\bullet$ We introduce a combination of pre-trained DNN model and semi-supervised learning algorithm. We also utilize the dependency of required network depth on data and propose early termination of a deep neural network. We also propose a light-weight utility for this system and tie our scheduling algorithm with DNN models.

%$\bullet$ To maximize the early termination accuracy, we propose a layer-aware loss function which considers loss across each layer of the network. We also propose an approximate adaptation of the deeper layers of networks for the data which terminates the network early. To our knowledge, we are the first to consider layer-aware loss function. 


==> Tamzeed_ArXIV%20(Copy)/02_motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\parlabel{On-Device Learning.} Resource-constrained sensing and inference systems enjoy the benefit of machine learning in two ways -- either they send raw or partially processed sensor readings to a remote server for inference, or they do everything on device. While most low-power IoT systems largely use the former method~\cite{de2018paws, shao2018marble, choudhurysuper, chandrasekaran2016seus, xia2019improving}, in recent years, we see an increasing trend in on-device machine learning on embedded systems ~\cite{google_federated_learning, OVIC, ravi2017projectionnet, google_projectionnet}. This can partly be attributed to the limitations of server-based systems -- which are generally energy-demanding, slow, less reliable, and privacy invasive. The other reason behind this increasing trend is the advancement in hardware and software technologies~\cite{qualcommOnDevice, qualcommOnDeviceSlide,EdgeTPU,appleAI, QualcommNPS,google_federated_learning,appleAI} that are enabling powerful machine learning features into small and low-power systems.     


%Artificial Intelligence is the ability to automate intellectual tasks usually performed by humans~\cite{chollet2017deep}. Similar to a human, a system learns from experience to exhibit intellect where experience comes as large datasets. Most machine learning operations execute in the cloud/server and have several drawbacks, e.g., latency, privacy, and reliability~\cite{nirjon2018lifelong, bashima2019ondevice}.

%On-device learning addresses these short-comings with the need for more optimized operation. It achieves \emph{lower latency} than cloud-based solutions by saving the round-trip to the server. It increases \emph{reliability} as communication with a server is still tricky in several parts of the world due to the bad or no network signal. Besides, limited communication \emph{saves energy} by reducing the usage of power hungry network modules. Low-power networks (e.g., backscatter) has lower data-rate, which results in the prolonged transmission period. On-device learning saves scarce and limited \emph{network bandwidth} resource. Finally, on-device learning \emph{preserves privacy} and thus avoids security hazards. For example, last year sensitive information of 31 million Android users was leaked due to the hacking of a popular keyboard~\cite{keyboardBreach}. To enable on-device learning in current smartphones, special purpose hardware~\cite{qualcommOnDevice, qualcommOnDeviceSlide,EdgeTPU,appleAI} and software~\cite{QualcommNPS,google_federated_learning,appleAI} have been introduced.


%Today's low power computing devices commonly offload the majority of computations~\cite{de2018paws, shao2018marble, choudhurysuper, chandrasekaran2016seus, xia2019improving}. With the exponential growth of the internet of things (IoT)~\cite{iotgrowth}, this design is causing stress on the limited bandwidth. The power consumption for communication (23,000mJ) costs 360$\times$ higher than local inference (198mJ) on a MNIST~\cite{lecun1998mnist} input~\cite{gobieski2019intelligence}. Therefore sending the result rather than the raw data is more efficient~\cite{gobieski2019intelligence, islam2018glimpse}. 

\parlabel{Learning on Batteryless Systems.} Previous works have addressed the need for computation including inference of deep neural network on energy harvested devices ~\cite{gobieskiintermittent, gobieski2019intelligence, ransford2012mementos, colin2016chain, maeng2017alpaca}. However, the necessity of updating the models and timeliness is yet to be explored. As no two scenarios or people are genuinely similar, the need to have a customized model is inevitable. Besides, the models of a forever executing batteryless system become outdated with time. To address the same issue, on-device learning (including training) is introduced~\cite{google_federated_learning}, which improves accuracy and provides a personalized system that ensures privacy, lower latency, and reliability.
Moreover, most batteryless systems are deployed at unreachable places (e.g., deep jungles, calamity-prone areas) where the traditional power source is absent and replacing a battery is unrealistic. It is also not feasible to collect data and update the model on-site in such cases. With time, such devices observe a massive amount of information which is likely to be wasted due to the inefficiency of data transmission. To fully utilize the potential of batteryless devices, training the models is needed. However, the small footprint of batteryless devices works against the extra computational and energy load enforced by training models and the unavailability of labeled data obstruct complicated adaptation techniques (e.g., back propagation). Light-weight semi-supervised learning algorithms needs to be considered to evolve previously trained models with the incoming data stream. 

\parlabel{Deep Inference. }
Due to its non-linear and parametric model, Deep Neural Network (DNN) exhibits better performance than other traditional models, e.g., Support Vector Machine  (SVM). Here, DNN refers to neural networks with more than one hidden layer. Sending the inference result instead of the raw data is more energy efficient and high accuracy is essential to maintain the system's usability. ~\cite{gobieski2019intelligence} shows that inference accuracy determines the end-to-end system performance. 

\parlabel{Time-Aware Inference. }
The higher accuracy of DNN is achieved using more rigorous computations that result in higher execution and response time.  For a usable system, the response time needs to be tolerable~\cite{zhu2012deos, moser2006lazy, moser2007real}. High delay of a system hampers its usability despite accuracy. Though some works have addressed real-time requirements for batteryless sensor nodes, the accuracy of the system itself has not been considered yet. Precision and responsiveness both are crucial for the usability of a learning system and are contradictory to each other. The goal is to find the sweet spot where the highest accuracy can be achieved with acceptable delay. Such a time-aware application includes event detection and  monitoring wildlife, natural calamities, wearable, implantable, infrastructure, and buildings. To illustrate, an acoustic event detector at home enables home activating monitoring, intruder detection, and elderly monitoring. Similarly, gym-equipment and shared bike usage can be monitored using kinetic energy harvesting systems which can inform the authority about the required maintenance of the system. 

==> Tamzeed_ArXIV%20(Copy)/03_pre_study.tex <==
\section{System Modeling}
\label{sec:model}
In this section, we study and model the energy harvesting pattern of energy harvesters and the accuracy-execution trade-off of deep neural networks. 

\subsection{Modeling Energy Harvesting Pattern}
\label{sec:energy_study}

\parlabel{Energy Events.} 
Transiently powered systems operate intermittently because energy is not always available to harvest and, even when energy is available, buffering sufficient energy to perform adequate work takes time. In most cases, the pattern of this intermittency is stochastic and thus modeling this patter is not straight forward. To schedule the workload of an intermittently operating system at run-time, we decide whether to start execution of a task or not at a time instant. This decision heavily depends on the availability of harvestable energy. To model the availability of energy, we define \emph{energy event} which expresses the availability of sufficient energy during a period. Energy event represents a successful generation of at least K Joules of energy in total during T time slot. Here, K and T are system dependent. In order to better understand the property of energy events, we observe the phenomenons causing energy events. For example, in a piezo-electric harvester, taking a minimal number of steps that generates at least K Joule of energy during T time slot is considered equivalent to the occurrence of an energy event. Similarly, we consider a minimal number of packet transmissions per time slot and minimum intensity of solar per time slot as energy events for RF and solar harvesters, respectively.

\parlabel{Properties of Energy Events.}
We study energy event patterns of three commonly used harvesters -- piezo-electric harvester, solar harvester, and RF harvester from datasets ~\cite{meyer2016daily, ipdataset}. These datasets contain the number of steps taken during every 5-minute time-slot for 61 days, harvested solar energy measurements for three days and outbound packet transmission rate by an RF transmitter for 30 days. This study reveals two interesting observation about the pattern of energy events -- (1) energy events occur in bursts where burstiness is the intermittent increases and decreases in activity or frequency of an event~\cite{akbarpour2018diffusion}, (2) a probabilistic relation exists among the consecutive energy events during a short period. In other words, the occurrence of an energy event increases the probability of the next energy event during a short period. To illustrate, when a person starts walking, the probability of continuing the walk is high within the first few time slots and it decreases with time. Likewise, when a person is sitting, the probability of remain seated is high immediately, but decreases after a while. 

\parlabel{Conditional Energy Event. }
We define \emph{conditional energy event (CEE)} that represents the conditional probability of an energy event occurrence based on the occurrence/absence of previous consecutive energy events. CEE(N) is the probability that an energy event will occur given immediately preceding N consecutive energy events occurred (for $N >0$) or not occurred (for $N < 0$). The following equation expresses CEE.
\begin{equation}
\resizebox{0.43 \textwidth}{!}{
    $CEE(N) = 
        \begin{cases}
        $p$($occurrence $|$ N consecutive occurrence$),& $if $ N > 0 \\
        $p$($occurrence $|$ N consecutive non-occurrence$) ,& $if $ N < 0
        \end{cases}$
}
\end{equation}
To illustrate CEE(10) = 90\%  implies that the next energy event will occur with 90\% probability if 10 immediately preceding consecutive energy event occurred. Similarly, CEE(-15) = 5\% indicates the probability of an energy event at the current time slot is 5\%, given that there were no energy events in the last 15 slots.)
\begin{figure}[!htb]
    \centering
    \vspace{-.2in}
    \subfloat[KW=0, \Factor=1]{\includegraphics[width=.24\textwidth]{plot/Ideal_CEE.pdf}}
    \subfloat[KW=0.17, \Factor=0.65]{\includegraphics[width=.24\textwidth]{plot/step_CEE_1.pdf}}
    
    \subfloat[KW=0.06, \Factor=0.84]{\includegraphics[width=.24\textwidth]{plot/solar_CEE_1.pdf}}
    \subfloat[KW=0.11, \Factor=0.76]{\includegraphics[width=.24\textwidth]{plot/RF_CEE_1.pdf}}
    \caption{(a)CEE for persistent power source. (b) CEE for piezo-electric harvester. (c) CEE for solar harvester. (d) CEE for RF harvester. We use N=20 for calculating KW and \Factor. 
    }
    \label{fig:assumption_proof}
\end{figure}

The CEE of a system powered by a persistently power supply or an ideal harvester that has no intermittence looks like Figure ~\ref{fig:assumption_proof}(a). Figure ~\ref{fig:assumption_proof}(b-d) shows the CEE of three energy harvested systems. From these figures, we observe that for a small value of N these systems demonstrate similarity with the ideal correlative harvester. We measure the similarity of CEE of a harvested system with persistent powered or ideal harvested system using Kantorovich-Wasserstein (KW) distance~\cite{ramdas2017wasserstein}. Through out this paper, we use KW to express the Kantorovich-Wasserstein distance between the CEE a system (H) and the CEE of persistently powered system (P) as given in Equation~\ref{eq:kw}.  We also observe that for a large $|$N$|$ the CEE drops significantly because when the interval time between the first and current event increases their probabilistic relation decreases. For example, a person is walking for a long time has a high probability of stopping.
\begin{equation}
    KW(H, P) = \int_{-\infty}^{+\infty} |CDF(H) - CDF(P)|
\label{eq:kw}
\end{equation}

\parlabel{\Factor~Factor. }
To quantify the predictability of a harvester, we take inspiration from ~\cite{srinivasan2008beta} and define a predictability metric \Factor. Despite being informative, distance alone is not sufficient to measure predictability. Because distance does not address the imbalance between the number of elements in CEE with positive and negative N values. To address this, we quantify \Factor~ as the distance of the harvester (H) from a persistently powered system compared to the distance of the random harvester from a persistently powered system with same energy event rate. Random harvester (R) refers to harvesters where energy events are completely independent. \Factor~ is expressed as follows. 
\begin{equation}
    \eta = \frac{KW(R, P) - KW(H, P)}{KW(R, P)}
\end{equation} 

\Factor~$=1$ indicates that the power is persistent, while \Factor~$=0$ indicates energy events are totally random. This metric is also depends on the number of consecutive energy events. As CEE(N) is close to zero for high $|$N$|$, we consider small $|$N$|$ throughout the paper.
Figure~\ref{fig:assumption_proof}(b-d) shows the KW and \Factor~ where $|$N$|$ is 20. 

\Factor~ not only varies across different harvesters but also changes for a specific harvester. For transiently powered devices this change over time depends on different parameters, e.g., change of human weight, change of seasons or locations, the distance between RF transmitter and receiver. However, due to the infrequency of these changes, they can be ignored.



\subsection{Modeling Deep Neural Network}
\label{sec:study_dnn}
In order to execute machine learning tasks (e.g., deep neural network (DNN) inference with convolution and fully connected layers) in a resource-constrained batteryless system, we need to minimize memory and computation costs. To achieve this goal, we study several attributes that are unique to deep learning processes. 

\parlabel{Significance of Depth.} DNN have layered structures where the input of the first layer is from an external source, e.g., sensors. The output of a layer is fed as the input of the next layer, and it goes on until the end of the network. The total number of layers in a DNN is called \emph{depth}. A shallow neural network, e.g. first perceptrons are composed of one input layer, at most one hidden layer and one output layer. A neural network having more than three layers (including input and output) qualifies as "deep" neural network. Increased number of layers and neurons both contribute to more complicated calculation resulting in higher accuracy~\cite{he2016deep}. However, a shallow network requires width exponential to that of a deeper network to achieve similar accuracy.  Therefore, the performance of a neural network depends on not only the number of parameters but also depth. For example, VGGNet has 16 layers with ~140M parameters, while ResNet beats it with 152 layers but only ~2M parameters. 
\begin{figure}[!htb]
    \centering
    \vspace{-0.19in}
    \includegraphics[width=0.45\textwidth]{fig/face5.pdf}
    \vspace{-0.19in}
    \caption{Example of deep learning learns layers of features.}
    \vspace{-0.16in}
    \label{fig:depth_example}
\end{figure}

The depth of a DNN is significant because at each layer nodes train on a distinct set of features based on the output of the previous layer. The complexity and abstraction of features increase with the depth of layers, and it is known as the feature hierarchy. Deep learning can extract features from data without human intervention. This automatic feature extraction is known as representation learning. 
To understand the effect of the depth of a DNN, let us consider a face detector in Figure~\ref{fig:depth_example}(a). The first layer of this deep learning based face detector learns basic features, e.g., edges. In the next layer, a collection of edges, e.g., nose, is learned.  A deeper layer learns a higher level feature, e.g., face abstraction.
\begin{figure}[!htb]
    \centering
    \vspace{-0.25in}
    \subfloat{\includegraphics[width=.4\textwidth]{plot/layer_class.pdf}}
    \vspace{-0.22in}
    \caption{Hard data requires complex representation to achieve similar accuracy.}
    \label{fig:exit_motivation1}
\end{figure}
\vspace{-0.22in}

\parlabel{Required Depth.} To decrease the execution time we observe the fact that depth is highly \emph{data-dependent}~\cite{bolukbasi2017adaptive}. If target classes are profoundly distinctive, then simple features can be used to distinguish them. For example, in Figure~\ref{fig:exit_motivation1}, audio of cat and water (easy data) are very distinguishable; thus a single layer CNN achieves 93\% classification accuracy. On the other hand, similar classes, e.g., train and helicopter (hard data) needs more complex representations to be distinct and thus require five layers of CNN to achieve 81\% accuracy. \emph{Representation learning} uses deep neural network to extract features from raw data. By executing only necessary layers based on the complexity of data we can achieve similar accuracy with decreased execution time. We consider execution of each data sample as a task and introduce the requirement of depth as a imprecise task model~\cite{shih1992line, liu1991algorithms, canon2018scheduling}. Each imprecise task consists of two portions -- mandatory and optional. Mandatory portion of a task is necessary to achieve required accuracy while executing optional portions further improves the performance. We consider the required depth for a data sample as mandatory portion and rest as optional.

\parlabel{DNNs for Ultra-Low-Power Systems.}
Fitting neural networks in resource-constrained energy harvesting systems is a challenge especially due to limited memory capacity. Most commonly used processors in existing intermittent systems are TI MSP430 low-power microcontrollers~\cite{colin2018reconfigurable, hester2016amulet, gobieski2019intelligence,hester2015tragedy,hester2017flicker} that include 1-4KB of SRAM and 32-256KB of FRAM. Therefore, only small compressed networks are suitable for these systems. Compressed networks mentioned in Table~\ref{tab:network} and previous work~\cite{gobieski2019intelligence} have 48,136-10,411 parameters. For 16-bit fixed point data type these parameter requires 96.3-20KB of memory. On the other hand, same networks require 943.66-180KB of memory without compression. Such networks can be executed in batteryless systems only after compression. However, larger networks  e.g., Resnet (image) and EnvNet (audio) requires 5MB and 94MB of memory which is not suitable for small memory footprint devices even after compression.

We execute MNIST(compressed) in TI MSP430 to estimate the size of code and other variables in the FRAM. We observed that instructions and other parameters (including a buffer to perform matrix operations) require around 128KB of memory. Though the increasing number of parameters increases the buffer size, for simplicity we ignore it. The remaining memory can be used for storing approximately 64,000 16 bit fixed point parameters. A deep neural network that requires less than 64,000 parameters can execute in a microcontroller having 256KB of FRAM. The number of hidden layers and the number of neurons at each layer depend on the number of input and output~\cite{heaton2011programming}. Therefore, very large dataset e.g., Imagenet is not suitable for such systems. These conditions are sufficient for executing 4-6 layer networks depending on the network configuration~\cite{gobieski2019intelligence}.


% HAR = 14,754 -- 524,616 
% OkG = 48,136 -- 330,896
% MNIST = 13,645 -- 475,500
% ESC-10 = 10,411 -- 65,936


%  An MSP430 with 256 KB of memory, for 28$\times$28 input and 10 outputs can support either -- (1) 4 fully connected(FC) hidden layers having an average of 64 neurons at each layer,  or (2) 2 convolution hidden layers where average filter size is 5$\times$5, and number of filters are 24 on average followed by 2 fully connected hidden layers having an average 64 neurons at each layer. }

This paper considers two networks summarized in Table~\ref{tab:network}. MNIST~\cite{lecun1998mnist} represents the image-based application, and ESC-10~\cite{piczak2015dataset} represents audio applications. We use two known techniques -- rank decomposition or separation~\cite{bhattacharya2016sparsification, chollet2017xception, xue2013restructuring, de2000multilinear, de2000best, tucker1966some} and pruning~\cite{han2015deep, nabhan1994toward} to compress each layer of the networks. Note that, our semi-supervised models avoid the last layers for inference.

% \rnote{Add a table comparing the traditional DNN's size and accuracy with compressed DNN's size and accuracy.}

\begin{table}[!thb]
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}cccc@{}}
\toprule
Dataset                & Layer & \begin{tabular}[c]{@{}c@{}}Uncompressed\\ Size\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Compressed\\ Size\end{tabular} \\ \midrule
\multirow{4}{*}{MNIST} & Convolution  & 20$\times$1$\times$5$\times$5                                                                                                               & 3$\times$1D Convolution                                                 \\ 
                       & Convolution  & 100$\times$20$\times$5$\times$5                                                                                                     & 1253                                                      \\ 
                       & Fully Connected    & 200$\times$1600                                                                                                     & 5456                                                      \\ 
                       & Fully Connected    & 500$\times$200                                                                                                       & 1892                                                      \\
                       & Fully Connected    & 10$\times$500                                                                                                     & --                                                      \\
                       \midrule
\multirow{4}{*}{ESC-10} & Convolution  & 16$\times$1$\times$5$\times$5                                                                                                            & 3$\times$1D Conv                                                 \\ 
                       & Convolution  & 32$\times$16$\times$5$\times$5                                                                                                     & 1280                                                      \\ 
                       & Convolution    & 64$\times$32$\times$5$\times$5                                                                                                 & 5068                                                      \\ 
                       & Fully Connected    & 96$\times$256                                                                                                      & 2703                                                      \\
                       & Fully Connected    & 10$\times$96                                                                                                  & --                                                      \\ \bottomrule
\end{tabular}
}
\caption{Networks considered in this paper.}
\vspace{-.3in}
\label{tab:network}
\end{table}

==> Tamzeed_ArXIV%20(Copy)/04_overview.tex <==
\section{\Sys~System Design}
\label{sec:overview}

\Sys~is a system architecture that executes semi-supervised deep learning with timing constraints in an intermittently powered system. It uses a deep neural network to extract complex features from data samples, where the deep neural network is pre-trained on a high-end device. \Sys~adapts to new unlabeled incoming data by using semi-supervised models, e.g., seed-based k-means~\cite{basu2002semi}. In seed-based k-means, initial centroids are defined from labeled data in training phase and at runtime the unlabel data update these centroids. \Sys~ relies on imprecise computing to maximize the number of samples meeting timing constraints in a batteryless platform. 

\Sys~aims to achieve three goals simultaneously -- (1) minimize classification error, (2) maximize the number of samples meeting time constraints, and (3) minimize energy waste. \Sys~addresses this by terminating the deep feature extraction network early when necessary and scheduling the samples with a special online scheduling algorithm for batteryless system that considers time, classification error and availability of energy simultaneously. 
\begin{figure}[!thb]
    \centering
    \vspace{-.5em}
    \includegraphics[width=.48\textwidth]{fig/flow_chart.pdf}
    \caption{\Sys~system architecture.}
    \vspace{-.2in}
    \label{fig:sys}
\end{figure}

\subsection{System Components}
\Sys~consists of five major components -- task generator, energy manager, agile DNN model, scheduler and adaptive models. 

$\bullet$ \textit{Task Generator. } 
\Sys~ gathers data from sensors (e.g. microphone, camera) and considers each data sample as a task. A task includes inference of agile DNN model and semi-supervised learning using adaptive model with adaptation for a data sample. To sense, it takes advantage of the analog to digital converter (ADC) and direct memory access (DMA) which writes sensor data to non-volatile memory without occupying the CPU. Each task (data sample) is pushed in the \emph{task queue} upon arrival. Each task contains two portions -- mandatory and optional. Only tasks in the task-queue are considered for execution and a task leaves the queue at the end of execution or at deadline.

$\bullet$ \textit{Energy Manager. }
The energy manager monitors the status of the energy storage (e.g. capacitor) and the energy harvesting rate. To measure the energy harvesting rate it relies on the system operating voltage and the voltage across the capacitor. These parameters are fed to the scheduler that determines whether to execute a task depending on these parameters. When energy is less than a minimum threshold ($E_{man}$), power failure occurs and nothing gets executed. We use SONIC~\cite{gobieski2019intelligence} to handle intermittent execution of tasks in this system.

$\bullet$ \textit{Agile DNN Model. }
Agile DNN model is a pre-trained feature extraction deep neural network. This deep neural network is trained with labeled data to extract the features from data for semi-supervised learning. This network is trained in a high-end device (e.g. server or GPU). We compress the trained network using rank decomposition and separation to fit in memory-constrained systems. To achieve better classification/ clustering accuracy in the earlier layer of the network, we propose a layer-aware loss function. The goal of this loss function is to extract distinctive features in the early stages of the network if possible. 

$\bullet$ \textit{Adaptive Models. } 
Adaptive models are a set of seed-based k-means models. These models classify the sensor data by using the features extracted from the Agile DNN models. To select only useful features and to decrease the model size, these models use features with highest Chi-squared stats. Adaptive models are incrementally updated to evolve with new data and adapt to dynamic environment. These models are utilized to determine confidence of accuracy (utility) to exit the DNN layers.

$\bullet$ \textit{Scheduler. }
The scheduler decides which task to process and partitions the task based on utility. This utility decides if the data sample requires further processing for more confident decision making. The scheduler uses this mandatory and optional segments, achieved confidence (utility) and energy status from the energy manager to decide which data sample to process. 
When a function of current energy of the system ($E_{curr}$) and \Factor~ is less than a threshold ($E_{opt}$), \Sys~ becomes conservative in its choice for execution and considers only mandatory portions of tasks. The high probability for low energy harvesting and possible power failure in the near future leads to this decision. Otherwise \Sys~ considers both mandatory and optional portions for execution. 



\begin{table}[!htb]
\begin{tabular}{@{}cccccc@{}}
\toprule
Task & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total\\ Layers\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mandatory\\ Layers\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Optional\\ Layers\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Release\\ Time\end{tabular} & Deadline \\ \midrule
$\tau_1$   & 4            & 1                & 3               & $t_1$           & $t_7$      \\
$\tau_2$    & 4            & 2                & 2               & $t_3$           & $t_9$      \\ \bottomrule

\end{tabular}
\caption{Task Description}
\label{tab:load_des}
\end{table}
\vspace{-.5in}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/example.pdf}
    \vspace{-.15in}
    \caption{Example of execution of \Sys.} 
    \vspace{-.25in}
    \label{fig:example}
\end{figure}
% \vspace{-.25in}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[!htb]
\begin{tabular}{cp{7cm}}
\toprule
Time                 & \multicolumn{1}{c}{Reason of the Action}                            \\ \midrule
$t_0$                  & No task in the system.                                              \\
$t_1$                  & $\tau_1^1$ (the only task) gets scheduled.                          \\
$t_2$                  & Since $E_{curr}$ < $E_{opt}$, optional $\tau_1^2$ is not scheduled.  \\
$t_3$                  & System prioritized $\tau_2^1$ over $\tau_1^2$ (See: Section 5).     \\
$t_4$                  & Since $E_{curr}$ < $E_{man}$ no task is scheduled.                  \\
$t_5$                  & System prioritized mandatory $\tau_2^2$ over optional $\tau_1^2$ .  \\
$t_6$                  & Only optional tasks remain and $E_{curr}$ >$E_{opt}$. The system prioritizes $\tau_1^2$ over $\tau_2^3$ due to its tighter deadline. \\
$t_7$                  & $\tau_2^3$ (the only task) gets scheduled.                          \\
$t_8$                  & $\tau_2^4$ (the only task) gets scheduled.                          \\ \bottomrule
\end{tabular}
\caption{Description of Figure~\ref{fig:example}}
\vspace{-.35in}
\label{tab:example_des}
\end{table}

\subsection{Example Execution}

We describe a simple workload consisting of real-time inference of two examples and demonstrate how \Sys~ executes the workload.
We describe the tasks in Table~\ref{tab:load_des}, where $\tau_i$ refers to task i. Figure~\ref{fig:example} demonstrates execution of task $\tau_1$ and $\tau_2$ along with energy status. Here, $\tau_i^j$ refers to $j^{th}$ layer of task i. Table~\ref{tab:example_des} provides the actions and reasons of the actions taken at each time step. Note that this example uses simplified assumptions (e.g. each layer requires single time unit to execute). The algorithm mentioned in Section 5 handles complexities (e.g., different execution time for each layer, multiple time units per layer, unknown mandatory layer number and, power-failure during layer execution).


==> Tamzeed_ArXIV%20(Copy)/05A_scheduler.tex <==
\section{Real-Time Scheduler}
\label{sec:algo_rt}

This section describes a generic real-time task scheduler for intermittently powered systems where each task executes as a chain of sequential subtasks that can be partitioned into mandatory and optional parts. We define the task model and task prioritization metric, and describe the scheduling algorithm.
\begin{figure}[!htb]
    \centering
    \vspace{-.12in}
    \includegraphics{fig/task_model.pdf}
    \vspace{-.7in}
    \caption{Task model for task $\tau_i$}
    \vspace{-.2in}
    \label{fig:task_model}
\end{figure}
\subsection{Task Model}

\parlabel{Define Task.}
We define each data sample entering \Sys~ as an imprecise task\footnote{According to the definitions in the real-time systems community, we should call each data sample a job. However, as each task has only one job in this system, we use task for each data sample for simplicity.}~\cite{shi2009hash, liu1991algorithms}, $\tau$. Data samples enter \Sys~ in a sporadic manner and multiple data samples/tasks can exist at any time point. The $i^{th}$ task is defined at $\tau_i$ where $D_i, e_i^j$ are the deadline of task $\tau_i$ and execution time of $j^{th}$ subtask of task $\tau_i$. The subtasks maintain a strict precedence order. An imprecise task $i$ is divided into two portions -- mandatory and optional. According to the definition of imprecise scheduling, successful execution of the mandatory portion within deadline is considered as schedulable~\cite{shi2009hash, liu1991algorithms}. Figure~\ref{fig:task_model} shows the task model of a task $\tau_i$. Each subtask consists of multiple units that execute atomically in an batteryless system that maintain the precedence order. A unit is similar to a task in task-based intermittent models mentioned in ~\cite{gobieski2019intelligence, gobieskiintermittent, colin2018termination, maeng2017alpaca} that needs to be restarted if there is a power down before it finishes. The scheduler of \Sys~ works with the subtasks and the units are maintained by SONIC~\cite{gobieski2019intelligence}.

\parlabel{Utility and Runtime Task Partitioning.}
The utility is an application specific parameter that indicates the system's goal. For example, in a control system, the completion of a correct control task results in maximum utility.  The utility of a task has a non-decreasing and non-linear correspondence with execution of each subtask. Mandatory portion of a task contains the subtasks which need to be executed to achieve a minimum utility. The rest of the subtasks belong to the optional portion. Unlike traditional imprecise computing ~\cite{shi2009hash, liu1991algorithms} where the number of subtasks in the mandatory portion is a pre-knowledge, the number of subtasks in the mandatory portion of \Sys~ is determined at run-time. We define such imprecise computing model as \textit{Dynamic Imprecise Computing}. 

\parlabel{Preemption and Task Switching.}
Each subtask performs a semantically integrated operation and cannot be preempted by the scheduler. However, the scheduler is allowed to preempt a task at the end of each subtask. This task-model follows the cooperative preemption task model at the subtask level~\cite{musliner1993circa}. Note that, a subtask can be preempted due to a power failure by the energy manager, but this is not related to the scheduler.

\subsection{Scheduling for Persistent Systems}
\label{sec:persistent}
Before we introduce the scheduling algorithm for an intermittently powered system, we discuss the scheduling algorithm for a persistently powered system. We consider that the CPU utilization~\cite{yuan2003energy} can be higher than one because in the intermittent system the power failure virtually blocks the CPU and increases the CPU utilization. As theoretically no scheduler can schedule all the tasks when the CPU utilization greater than one~\cite{yuan2003energy}, our goal is to maximize the number of tasks that can be scheduled.

In order to schedule dynamic imprecise tasks online, we propose a priority function ($\zeta$) which considers both the deadline and the utility of tasks. It also considers the effect of mandatory and optional portions which are crucial for imprecise scheduling. We define the priority function  as following:
\begin{equation}
    \zeta = (1 - \alpha (D_i - t_c)) + (1 - \beta U_i) + \gamma
\end{equation}
Here, $D_i$ and $U_i$ is the deadline and current utility of the task $\tau_i$ respectively. $t_c$ is the current time, and $\alpha$ and $\beta$ are the scaling factors. Finally, $\gamma$ is the \textit{imprecise factor} which defines if a task $\tau_i$ is currently executing a mandatory subtask or an optional one. The following equation expresses the imprecise factor ($\gamma$). 
\begin{equation}
    \gamma = 
    \begin{cases}
    1, & $mandatory portion $ (U_i < U_t)\\
    0, & $optional portion $ (U_i \geq U_t)
    \end{cases}
\end{equation}
Here, $U_t$ is the utility threshold that indicates the end of the mandatory portion. Imprecise factor guarantees the precedence of the mandatory portions before the optional portions. 

\begin{table}[!htb]
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{1}{|c|}{\multirow{2}{*}{Task}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Release \\ Time\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Total\\ Layers\end{tabular}}} & \multicolumn{2}{c|}{Task Set 1}                                                                                 & \multicolumn{2}{c}{Task Set 2}                                                             \\ \cmidrule(l){4-7} 
\multicolumn{1}{|c|}{}                      & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{c|}{}                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mandatory\\ Layers\end{tabular}} & \multicolumn{1}{c|}{Deadline} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mandatory\\ Layers\end{tabular}} & Deadline \\ \cmidrule(r){1-7}
$\tau_1$                                    & 0                                                                                             & 7                                                                                            & 2                                                                               & 45                            & 5                                                                               & 59       \\
$\tau_2$                                    & 25                                                                                            & 7                                                                                            & 4                                                                               & 56                            & 2                                                                               & 69       \\
$\tau_3$                                    & 50                                                                                            & 7                                                                                            & 3                                                                               & 93                            & 1                                                                               & 84       \\ \bottomrule
\end{tabular}
}
\caption{Task Description}
\vspace{-.1in}
\label{tab:load_des_algo}
\end{table}

\begin{figure}[!htb]
    \centering
    \includegraphics{fig/task_algo.pdf}
    \vspace{-.2in}
    \caption{Subtask execution time}
    \label{fig:exec_algo}
\end{figure}

\begin{figure}[!htb]
    \centering
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/EDF_example.pdf}}
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/Priority_example.pdf}}
    % \\
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/EDF_example2.pdf}}
    % \subfloat[]{\includegraphics[width=.24\textwidth]{fig/Priority_example2.pdf}}
    \includegraphics[]{fig/steady_example.pdf}
    \caption{(a) EDF fails to meet imprecise deadline. (b) Priority function meets imprecise deadline (c) EDF meets deadline with 80\% accuracy (d) Priority function meets deadline with 88.7\% accuracy.}
    \vspace{-.2in}
    \label{fig:schedule_example}
\end{figure}


\parlabel{Example.} 
We consider two sets of three tasks described in Table~\ref{tab:load_des_algo}. We consider accumulated accuracy as utility function. Each task has seven subtasks with execution time shown in Figure~\ref{fig:exec_algo}. 
Figure~\ref{fig:schedule_example}(a-b) shows the execution of tasks from set1 using EDF and priority based scheduling algorithm. In Figure~\ref{fig:schedule_example}(a), EDF fails to schedule the second task; however, priority based scheduler can schedule all three tasks in Figure~\ref{fig:schedule_example}(b). In Figure~\ref{fig:schedule_example}(c-d) we consider tasks from set2. Even though both EDF and priority function succeeds to schedule all the tasks, the accumulated accuracy of the EDF schedule (80\%) is higher than that of priority function schedule (88.7\%). 

\subsection{Scheduling for Intermittent System}
\label{sec:intermittent}
Scheduling in intermittently powered system is challenging due to the occurrence of power failure. In Section~\ref{sec:energy_study}, we introduce a probability of metric $\eta$ to measure predictability of an energy harvester. We use $\eta$ influenced priority function ($\zeta_I$) to schedule an intermittent system. 
\begin{equation}
    \zeta_I = 
    \begin{cases}
    (1 - \alpha (D_i - t_c)) + (1 - \beta U_i) + \gamma, &  \eta E_{curr} \geq E_{opt}\\
    \gamma( (1 - \alpha (D_i - t_c)) + (1 - \beta U_i)), &  \eta E_{curr} < E_{opt}
    \end{cases}
\end{equation}

Here, $E_{curr}$ is the current energy generation rate and $E_{opt}$ is the threshold energy generation rate. For an energy harvester with high \Factor, we leverage the predictability of energy generation and boost the utilization. When the $E_{curr}$ is high, we schedule both mandatory and optional subtasks, opportunely taking advantage of correlated energy event occurrence. Otherwise, the scheduler considers the high probability of energy event non-occurrence and schedules \textit{conservatively}. In this case we only schedule the mandatory subtasks. When \Factor~ is low, the predictability of energy generation is minimal and thus the system schedules conservatively unless the energy generation is very high.

$\zeta_I$ minimizes two types of energy waste in energy harvesting systems~\cite{buettner2011dewdrop}. The first one is running unnecessary tasks which we avoid when $\eta E_{curr} < E_{opt}$. The second wastage occurs by not running tasks when the harvester is getting continuous energy from the source to keep the capacitor charged. We handle this wastage by running optional subtasks when $\eta E_{curr} \geq E_{opt}$.


\subsection{ A Special Case: Scheduling Deterministic Intermittent System.}
\label{sec:intermittent_special}
Deterministic intermittent power source is a special type of intermittent source where energy harvesting pattern is known; e.g., RF harvester with periodic signal transmission. We propose a more simplistic approach for such systems. To schedule in such a system, we pretend this energy intermittence as a hypothetical periodic task (termed \textbf{energy task}) with the highest priority, and it is pre-scheduled offline. This assumption allows us to schedule the tasks with energy constraints taken in to account. Note that we assume that energy task can preempt the conditional-preemptive tasks at any time instance.
\begin{figure}[!htb]
    \centering
    \vspace{-.3in}
    \subfloat{\includegraphics[width=.45\textwidth]{fig/deterministic_EH_example.pdf}}
    \caption{(a) Missed a imprecise deadline of the job by not taking  the deterministic intermittence power into account. (b) Successfully scheduled two tasks by considering deterministic energy pattern as energy tasks.  }
    \vspace{-.1in}
    \label{fig:deterministic_EH_example}
\end{figure}

In Figure~\ref{fig:deterministic_EH_example}, we consider the first two tasks ($\tau_1$ and $\tau_2$) from Figure~\ref{fig:schedule_example}(a-b). We consider a periodic power source with a period of 8 time units. In Figure~\ref{fig:deterministic_EH_example}(a), the system does not consider the energy intermittence and misses the imprecise deadline for $\tau_2$. However, by considering the deterministic power source as energy tasks, the system schedules both tasks successfully.  


==> Tamzeed_ArXIV%20(Copy)/05B_agileDNN.tex <==
\section{Agile DNN and Model Adaptation}
In this section, we first describe the task model for semi-supervised learning with deep neural features. Then we describe the construction of agile DNN Model and approximate adaptation of adaptive models. 

\subsection{Agile DNN Task Model}

\parlabel{Define Task. }
We define each data sample entering \Sys~ as a task. The execution of one layer of agile DNN along with corresponding k-means model is defined as a subtask. In a subtask, \Sys~ extracts features of the data sample  from a specific layer of the agile DNN model, use those features to execute a semi-supervised k-means model and update the centroids. 
Figure~\ref{fig:dnn_flow} shows the task model of a task, $\tau_i$. $\tau_i^{k-1}$, $\tau_i^{k}$ and $\tau_i^{k+1}$ are the subtasks of $\tau_i$ that represent the $k-1$, $k$ and $k+1$ layers of the DNN with corresponding semi-supervised k-means clustering, respectively.
\begin{figure}[!htb]
    \centering
    \vspace{-.2in}
    \includegraphics{fig/dnn_flow.pdf}
    \vspace{-.15in}
    \caption{Flow of agile DNN task $\tau_i$ where $k-1$, $k$ and $k+1$ are different DNN layers (subtasks). $U_i^{k-1}$, $U_i^{k}$ and $U_i^{k+1}$ are the utility of $\tau_i$ after execution of $k-1$, $k$ and $k+1$ layers.}
    \vspace{-.18in}
    \label{fig:dnn_flow}
\end{figure}

\parlabel{Early Termination. }
For an energy constraint system, computing accuracy of unlabeled data is expensive. Popular model validation techniques including inter-intra cluster distance measure are computation heavy~\cite{bashima2019ondevice}. Therefore, instead of using accuracy as utility, we propose a light weight utility function. We define the difference between the distances of the data point from two nearest centroids as utility. 
\begin{equation}
    U_i = |d_a - d_b|
\end{equation}
Here, $d_a$ and $d_b$ are the distance of the data sample from the closest and the second closest centroid. The intuition behind this definition is that a data point at similar distances from two centroids is not confident enough regarding which cluster it belongs to. Therefore, more complex representation is required to determine the cluster with confidence. In Figure~\ref{fig:policy}, the distance between the data sample and two nearest centroids, $c_1$ and $c_3$ are $d_1$ and $d_3$ respectively. In Figure~\ref{fig:policy}(a) the difference between $d_1$ and $d_2$ are very small and thus the confidence of the data sample being a member of cluster 3 is low. Therefore more complex representation is needed to provide more confident result and further execution of agile DNN is needed. On the other hand, in Figure~\ref{fig:policy}(b) the difference between $d_1$ and $d_2$ are prominent and thus the data sample belongs to cluster 3 with high confidence. Thus further execution is not needed. 
\begin{figure}[!htb]
    \centering
    \vspace{-.12in}
    \includegraphics[width=0.35\textwidth]{fig/policy.pdf}
    \vspace{-.16in}
    \caption{Early Termination Policy}
    \vspace{-.16in}
    \label{fig:policy}
\end{figure}
Figure~\ref{fig:dnn_flow}, shows the early termination policy and the execution of subtasks. Here, $U_i^{k-1}$, $U_i^{k}$ and $U_i^{k+1}$ are the utility of $\tau_i$ after execution of $k-1$, $k$ and $k+1$ layers. $U_t$ is the threshold utility.


\subsection{Agile DNN Construction}
Our termination policy utilizes the output vector at each layer as learned representation rather than solving a joint optimization problem to perform both classification and clustering at the last layer~\cite{yang2016towards}. To ensure higher utility, we need to learn a representation which maximizes the distance between the representation of different classes and also minimizes the space between the representation of the same class. Contrastive loss function obtain this at the final ~\cite{islam2019soundsemantics}. However, easier samples can be distinguished with simpler representation from previous layers. Thus, we need to achieve distinctive representation in earlier layers.

\parlabel{Layer-Aware Loss Function. }
In order to accomplish this, we propose a layer-aware loss function inspired by the contrastive loss ~\cite{islam2019soundsemantics}. We use a convex combination of contrastive loss at each layer as a loss function that allows the system to have better distinguishable representation at the preceding layer. To ensure distinctive representations at earlier layers, early layers have more weights than the deeper layers. Therefore, easy samples get enough distinguishable representation at an earlier layer of a network mitigating their need to execute all the layers. Note that this loss function is used during the training of the agile DNN model in a traditional deep learning computing system.

The layer-aware loss function, $l$ is represented as follows. 
\begin{align}
\label{eqn:eqlabel}
\begin{split}
     l = \sum_{i=1}^{i=L} \alpha_i \times l_c(W_i, X_i^1, X_i^2, ... , X_i^N); & 
    ~where, \sum_{i=1}^{i=L} \alpha_i = 1
\end{split}
\end{align}
Here, $\alpha_i$ is the convex coefficient at layer $i$. $L$ and $N$ represent the total number of layers  and classes in the network respectively. $W_i$ is the learnable weights of the network at layer $i$. $X_i^1, X_i^2, ... , X_i^N$ are the vectors of each class at layer $i$. $l_c$ is the contrastive loss function and for two classes $X_i^1$ \& $X_i^2$ at layer $i$ it is defined as following. 
\begin{multline}
    l_c(W_i, X_i^1, X_i^2) = (1-Y) \dfrac{1}{2} G_{W_i}(X_i^1)−G_W(X_i^2) \\
    + Y \dfrac{1}{2} max(0, \Delta - G_{W_i}(X_i^1)−G_{W_i}(X_i^2))
\end{multline}
Here, $G_{W_i}(X_i^j)$ is the representation output of a member of class j; where j = 1, 2, .., N; at layer $i$. Coefficient $Y = 0$ if $X^1$ and $X^2$ belong to the same class and $Y = 1$ otherwise. The term $\Delta$ represents the distance margin that is maintained between the representation of different classes.





==> Tamzeed_ArXIV%20(Copy)/05C_adaptation.tex <==
\parlabel{Adaptation. }
Due to the prior termination in previous layers, a group of data fails to affect the clustering model with complex representation from deeper layers. It hinders the adaptation of cluster model with more complex features. One solution is to execute the non-linear calculation for each sample to get more complex representation and update the models.  This calculation includes matrix multiplications, addition, and a non-linear function; e.g., RELU activation. However, this execution contradicts to our goal of avoiding unnecessary computations for simple data. This dispute imposes an exciting challenge of updating the centroid of layer $L_{i+k}$ from the centroid of layer $L_i$ with light-weight calculation, where k = 1,2,3, ..., n. Such a challenge never occurred before as this is the first work combining model update with prior termination.

Let $C_j^i$ be a centroid of the clustering model at layer $i$ where $j$ is the number of members in the cluster where $C_{j}^i = \frac{\sum_{k=1}^j X_k^i}{j}$. For the next layer, $i+1$, the centroid is 
\begin{equation}
\label{eq:actual}
    C_{j}^{i+1} = \frac{\sum_{k=1}^j \sigma(W^{i+1} \times X_k^i)}{j}
\end{equation}
Here, $W^{i+1}$ and $B^{i+1}$ are weight and bias for layer $i+1$ respectively. $\sigma$ is the non-linear function; e.g., RELU. This formula requires at least $j$ multiplication. As multiplication is an expensive function, our goal is to avoid using them. Therefore, we approximate Equation~\ref{eq:actual} using the following equation and reduce the number of multiplication by $j-1$. 
\begin{equation}
\label{eq:actual1}
    C_{j}^{i+1} = \frac{\sigma(W^{i+1} \times \sum_{k=1}^j X_k^i)}{j}
\end{equation}
We assume that the non-linear function is RELU activation function. So, $\sigma(x) = max\{0, x\} = \frac{x + |x|}{2}$. After applying the RELU function, we observe that the error, $er$ is 
\begin{equation}
    er^{i+1} = \frac{\sum_{k=1}^j |W^{i+1} \times X_k^i| - |W^{i+1} \times \sum_{k=1}^j X_k^i|}{2j}
\end{equation}



==> Tamzeed_ArXIV%20(Copy)/07_evaluation.tex <==
\section{Evaluation}
\begin{figure}[!htb]
     \centering
     \subfloat{
         \includegraphics[width=0.16\textwidth]{fig/MCU.jpg}
     }
     \subfloat{
         \includegraphics[width=0.12\textwidth]{fig/Solar.jpg}
     }
     \subfloat{
         \includegraphics[width=0.16\textwidth]{fig/RF.jpg}
     }
     \vspace{-.1in}
    \caption{\Sys~ experimental setup}
    \label{fig:hardware}
    \vspace{-.18in}
\end{figure}
\subsection{Experimental Setup}
\label{sec:setup}
\parlabel{Computational Device. }
For evaluation we use TI-MSP430FR5994~\cite{msp430} at 16MHz. This micro-controller is equipped with 256KB of FRAM, 8KB of SRAM, 16-channel 12-bit ADC, 6-channel direct memory access (DMA) and a Low Energy Accelerator (LEA). It has an operating voltage range of 1.8V to 3.6V. To program this device we use the Linux distribution and GCC compiler with an ez-FET programmer. \Sys~ uses fixed point calculation and flip-flop buffers to enable DNN execution in MSP430\footnote{The implementation of \Sys~ is available on \href{https://github.com/zygarde-sensys/Zygarde.git}{https://github.com/zygarde-sensys/Zygarde.git}}. 

To train the agile DNN model mentioned in Table~\ref{tab:network} we use an Intel Core i7 PC with RTX2080 GPU. We train the network offline and compress it with rank decomposition or separation ~\cite{bhattacharya2016sparsification, chollet2017xception, xue2013restructuring, de2000multilinear, de2000best, tucker1966some} and pruning~\cite{han2015deep, nabhan1994toward}. We execute this compressed trained network for inference in our target device TI-MSP430FR5994.


\parlabel{Energy Harvester. }
We harvest energy from two ambient sources -- solar and RF. We use a flexible Ethylene Tetrafluoroethylene (ETFE) based solar panel~\cite{solar_panel} that outputs 6V at 1W. We use a LTC3105 step up DC/DC converter with a start up voltage of 250mV~\cite{ltc_3105} to charge the capacitor with the solar panel. A Powercast P2210B~\cite{power_cast} is used to harvest RF energy from  a 3W Power-caster transmitter~\cite{powercase_transmitter}, Figure~\ref{fig:hardware}. For all the experiments with intermittent power we use a 50mF capacitor. For persistently powered experiments we rely on the power supply from the ez-FET of the MSP430 launchpad.

\parlabel{Sensor Peripheral. }
For audio sensor, we use a Electret microphone~\cite{BOB} that draws 3.1mA current and has a start up time of 125ms. We utilize the built in ADC and internal clocks to read data from the microphone. To calculate the FFT we use the LEA and use DMA to write data to the FRAM without occupying the CPU. 

\parlabel{Time Keeping Peripheral. }
Like ~\cite{yildirim2018ink,hester2017timely}, we use a real-time clock, DS3132~\cite{timer} via I2C, for time keeping. This choice is made for the ease of implementations. Note that, we only use this clock during power up for syncing up and maintaining time with the internal clock of the MCU. This real-time clock is easily replaceable with SRAM and capacitor based time-keeping system during power off periods~\cite{rahmati2012tardis, hester2016persistent}. Note that both time-keeping and intermittent execution in batteryless system is out of the scope of this paper.

\parlabel{Libraries. }
We use MSP430 libraries provided by Texas Instrument. For maintaining intermittent execution \Sys~ uses SONIC~\cite{gobieski2019intelligence} and the dependant libraries (e.g. ALPACA~\cite{maeng2017alpaca}) of this project. For training the agile DNN model we use Google's Tensorflow~\cite{45381}. 

\parlabel{Datasets. }
To evaluate our algorithms we use two popular datasets MNIST~\cite{lecun1998mnist} and ESC-10~\cite{piczak2015dataset}. MNIST is a image based dataset which consists of $28 \times 28$ pixel images and 10 classes. ESC-10 consists environmental sounds of 10 classes. Each audio clip is 5s long and has a sampling rate of 44KHz. To accommodate this dataset with our resource constrained device, we take the middle 1s audio and down-sampled it to 8KHz.  

\parlabel{Controlled Energy Source. }
To evaluate the system with different \Factor, we perform controlled experiments with the energy sources. For RF, we vary the distance between the harvester and the transmitter from 1 feet to 5 feet. For solar, we simulate the sun with three dimmable bulbs with varying intensity (5.6 Klx - 35 Klx) as shown in Figure~\ref{fig:hardware}. Note that, for the real-life experiment we use outdoor scenarios and windowed rooms to get the sunlight.  


\subsection{Algorithm Evaluation}

\parlabel{Effect of Layer-Aware Loss Function and Early Termination. }
In this section, we evaluate our proposed layer-aware loss function, early termination and adaptation. We train all models with same hyper-parameters and only use the training dataset. While inference we rely on the testing dataset provided by MNIST and ESC-10 (we use fold 1 only) containing 10,000 and 80 samples respectively. Note that, layer-aware loss function and early termination are applicable for any system, not just intermittently powered ones. Therefore, we do not bring the energy harvesting aspect in this evaluation and perform the evaluation on a persistently powered system. We compare our layer-aware loss function (L) and layer-aware loss function with adaptation (AL) with cross-entropy loss (CE)~\cite{zhang2018generalized} and contrastive loss (C)~\cite{islam2019soundsemantics}. We also consider a network trained with cross-entropy loss which only exits in the last layer similar to the one shown in SONIC~\cite{gobieski2019intelligence}.

\begin{figure}[!htb]
    \centering
    \includegraphics{plot/Early_exit_mnist.pdf}
    \vspace{-.18in}
    \caption{Prior Termination Evaluation MNIST.}
    \label{fig:early_exit_mnist}
\end{figure}
\begin{figure}[!htb]
    \centering
    \includegraphics{plot/Early_exit_esc.pdf}
    \vspace{-.18in}
    \caption{Prior Termination Evaluation ESC-10.}
    \vspace{-.18in}
    \label{fig:early_exit_esc}
\end{figure}
For MNIST dataset in Figure~\ref{fig:early_exit_mnist}, we observe that for cross-entropy loss (CE) with early termination decreases the accuracy along with the execution time. However, with the layer-aware loss(L) we increase the accuracy by 9.45\% from cross-entropy loss (CE) and 3.19\% from contrastive loss (C) while keeping similar execution time. Layer-aware loss function with adaptation (AL) increases the accuracy by 1\% and allows more samples to terminate in the early layers. 

\begin{figure*}[!htb]
    \centering
    \includegraphics{plot/mnist_schedule.pdf}\vspace{-.2in}
    \vspace{-.15in}
    \caption{Realtime Scheduling for Systems with different ($\eta$) on MNIST test dataset.}
    \label{fig:schedule_mnist}
\end{figure*}
\begin{figure*}[!htb]
    \centering
    \includegraphics{plot/esc_schedule.pdf}
    \vspace{-.2in}
    \caption{Realtime Scheduling for Systems with different ($\eta$) on ESC-10 test dataset.}
    \label{fig:schedule_esc}
\end{figure*}

ESC-10 is a complex dataset where previous works achieves 73\% accuracy using models with three convolution layers, data augmentation and, 44KHz sampling rate~\cite{piczak2015environmental}. Our network takes downsampled audio data of 1s duration and achieves 70\% accuracy. 
In Figure~\ref{fig:early_exit_esc}, layer-aware loss function(L) achieves 76.25\% accuracy and decreases the execution time by 1.22 minutes. Note that, layer-aware loss function with approximation (AL) does not show any improvement over layer-aware loss in this scenario because all data samples of several classes exit the network in earlier layers minimizing the need of approximate adaptation for deeper layers. 



\parlabel{Performance of Real-Time Scheduler. }
In this section, we evaluate our proposed scheduling algorithm for dynamic imprecise tasks that is applicable to both persistently (Section~\ref{sec:persistent}) and intermittently (Section~\ref{sec:intermittent}) powered systems for different \Factor. We evaluate the system with two different CPU utilization. 

For MNIST dataset in Figure~\ref{fig:schedule_mnist}, we consider a CPU utilization$\geq1$. Thus even with persistent power we can not schedule all tasks. Without early termination the majority of samples could not be scheduled as they keep on waiting in the queue. But, with early exit 75\% of samples can be scheduled. We consider sporadic tasks with a period of 3 seconds and the deadline is twice the period. According to the definition of imprecise computing, we consider completion of mandatory portion as a successful scheduling~\cite{shih1992line}. For ESC-10 dataset in Figure~\ref{fig:schedule_esc}, we consider that CPU utilization$\leq1$, the period is 0.36 minute and the deadline is twice the period.

We compare our approach with earliest deadline first (EDF) algorithm and a variation of EDF that only executes the mandatory portion (EDF-M). We consider various \Factor~ and use three systems that persistently powered, solar powered and RF powered. We notice that in all the cases \Sys~ can successfully schedule higher number of tasks with higher accuracy. There are two major things to notice in Figure~\ref{fig:schedule_mnist} and Figure~\ref{fig:schedule_esc}.

$\bullet$ When \Factor~ is high \Sys~ increases the number of tasks with correct result by executing some of the optional portion. For a 100\% accurate utility function the performance of ~\Sys~ and EDF-M would be same. 

$\bullet$ For small \Factor~ the performance of \Sys~ and EDF-M is the same because it satisfies the second condition of Equation~6 which only executes mandatory portion. 

$\bullet$ The number of tasks that can be scheduled does not depend only on \Factor~ but also on the harvested energy.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics{plot/eta_runtime_solar.pdf}
%     \caption{Active Execution Time of Realtime Scheduling for systems with different $\eta$ with solar harvester.}
%     \label{fig:persistent_time}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{plot/real_solar.pdf}
    \vspace{-.2in}
    \caption{Real-life evaluation of \Sys~ with solar}
    % \vspace{-.2in}
    \label{fig:real-solar}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{plot/real_rf.pdf}
    \vspace{-.2in}
    \caption{Real-life evaluation of \Sys~ with RF}
    % \vspace{-.2in}
    \label{fig:real-rf}
\end{figure}

\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccllcl@{}}
\toprule
Scenario  & Energy Source & Source Power & Harvester Placement & Additional Cause      & Target Event & \multicolumn{1}{c}{Other Audios}          \\ \midrule
Street           & Solar         & 74 -- 80 Klx    & Pavement    & Vehicle on the closest lane & Car Honk     & Silence, Dog, Human Voice, Car            \\
Shaded Park           & Solar         & 1.8 -- 0.6 Klx    & Under Tree          & People, objects and cloud   & Dog Bark     & Silence, Car, Car Honk, Human Voice       \\
Staircase  & Solar         & 0.5 -- 0.3 Klx    & Edge of the Railing & People and cloud            & Human Voice  & Silence, Car, Car Honk, Dog Bark          \\
Nursery               & RF            & -.48 -- -1.66dB    & On Desk             & Change of distance                  & Baby Cries   & Silence, Human Voice, Washer, Printer     \\
Laundry               & RF            & -.48 -- -1.91dB      & On Counter          & Change of distance                  & Washer       & Silence, Human Voice, Baby Cries, Printer \\
Office                & RF            & -1.59 -- -1.91dB      & On Desk             & Change of distance                  & Printer      & Silence, Human Voice, Baby Cries, Printer \\ \bottomrule
\end{tabular}
}
\caption{Real-life evaluation setup}
\vspace{-.3in}
\label{tab:real_setup}
\end{table*}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics{plot/solar_eta_hi_schedule.pdf}
%     \caption{Realtime Scheduling for Solar Powered System ($\eta$=0.712). 7717 data samples (tasks) entered the system.}
%     \label{fig:persistent_system}
% \end{figure}

\subsection{Real-World Application Evaluation}
 
\parlabel{Experimental Setup.}
In this section, we evaluate your system in an uncontrolled environment. We present an acoustic event detector as the application. We choose six scenarios with seven acoustic events. In three of these scenarios we use a solar harvester and for the rest we use a RF harvester. Table~\ref{tab:real_setup} describes the different scenarios along with the target events. We rely on the natural events for hindrance in power generation for the solar harvested systems. For example in the \emph{street} scenario, the harvester with solar panel is kept on the edge of the pavement. The vehicles (cars, buses) passing through the nearest lane to the pavement is blocking the sun and thus introducing hindrance in energy generation. However, due to the lack of programmable RF harvester or proper setup to harvest from WiFi, we change the distance between RF harvester and transmitter. We use the same setup mentioned in Section~\ref{sec:setup} for the computation and sensing unit. Note that other sound sources were present in all scenarios and we included silence as an event in the classifier for training. 




% \begin{table}[]
% \begin{tabular}{@{}p{1cm}p{.6cm}p{1.3cm}p{1.5cm}p{1.3cm}p{1.5cm}@{}}
% \toprule
% Scenario  & Energy Source & Source \bnote{Power} & Harvester Placement & Hindrance Cause      & Target Event \\ \midrule
% Street           & Solar         & 74-80 Klx    & Pavement    & Vehicle & Car Honk     \\
% Park           & Solar         & 1.8-0.6 Klx    & Under Tree          & People   & Dog Bark     \\
% Staircase            & Solar         & .5-.3 Klx    & Railing & People            & \bnote{Voice}  \\
% Nursery               & RF            & 0.5 ft - 3 ft    & On Desk             & Distance                  & \bnote{Baby Cries}   \\
% Laundry               & RF            & 1 ft - 5 ft      & On Counter          & Distance                  & Washer       \\
% Office                & RF            & 2 ft - 5 ft      & On Desk             & Distance                  & Printer      \\ \bottomrule
% \end{tabular}
% \end{table}


\parlabel{Performance.}
In Figure~\ref{fig:real-solar} shows the voltage across the capacitor along with the operating voltage of the computational unit of the three scenarios where the system is powered by a solar harvester. Note that the voltage across the capacitor and operating voltage is used to measure energy generation rate. The system runs a DNN with a single convolution layer and two fully connected layers. The execution time varies between 1.7 s and 3 s depending on the early exit. Among the 30 events we experienced we have four incorrect detection. We experience three deadline misses even though the detection is accurate. We miss four samples due to intermittence as the system did not have enough energy to be turned on. 

Similar to Figure~\ref{fig:real-solar}, Figure~\ref{fig:real-rf} shows the result for scenarios with RF harvester. We notice two interesting facts with this experiment. The first one is that the MCU experience higher intermittence rate for RF harvester than solar harvester. However, the duration of power off is much higher in solar harvester specially when we do not have the direct sunlight.  



%  need to do as much as possible with msp430
% \begin{itemize}
%     \item In dataset accuracy and time with and without termination policy
%     \item Layer Aware Loss Function $\checkmark$
%     \item Approximate Representation Transformation vs no transformation vs all computation. Accuracy and time. 
%     \item With + Without the algorithm in both powered and powerless systems
%     \item Real-life performance accuracy and #deadline miss
% \end{itemize}
% \subsection{Layer-Aware Loss Function}
% We use audio dataset ESC-50 for evaluating the performance of layer-wise loss function. 
% \\
% In Figure~\ref{fig:cluster_data}, we randomly select classes and observe the number of layers needed for achieving at least 80\% accuracy for clustering. We notice that for various number of clusters, some class combination requires more layers than the previous. To illustrate, cat and toilet flush are very distinguishable sounds and can be clustered with 93\% accuracy using the representation learned from the first layer of the network. On the other hand, train and helicopter both having similarity in audio needs execution of 5 layers to achieve 81.25\% accuracy.
% % Accuracy with and without Layer Adaptation for different dataset (Lenet, Urban Sound 8K, ESC-10, Google Keyword Dataset). (same configuration)/ X-axis runtime, Y-axis accuracy, Shape for different Dataset, Colored chart for the data distribution. 

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.45\textwidth]{plot/layer_class.pdf}
%     \caption{Different combination of classes needs different number of layers to achieve at least 80\% accuracy \textbf{NUMBER OF CLUSTERS}}
%     \label{fig:cluster_data}
% \end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.45\textwidth]{plot/loss_compare.pdf}
%     \caption{Performance comparison of layer-aware loss function, contrastive loss function and regular loss function. \textbf{LAYER-AWARE LOSS}}
%     \label{fig:zygarde_loss}
% \end{figure}

% In Figure~\ref{fig:zygarde_loss}, we compare the performance of our proposed layer-aware loss function, contrastive loss function and regular loss function with Adam optimized commonly used in deep neural network. We train all three systems for same number of epoch and same dataset. As easy data we choose 10 classes from ESC-10 dataset consisting of sneezing, dog barking, clock ticking, crying baby, crowing rooster, rain, sea waves, fire crackling, helicopter and chainsaw. As hard data we choose two classes from each of the five categories of ESC-50 dataset. These classes are -- church bells, clock ticking, frog croaking, baby crying, crickets,  mouse clicking, siren, insects flying, sneezing and water pouring. We observe that for easy data using our layer-aware loss function the system needs to execute four layers to achieve at least 65\% accuracy where as using contrastive loss function and regular loss function it needs to execute five layers. In the scenario of hard data, we can achieve 65\% accuracy after executing six layers using layer-aware loss function. However, the other two loss functions failed to achieve 65\% accuracy even after executing all the six layers. They achieved 61.25\% and 56.25\% accuracy at the final layer using contrastive loss function and regular loss function, respectively. 



% \subsection{Early Exit Policy}
% We use the ESC-Audio dataset.

% \subsection{Representation Transform}
% X axis different layer of different dataset. Y axis error of the transformed data. 

% \subsection{Online Real-time Scheduler}
% In order to verify the usability of the real-time scheduler, we develop a simulated scenario. In this simulation, we have a periodic task with 50 periodic jobs with a representation learner of 10 layers. Each layer execution consists of the time needed for representation learning and clustering. We have a random energy simulator system to simulate the energy harvesting system. 

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=.45\textwidth]{plot/simulation_acc.pdf}
%     \caption{Simulation Accuracy }
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=.45\textwidth]{plot/simulation_en.pdf}
%     \caption{Simulation Energy}
%     \label{fig:my_label}
% \end{figure}


% \bnote{change beta in scheduling to compare quality of inference vs diversity of inference}

% create an simulation to stochasticity of energy harvester
% first half i sregular pattern and second half is irregular pattern
% real timeline over data.

% First audio data comes in and exdecute few layer and execute in hardware
% Early Exit
% Scheduling 
% do the real system first. 
 


==> Tamzeed_ArXIV%20(Copy)/0X_related.tex <==
\section{Related Work}
\label{sec:related}

\parlabel{Intermittent Computing. }
Intermittently powered systems experience frequent power failure that resets the software execution and results in repeated execution of the same code and inconsistency in non-volatile memory. Previous works address the progress and memory consistency using software check-pointing~\cite{ransford2012mementos, maeng2018adaptive, hicks2017clank, lucia2015simpler, van2016intermittent, van2016intermittent, jayakumar2014quickrecall, mirhoseini2013automated, bhatti2016efficient}, hardware interruption~\cite{balsamo2015hibernus, balsamo2016hibernus++, mirhoseini2013idetic}, atomic task based model~\cite{maeng2017alpaca, colin2016chain, colin2018termination} and, non-volatile processors(NVP)~\cite{ma2017incidental, ma2015architecture}. Recently ~\cite{gobieskiintermittent, gobieski2019intelligence} proposes a special software system for intermittent execution of deep neural inference combining task atomic task based model with loop continuation. \Sys~ relies on  ~\cite{gobieskiintermittent, gobieski2019intelligence} for intermittent computation of deep neural network.   

\parlabel{Timeliness of Batteryless Systems. }
Prior works on intermittent computing proposes runtime systems that increases the likelihood of a task completion by finding optimum voltage for task execution~\cite{buettner2011dewdrop}, adapting execution rate~\cite{sorber2007eon, dudani2002energy} and discarding stale data~\cite{hester2017timely}. However, none of these works consider the accuracy/utility of the running application or the real-time deadline-aware execution of tasks. 
Some works have addressed scheduling in wireless sensors~\cite{zhu2012deos, moser2006lazy, moser2007real} but none of them consider the higher computation load of intermittent computing systems. ~\cite{yildirim2018ink} proposes a reactive kernel that enables energy aware dynamic execution of multiple threads. Note that they do not consider deep neural tasks or utilize early termination of tasks for increasing schedulability. Unlike \Sys~ which schedules multiple incoming data samples,  ~\cite{yildirim2018ink} schedules kernel threads and can only have one data sample in the system at a time point. 
Other works focuses on maintaining time-keeping through power loss~\cite{rahmati2012tardis, hester2016persistent}. Our work is a complementary of these works and relies on these techniques for time keeping. 

\parlabel{Compression and Partial execution of DNN. }
Recent works have focused on reducing the cost of DNN inference by pruning and splitting models without compromising accuracy~\cite{han2015deep,nabhan1994toward, yao2017deepiot, yao2018rdeepsense, yao2018apdeepsense, yao2018fastdeepiot}. Other works have focused on reduction of floating point and weight precision~\cite{johnson2018rethinking, de2017understanding, han2016eie}, and factorization of computation~\cite{bhattacharya2016sparsification, chollet2017xception, nakkiran2015compressing,szegedy2017inception, szegedy2015going, szegedy2016rethinking, wang2017factorized} to reduce storage and computation cost. The proposed binary networks~\cite{courbariaux2015binaryconnect, hubara2016binarized,rastegari2016xnor, courbariaux2017binarynet} are not suitable for energy harvesting systems due to the higher number parameters needed by such systems~\cite{gobieski2019intelligence}. Even though these works are crucial for enabling DNN execution in batteryless system these can be enhanced by exploiting the fact that in real-life data are usually is a combination of easy examples and difficult examples and the easy examples do not need the full DNN inference~\cite{bolukbasi2017adaptive, figurnov2017spatially, leroux2017cascading}. Unlike prior works that require an additional classifier after each layer, \Sys~ depends on semi-supervised models to reduce computational overhead. ~\cite{bateni2018apnet, zhou2018s} proposes scheduling algorithm for deep neural network in GPU and does not consider the constraints introduced by embedded system and intermittent power supply. 

\parlabel{Modeling Energy Harvesting System. }
~\cite{san2018eh} analytically model the trade-off associated with backing up data to maximize forward propagation. Even though energy harvesting system for a specific energy source has been analyzed and modeled before~\cite{crovetto2014modeling, sharma2018modeling, jia2018modeling}, none of the prior works focus on modeling energy harvesting systems irrespective of energy source. 

\section{Discussion}
After execution an DNN layer, \Sys~ calculates the manhattan distance of the data sample from all $n$ centriods using top $k$ features, where $n$ is the number of clusters. This requires $n\times k$ subtractions, $n\times k$ comparison (to determine absolute value) and $n\times k$ addition. \Sys~ needs $n+1$ comparisons to find the minimum distance and $k$ additions, $k$ multiplications and $k$ divisions to update a centroid. In our implementation, the highest number of $n$ and $k$ are 10 and 50, respectively. The total computation needed after each layer is 10$\times$ smaller than the required multiplication and addition needed for the smallest network layer mentioned in Table~\ref{tab:network}.

\section{Conclusion}
In this paper we propose a generic metric \Factor~ that expresses the stability on an energy harvesting system. We also utilize the fact that real-life data samples are a combination of easy and hard samples and all samples do not require the same amount of computation to achieve similar performance. We propose early termination of deep neural network without compromising much accuracy. To decrease the accuracy loss due to early termination, we propose a layer-aware loss function and achieve 9.45\% - 3.19\% increase in accuracy and 14\% decrease in execution time. We then model such DNN tasks as imprecise tasks and propose a scheduling algorithm that considers time, energy condition, \Factor~ and performance of the system. We evaluate our system with state of the art scheduling algorithms and our algorithm schedules 33\%-12\% more tasks successfully.

==> Tamzeed_ArXIV%20(Copy)/tex/01_Abstract.tex <==

\begin{abstract}
The lack of adequate training data is one of the major hurdles in WiFi-based activity recognition systems. In this paper, we propose \Sys, which is a WiFi CSI-based device-free human gesture recognition system that recognizes \emph{named} gestures, i.e., activities and gestures that have a semantically meaningful name in English language, as opposed to arbitrary free-form gestures. Given a list of activities (only their names in English text), along with zero or more training examples (WiFi CSI values) per activity, \Sys is able to detect all activities at runtime. In other words, a subset of activities that \Sys detects do not require any training examples at all. This is achieved by leveraging prior knowledge of these activities from another domain, i.e., text. We show for the first time that by utilizing the state-of-the-art semantic representation of English words, which is learned from a massive dataset such as the Wikipedia (e.g., Google's word-to-vector~\cite{mikolov2013efficient}) and verb attributes learned from how a word is defined (e.g, American Heritage Dictionary), we can enhance the capability of WiFi-based named gesture recognition systems that lack adequate training examples per class. We propose a novel cross-domain knowledge transfer algorithm between radio frequency (RF) and text to lessen the burden on developers and end-users from the tedious task of data collection for all possible activities. To evaluate \Sys, we collect data from four volunteers for 20 activities in two environments. %We \rnote{sample 10 random activities at a time and} 
We show that \Sys achieves an accuracy of up to $90\%$ for two unseen activities and $61\%$ for up to six unseen activities.
\end{abstract}





% We show for the first time that by utilizing the state-of-the-art semantic representation of English words, which is learned from a massive dataset such as the Wikipedia (e.g., Google's word-to-vector~\cite{mikolov2013efficient}), we can enhance the capability of WiFi-based \gnote{named gesture recognition systems} that lack adequate training examples per class. \rnote{We propose a novel cross-domain knowledge transfer algorithm between radio frequency (RF) and text to lessen the burden on developers and end-users from the tedious task of data collection for all possible activities. To evaluate \Sys, we collect data from four volunteers for 10 activities and show that \Sys achieves an accuracy of up to $90\%$ with two unseen activity classes and an accuracy of $51\%$ with up to five unseen activity classes.}








==> Tamzeed_ArXIV%20(Copy)/tex/02_Introduction_local.tex <==

\section{Introduction}

\label{sec:intro}




The widespread adoption of WiFi in indoor spaces, and the accessibility of WiFi signal characteristics such as the signal strength (RSSI) and channel state information (CSI) in commodity WiFi chipsets, make WiFi an attractive technology for human activity monitoring. Alternate solutions that use wearables like smartwatches and activity trackers are becoming less attractive due to their usage adherence issue, and systems that use cameras to monitor home activities raise serious privacy concerns. WiFi sensing, on the other hand, is device-free, non-intrusive, and less privacy-invasive. Hence, in recent years, we have seen an increase in WiFi-based sensing and inference systems whose feasibility has been demonstrated in application scenarios such as home activity monitoring~\cite{wang2014eyes}, sleep monitoring~\cite{liu2014wi}, gesture-based smart device interaction~\cite{abdelnasser2015wigest, adib2013see}, and health vitals tracking~\cite{liu2016contactless}. 

 \begin{figure}[!thb]
	\centering
	\includegraphics[width = 0.45\textwidth]{images/intro.pdf}
	\caption{Unlike existing systems, \Sys is able to recognize \textit{run} in the testing phase, even though it did not see any training example of \textit{run} in the training phase. }
	\label{fig:intro}
\end{figure}



A vast majority of WiFi-based activity recognition systems employ either template matching algorithms or machine learning classifiers --- ranging from traditional classifiers like support vector machines~\cite{wang2015robust} to advanced deep convolutional neural networks~\cite{yue2018extracting}. These algorithms require a decent number of training examples for each class of activity in order for the system to accurately model them. Furthermore, the capability of these systems are fundamentally limited by the number of activity classes for which the system has been trained for. When these systems are presented with a completely new type of activity, there is no built-in mechanism to make an educated guess about the possible class label for that unseen example. 

Figure~\ref{fig:intro} illustrates this scenario. When a system is trained to recognize only \mytt{\{walk, drink\}}, but is presented with an example of an unseen activity, e.g., \mytt{run}, it is likely to detect the activity as either \mytt{walk} (based on the closest match) or it will determine that it is an unknown category (based on a distance threshold). At present, existing systems have no inherent mechanism to infer that the activity could be \mytt{run}, as these systems have no prior knowledge of how an activity called \mytt{run} might be.         

A na\"ive way to deal with the above problem is to train a system with examples of all possible activities that it may ever encounter. However, this is not feasible for several practical reasons. First, despite recent efforts in environment-invariant activity classification~\cite{jiang2018towards}, existing WiFi-based sensing systems are prone to environment changes \bnote{due to RF signals' dependency on surroundings for reflection, refraction and scattering.} Hence, it puts the burden on the end-users to provide the training data --- which is time-consuming, error-prone, and in general, an inconvenience. Second, even with environment-invariant techniques, due to the diversity of human activities, it is not feasible to build models for all possible activities for users of all demographics. This motivates us to devise a WiFi-based sensing system that recognizes activities and gestures without prior examples.

In this paper, we propose the first system, called the \emph{\Sys}, which can infer activities from WiFi data without requiring prior training examples for all of its activity classes. The principle behind \Sys is popularly known as the \emph{zero-shot learning}~\cite{lampert2014attribute,frome2013devise}, which is an active research topic in computer vision and image classification fields. \bnote{Recently, zero-shot learning has also been applied to general-purpose sound recognition problem~\cite{islam2019soundsemantics}. These techniques are not directly applicable to RF-based gesture recognition problems, since gestures require tracking sequential properties of the signal and external knowledge about the attributes that defines an activity.} To the best of our knowledge, we are the first to apply zero-shot learning in RF-based device-free activity recognition problem. The core idea of zero-shot learning is to exploit information or learned knowledge from other sources such as textual descriptions, rules, and logic. For example, to teach the concept of \mytt{run} to a system that has already learned to recognize \mytt{walk}, instead of training it with many examples of \mytt{run}, we can add a rule into the system, e.g., ``\mytt{run} is just like \mytt{walk} but it's 3 to 5 times faster.'' At runtime, the system will use this additional information to classify a \mytt{run} activity correctly. 

In \Sys, to embed such rules between \emph{seen} classes (i.e., explicitly trained) and \emph{unseen} classes (i.e., not explicitly trained) in an RF sensing system, we exploit attributes and context-aware representation of English words as the additional source of knowledge. Through an advanced RF-domain to text-domain projection algorithm, we blur the difference between an activity's RF signature and its corresponding English word/phrase by representing them in the same vector spaces, i.e., \emph{word embedding}~\cite{mikolov2013distributed} and \emph{word attribute}~\cite{zellers2017zero} spaces. We exploit the attributes and semantic relationship between English words as the background knowledge to classify an activity from WiFi that the system has never seen before. We combine these algorithmic steps to develop an advanced activity recognition system that we name---\Sys, as it can detect previously unseen \emph{fringe} activities beyond what it is trained for. 

% The intuition behind \Sys ... (also a little touch on the assumptions: activity has to have a name so that we can find a word in the text domain and there needs to be some linkage between seen and unseen actions for zero shot to work.)...

The intuition behind \Sys is that the WiFi signature of an activity correlates with the corresponding verb's semantic and attribute information. Like two similar activities perturb the WiFi signals similarly, when we describe these two activities in English sentences, we see a similar likeness between the sentences. We generalize this notion for an arbitrary number of activities represented in both RF and text domains, and strive to find a projection between the two representations from the RF domain to the text domain. By learning this projection, we gain the ability to find the corresponding English word from the RF representation of any arbitrary activity. 

%The problem of finding the map thus becomes the central to enable recognition of unseen activities by a WiFi sensing system.       

%As the signal reflection is dependent on body movements, activities with similar movements have correlation in  RF domain. Based on this assumption, in the training phase we learn the non-linear mapping between RF and text space by projecting RF corresponding to their labels for the classes we have training data(\textit{seen} category). Using this non-linear mapping we are able to classify activities without examples(\textit{unseen} category). 


Projecting RF signals onto the space of textual representation is non-trivial and poses several challenges that are addressed in this paper. First, we propose the very first context-aware RF features by explicitly learning the transition of \textit{states} (i.e., micro-activities) in an activity . We show that such a representation is robust and yields better features for activity recognition in general. Second, we propose a neural network architecture to merge text- and RF-domain representations of activities so that WiFi CSI data are mapped to the attributes and distributional characteristics of English words. This results in the first \emph{cross-modal RF embedding} work, and paves the way for device-free WiFi-based activity classification without requiring training data for all activities. Third, we propose a two-level classifier that is capable of classifying both \emph{seen} and \emph{unseen} activity types. This makes \Sys a generalized system for classifying a wide variety of human activities. 

We develop \Sys using Intel Network Interface Card (NIC) 5300~\cite{nic-card} which captures the WiFi CSI data. To develop the machine learning models, we collect training and testing data from four volunteers in a multi-person apartment as well as in an office building for \bnote{20} activity classes --- which is, to the best of our knowledge, the largest collection of activities used in any WiFi-based device-free gesture recognition system till date. \bnote{We show that \Sys is able to recognize activities with 62\%-90\% accuracy, as we vary the number of unseen classes from six to two.}

%We evaluate \Sys by developing a real system with Intel NIC 5300 card to capture CSI and implemented the algorithms for activity recognition. We collect data from four volunteers in a multi-person apartment and gathered a rich dataset with ten activity types. We evaluate the whole pipeline as well as the proposed algorithms under various scenarios and report them. 

The contributions of the paper are the following:
\begin{itemize}
     \item We describe \Sys, which is the first system that addresses the problem of learning without examples for WiFi based device-free \gnote{named} activity recognition.
     
     \item We propose a new approach to learn state-aware RF representation  to preserve the transitional characteristics of states in an activity. This representation by itself improves the classification performance in supervised learning.    
     
     \item We propose the first algorithm that exploits semantic knowledge and attributes in text to enable classification of activities from WiFi data without prior training examples.
     
     \item We collect data from four volunteers, from two environments, for 20 activities, and show that \Sys beats state-of-the-art WiFi-based activity recognition algorithms by $30\%$.
     
 \end{itemize}










==> Tamzeed_ArXIV%20(Copy)/tex/03_usecase_local.tex <==
% \section{Example Usage \note{nirjon done}}
\section{Example Usage}

\label{sec:apps}
% Current state of the art activity recognition algorithms require prior examples of an activity to recognize it. These systems do not support activity recognition without training examples. However, it is not feasible for neither the developer nor the user to provide training examples for every possible activity.

%\Sys is a device free activity recognition system with capability of recognizing activities from WiFi CSI information without any training data. 
\Sys relieves the developers and end-users from the burden of extensive data collection and training and is able to classify new types of activities for which no training examples are provided. 

There are many WiFi-based activity recognition systems such as elderly monitoring~\cite{palipana2018falldefi}, home activity recognition~\cite{wang2014eyes}, gesture based media controller~\cite{abdelnasser2015wigest}, and gesture based gaming~\cite{he2015wig} where the use \Sys can significantly improve the performance as well as the intelligence of an application. We describe one such scenario to illustrate the capability and usage of \Sys.  


\begin{figure}[!htb]
	\centering
	\includegraphics[width = 0.45\textwidth]{images/concept_cartoon.pdf}
	\caption{\Sys is able to recognize activities for which is has not been explicitly trained for.}
	\label{fig:usecase}
	%\vspace{-1.5em}

\end{figure}


%We describe one such scenario  

%This ability of \Sys opens door to many potential applications such as elderly monitoring, home activity recognition, gesture based media controller, and gesture based gaming. 

%These applications would get benefit from \Sys as it is imperative for current WiFi based activity recognition systems to collect data beforehand. However, collecting a large number of CSI sample data for each type of activity is an inconvenience. 

%In such cases, \Sys is able to recognize activities even if a user provides no sample CSI data for some of the activity classes.



Consider a simplified home activity recognition scenario which is shown in Figure~\ref{fig:usecase}. The user of \Sys wants to monitor four activities: \mytt{\{run, walk, eat, drink\}}. At first, they input this list of four activities (only the names) to \Sys. \Sys then asks the user to provide zero or more training examples for each activity. However, our user provides training examples for two out of the four classes: \mytt{\{walk, drink\}} and does not provide any example for the remaining two classes: \mytt{\{run, eat\}}. 

Despite the lack of training examples, \Sys is able to recognize the \mytt{run} activity at runtime by combining its knowledge of \mytt{walk} (from training) with its knowledge of the relationship between \mytt{run} and \mytt{walk} (which it acquired from external sources such as textual embedding).  

%In Figure~\ref{fig:usecase}, we see that \Sys is still able to recognize \mytt{\{running\}} activity even without any training example provided by the user. This reduces the burden on the end-user part and makes \Sys a more robust activity recognition system than the current state of the arts.


%We envision the applications of \Sys in scenarios where the class imbalance problem~\cite{} for audio classification persists. To further explain, we are proposing \Sys for scenarios where training examples of all possible audio classes are not available when building the model. Following are some scenarios where \Sys has potential use-cases: 

% We propose \Sys with two capabilities: a) recognize gestures without training data, b) recognize gestures in present of other persons performing random movements. These two abilities make \Sys perfect for home applications. We describe \Sys's potential use-cases in home scenarios in the following sections:

% \subsection{Recognizing gestures without examples} Passive sensing with WiFi has major use cases in elderly monitoring because a) equipping users with sensors has major overhead, b) vision based monitoring with camera has privacy concerns. However, current ambient sensing systems require training data for every possible activities to be classified. This causes hindrance for such systems as collecting data for all kind of activities is not feasible. For example, in an elderly monitoring scenario it is not possible for the user to provide the training data of \emph{falling down} which is an important activity to recognize for elderly monitoring system. Such scenarios give rise to the need of a RF sensing system that requires no training data to recognize activities or gestures. We propose \Sys  to be used in these scenarios.

% \subsection{Recognizing gestures in presence of other movement} RF Sensing systems are also used in gesture based appliance control systems such as controlling TV sound with hand gestures. However, current RF sensing systems fail to to recognize gestures in presence of other persons random movement. Some works, recognize only when other users are performing pre-defined gestures but it is not feasible to think that all the users are performing gestures that are present in training database. \Sys has the capability to recognize gestures even with the presence of other user performing random movements.

==> Tamzeed_ArXIV%20(Copy)/tex/04_design_short.tex <==
% \newpage
\section{\Sys System Design}
 \Sys takes a short-duration WiFi CSI stream (e.g., 5--8 seconds) and a list of possible activity types (i.e., a list of tags) as the input, and processes the CSI stream through a signal processing pipeline to classify it as one of those given activity types. The design of \Sys is modular. Computationally expensive modules such as the one-time offline training of the classifiers are run on a server, while the end-to-end activity classification pipeline---from sensing to classification---is runnable on embedded systems such as smartphones and tablets\footnote{Recent developments~\cite{Schulz:WiNTECH:2017} have shown how to extract CSI on smartphones. In this paper, we conduct experiments using an Intel NUC~\cite{nuc-pc}.}.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.49\textwidth]{images/pipeline.pdf}
       
    \caption{\Sys signal processing pipeline. }
    \label{fig:overview}
    \vspace{-0.5em}

\end{figure}

Figure~\ref{fig:overview} shows the signal processing pipeline of \Sys, which consists of three main steps: \emph{State-Aware Representation}, \emph{Cross-Modal Projections}, and \emph{Two-Stage Classifier}. The State-Aware Representation step extracts local and contextual features from the CSI stream. These features are projected onto the word and attribute spaces to incorporate external knowledge from the text domain in the Cross-Modal Projections step. The two-stage classifier determines if the input belongs to a seen or an unseen class and then classifies it accordingly.

There are two classes of activities that \Sys may encounter at runtime: \emph{seen} and \emph{unseen} classes. The \emph{seen} class refers to those activity types for which \Sys has labeled CSI streams for training. The \emph{unseen} class, on the other hand, refers to activity types for which \Sys does not have any training CSI stream. For example, in the home activity monitoring scenario of Figure~\ref{fig:usecase}, \mytt{\{walk, drink\}} are seen classes and \mytt{\{run, eat\}} are unseen classes.

The next three sections describe the algorithmic details of these three components of \Sys. 



==> Tamzeed_ArXIV%20(Copy)/tex/05_background_new.tex <==

\section{Background}
\label{sec:back}

\subsection{Channel State Information (CSI)} 

%Channel State Information(CSI) represents the characteristics of a wireless channel~\cite{hanzo2010mimo}. This information captures the reflection, refraction, scattering \note{and other events WHAT?} that a wireless channel faces when a signal propagate through it. When a user moves, the movement causes changes in the CSI. Let $Y(f,t)$ and $X(f,t)$ represent the frequency domain received and transmitted signal. The relation between $Y(f,t)$ and $X(f,t)$ is $Y(f,t)= H(f,t)\times X(f,t)$. Here, $H(f,t)$ is the Channel Frequency Response(CFR) carrying the channel characteristic information. CSI is the compromised of these CFR values.

In wireless communication, a transmitter and a receiver talk to each other using a certain frequency or a range of frequencies, which is often called a \textit{channel}. The \textit{Channel State Information} (CSI), as the name implies, describes the properties of a wireless channel. For example, when wireless signals travel through the medium, they fade, they get reflected and scattered by obstacles on the way, and their power decays with the distance traveled. The CSI is a measure of all these phenomena of a wireless channel. Mathematically, using the frequency domain terms, we express the relationship between the transmitted signal $X(f, t)$, the channel frequency response (CFR) $H(f, t)$, and the received signal $Y(f, t)$ as: $Y(f, t) = H(f, t)\cdot X(f, t) + N(f,t)$, where $N(f,t)$ denotes the noise. The CSI comprises of the CFR values, i.e., $\{H(f, t)\}$.

Data communication over a WiFi channel happens by sending the data bits simultaneously over 64 distinct frequencies (called the \emph{sub-carriers}) in parallel. From the WiFi Network Interface Card (NIC)~\cite{nic-card}, it is possible to obtain the CSI values of these subcarriers. The frequency response, $H(f,t)$ of each sub-carrier is a complex number, where the real and complex parts represent the amplitude and phase response, respectively. We only use with the real part (i.e., amplitude) in this paper as we find the phase values too noisy to be useful. For $N_{TX}$ transmitting antennas, $N_{RX}$ receiving antennas, and $N_S$ sub-carriers, we get a CSI matrix of complex numbers having the dimensions of $N_{TX}\times N_{RX}\times N_s$.

\subsection{Word Embedding}

The process of \emph{Word Embedding}~\cite{mikolov2013distributed} maps words in a natural language to vectors of real numbers in a manner that words that are commonly used in the same textual context are positioned closely in the vector space. Intuitively, word embedding expresses the distributional semantics of words with the motto that \emph{``a word is characterized by the company it keeps''}~\cite{firth1957synopsis}. Word embedding extracts distributional similarities among the words from a large scale text data, such as the Wikipedia, by observing the words that appear with similar words which define their context. For example, consider the words: \mytt{love} and \mytt{adore}. Syntactically these two words are quite different, but they often appear in similar semantic contexts, i.e., with similar words. Hence, the word embedding process would map these two words to two vectors whose distance is relatively closer than the embedding of two random words.   

%Word embedding represents word's semantic similarity with vector representations by learning context of words from a large text corpora. 

\begin{figure}[!htb]
	\centering
	\includegraphics[width = 0.45\textwidth]{images/w2vec.pdf}
	\caption{(a) Semantically similar words appear close to each other in the word embedding space. (b) A two layer neural network is used for Word2Vec~\cite{mikolov2013efficient} word embedding.}
	\label{fig:w2vec}
	\vspace{-0.5em}
\end{figure}

In Figure~\ref{fig:w2vec}(a), we plot the embedding of six English words. We only show the first two principal components to be able to visualize the vector representation in 2D. We observe that words with similar semantic meaning are closer in the word embedding space, e.g., \mytt{\{run, walk, move\}}, whereas words having different semantic meaning are far, e.g., \mytt{run} and \mytt{eat}. In Natural Language Processing (NLP), researchers use techniques such as neural network~\cite{wu1992introduction} and co-occurrence matrix~\cite{partio2002rock} to project words onto a $k$-dimensional vector space, and words appearing in similar textual contexts get closer embedding in the vector space. One of the most popular method to extract word embedding from a large scale corpus is \textit{Word2Vec}~\cite{mikolov2013efficient}, which uses a two layer neural network to predict the surrounding words of a target word. 

Figure~\ref{fig:w2vec}(b) shows a two-layer neural network, where a word, represented by its one-hot encoding~\cite{turian2010word}, is the input and the last layer of the network outputs the probability of other words' being its neighbour. Word-pairs of the form $\{(word, neighbor)\}$ are used to train this network, which explicitly learns to predict neighbour words of a given word, and in the process, the network implicitly learns the context of the words. After the training phase, the output of the hidden layer is used as the embedding that projects an input word to a low-dimension vector space.

\subsection{Attribute Embedding}




% \begin{table}[]
% \caption{Word Definitions and Attributes}
% \label{tab:word-attr}
% \resizebox{.5\textwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% Word  & Dictionary Definition & Aspect & Motion & Social & On Object & Uses Head\\ \hline

% Drink & \begin{tabular}[c]{@{}l@{}}To take into the\\ mouth and\\ swallow a liquid\end{tabular} & activity & \begin{tabular}[c]{@{}l@{}}low\\ motion\end{tabular} & solitary          & True      & True      \\ \hline
% Sip   & \begin{tabular}[c]{@{}l@{}}To drink in small\\ quantities\end{tabular}                  & activity & \begin{tabular}[c]{@{}l@{}}low\\ motion\end{tabular} & solitary          & True      & True      \\ \hline
% Drool & \begin{tabular}[c]{@{}l@{}}To let run from\\ the mouth\end{tabular}                     & activity & \begin{tabular}[c]{@{}l@{}}no\\ motion\end{tabular}  & Social orsolitary & False     & True      \\ \hline

% \end{tabular}
% }
% \end{table}

While word embedding captures the co-occurrence information of words used in the same context, it does not quite describe the meaning of a word. Recently, natural language processing community has proposed an effective method to learn the attributes of English \emph{verbs} from their dictionary definitions~\cite{zellers2017zero}. In this new method, verbs are expressed in terms of a set of attributes. Each verb is expressed as a vector of real numbers where each element of the vector corresponds to an attribute.    

%where the dictionary definitions of \emph{verbs} are used to learn their defnitions.       

%In the recent past, researchers~\cite{} proposed to use dictionary definitions of words to learn attributes of \emph{verb} words which define them. For eg, in the Table~\ref{tab:word-attr} we see that the attributes extracted for the verbs: drink, sip, run. 

\begin{table}[!htb]
    \centering
    \resizebox{.475\textwidth}{!}{
    \begin{tabular}{r|l}
        \textbf{Word} & \textbf{Representation} \\ \hline   
        Drink &  Dictionary:  ``To take into the mouth and swallow a liquid.''\\
        & Attributes:  \textit{(Motion, Social, Object, Head, \dots) = (low, solitary, true, true, \dots)}\\

        Sip &  Dictionary:  ``To drink in small quantities.''\\
        & Attributes:  \textit{(Motion, Social, Object, Head, \dots) = (low, social, true, true, \dots)}\\
        
        Drool &  Dictionary:  ``To let run from the mouth.''\\
        & Attributes:  \textit{(Motion, Social, Object, Head, \dots) = (none, solitary, false, true, \dots)}\\        
    \end{tabular}
    }
    \caption{Word definitions and attributes.}
    \label{tab:word-attr}
	\vspace{-1.55em}

\end{table}


Table~\ref{tab:word-attr} provides a simplified example. Three verbs: \emph{Drink}, \emph{Sip}, and \emph{Drool} are expressed in terms of four attributes: \emph{Motion}, \emph{Social}, \emph{Object}, \emph{Head}, where the attributes correspond to the degree of motion, degree of social engagement, use of objects, and use of head, respectively. We intentionally left the list of attributes open to emphasize that additional attributes are necessary to encode the dictionary definitions of a large number of English verbs.  

%since there are many other attributes that are necessary to describe English verbs.  

%the list of attributes to define all English verbs is larger than this simplified example.  

% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[width = 0.45\textwidth]{images/word_attr.pdf}
% 	\caption{Word attribute extraction}
% 	\label{fig:word_attr}
% \end{figure}

The process of attribute extraction is a standard supervised learning task where the attributes are predicted from a word's dictionary definition. In~\cite{zellers2017zero}, 24 attributes (inspired by Linguistics and verb semantics) were chosen to represent a total of 1700 English verbs. The overall process has four steps. First, the \emph{Wordnik} API~\cite{word_link} is used to obtain the dictionary definitions of the verbs. Second, a deep neural network called the \emph{Bidirectional Gated Recurrent Unit} (BGRU)~\cite{zellers2017zero} is used to encode the dictionary definitions. Third, the word embedding of the verb is concatenated to the output of the BGRU to incorporate contextual information. Finally, the concatenated encoding is fed to another neural network to obtain the attribute embedding of the verb.      

%a standard supervised task where the attributes are predicted from the word's dictionary definition. 

%In the paper~\cite{}, the authors have selected 24 attributes inspired by classical literature on liguist theories and verb semantics. The attributes can be grouped into seven clusters, some of them are following: motion dynamics, temporal duration, social dynamics, body involvements and so on. 

%The authors used Wordnik API~\cite{} for dictionary definitions and word embedding from Word2Vec to learn the attributes. They used a Bidirectional Gated Recurrent Unit(BGRU) to encode the dictionary definition and appended the word embedding of the corresponding word to also add contextual information. This concatenated encoding is then fed into a neural network to predict the attributes. The whole process is depicted in Figure~\ref{}.



==> Tamzeed_ArXIV%20(Copy)/tex/06A_representation.tex <==
\section{State-Aware Representation}
\label{sec:state-aware}

The goal of this step it to obtain a state-aware representation  of WiFi CSI values corresponding to an activity which encodes both the \emph{local} features as well as the \emph{contextual} features of an activity. \bnote{The local features refer to the frequency response of an activity at a particular time-step. In contrast, the contextual features learn the contextual relationship among the local features.} At the end of this step, we obtain an information-rich, lower-dimension vector representation of a CSI stream that captures both local and contextual features of an activity. This state-aware feature is generic, and can be used directly with an off-the-shelf supervised classifier to recognize \emph{seen} activities\footnote{In Section~\ref{sec:eval_seen}, we conduct an experiment to demonstrate its performance.}. In \Sys, we use this representation as an intermediate output, which is used by the later stages of the processing pipeline to enable recognition of both \emph{seen} and \emph{unseen} activities.     

%This state-aware feature is generic and can be used with other off-the-shelf supervised classifiers. 

%The proposed activity representation model has two components: a) Convolutional neural network and b) Recurrent neural network.

\subsection{The Need for State-Aware Representation} 

The CSI stream is a time series of complex numbers, sampled at a rate of between 200Hz~\cite{virmani2017position} to 2.5KHz~\cite{wang2015understanding}. The raw CSI data are not practical for direct use in the training or in the classification steps, as with high sampling frequency, the dimension of the input vector becomes too large to process efficiently. Moreover, raw CSI signals do not explicitly reflect the intrinsic characteristics of the high-level activity, and generally, they contain artefacts of environmental factors that are not related to the target activity. Hence, like most sensing and inference systems, we map raw data to a lower dimensional vector, commonly known as the \emph{feature vector}, based on the time and frequency domain properties of the signal. 

A wide variety of features have been proposed in the literature for activity recognition from WiFi CSI data. The list includes classic time and frequency domain features such as cepstral coefficients and spectral energy~\cite{wang2014eyes}, as well as recent practices where a layer of a trained deep neural network is considered as the learned features~\cite{yue2018extracting}. However, none of these techniques consider the sequential nature of an activity when converting raw CSI values to feature vectors. 

%p2,r1
%p1,r2

\begin{figure}[!htb]%
\centering
\subfloat[Two Examples of \emph{`Run'}]{%
\includegraphics[height=.65in]{images/p2}
\includegraphics[height=.65in]{images/r1}
}%
\enspace
\subfloat[Two Examples of \emph{`Push'}]{%
\includegraphics[height=.65in]{images/p1}
\includegraphics[height=.65in]{images/r2}
}%
\caption{Different activities have different state sequences.}
\label{fig:state-seq}
	\vspace{-1.55em}

\end{figure}

% \begin{figure}[!htb]
%     \centering
%     % \vspace{-1em}
%     \includegraphics[width=0.45\textwidth]{images/run_push_spec.pdf}
%     \caption{Different activities have different state sequences. \rnote{Upload the images and PPT. Need polishing.}}
%     \label{fig:state-seq}
% \end{figure}

%Gestures and activities are time-series of states that occur sequentially. Each activity contains a sequence of micro-activities or \emph{states}. For example, in Figures~\ref{fig:state-seq}(a) and ~\ref{fig:state-seq}(b), we show the spectrogram of \emph{running} and \emph{pushing} activities over a duration of eight seconds. We observe that the two activities have distinct patterns and sequences of frequency response (state) in the time-frequency domain. 

Human gestures and activities are time-series of micro-activities that we call \emph{states}. For example, in Figures~\ref{fig:state-seq}, we show four spectrograms of CSI values where the first two correspond to two examples of the \mytt{run} activity, and the last two corresponds to two examples of the \mytt{push} activity. We observe that the pattern how the frequency response changes over the duration of an activity is similar (if not quite the same) for the same activity, and dissimilar for the two different activities. Hence, the key to recognize an activity is to model the sequential change in its frequency spectrum.       

%\emph{running} and \emph{pushing} activities over a duration of eight seconds. We observe that the two activities have distinct patterns and sequences of frequency response (state) in the time-frequency domain. 

To capture the sequential properties of gestures and activities, ~\cite{wang2015understanding} uses a \emph{Hidden Markov Model} (HMM)~\cite{srinivasan2017preventive} where traditional time-frequency features (\emph{Discrete Wavelet Transform} (DWT)~\cite{wang2015understanding}) are used to represent the states rather than learning representation that embeds the sequential properties of states. A fundamental limitation of this and any other classical HMM-based approaches is that the Markovian assumption, i.e., a state depends only on the previous state, does not hold for most activities. These models do not work when the number of states is large and variable, and an activity has longer term dependencies between the micro-activities that constitute it. 

\begin{figure}[!htb]
    \centering
    % \vspace{-1em}
    \includegraphics[width=0.45\textwidth]{plot/state_pred.pdf}
    \caption{Looking back deeper in time improves modeling accuracy. }
    \label{fig:markov}
	\vspace{-1.0em}

\end{figure}

% \bnote{Add and discuss a plot here showing how the Markovian property does not hold for a simple activity and how long-term dependency among states/micro-contions hold and that should justify the LSTM model.}
%The closest to our work is only~\cite{} which models the activity classifier as a hidden markov model, 

%But does not learn the feature considering the sequence of micro-activities. They use traditional time-frequency (Discrete Wavelet Transform) as features for their hidden markov model. 

%In our model, we want to recognize this sequential nature of activities and propose a state-aware representation for the activities. In this paper, we propose the first model to extract state-aware feature  representation for raw CSI stream. This state-aware feature is generic and can be used with other off-the-shelf supervised classifiers.

To demonstrate this, we conduct an experiment to predict the next state of an activity based on the previous states. We use five activities \{\mytt{push, pull, run, walk, eat}\} and divide each sample into five segments that represent the states that constitute an activity. To test the Markovian assumption about the longer term dependencies among the micro-activities, we consider two variants: (a) \emph{One step Look-Back}: a five-state Markov model resulting in a $5 X 5$ dimension transition matrix, $A$, where each entry, $A_{ij}$ represents the transitional probability of going from state $i$ to state $j$, and (b) \emph{Two Step Look-back}: a 25-state Markov model resulting in a $25 X 5$ dimension transition matrix, $A$, where each entry, $A_{ijk}$ represents the transitional probability of going from state $ij$ to state $k$. In Figure~\ref{fig:markov}, we observe that using the one step look-back, we get an average accuracy of $20\%$ for predicting the next state. We observe an improvement of prediction accuracy ($63\%$) when we use the two step look-back variant, which conditions on previous two states to predict the next state. This tells us that a strong Markovian assumption that the current state only depends on previous state does not hold strongly for activity's sequence of states and looking back deeper in time improves the modeling accuracy.  

To overcome the limitations of existing activity modeling techniques, we propose \emph{state-aware} feature representation of CSI streams that captures complex, non-linear dependencies between micro-actions that constitute an action---without requiring a strict Markovian assumption or a predefined, fixed set of states. To achieve this, we employ state-of-the-art deep neural networks that capture both the local (static) as well as contextual (sequential) properties of CSI spectrograms. Our proposed state-aware model is able to predict the next state of an activity with  $90\%$ accuracy(Figure~\ref{fig:markov}), which is $30\%-70\%$ higher than Markovian models. 

%\emph{Long-Short-Term-Memory} (LSTM)~\cite{} as the basis, and extend it to consider the bi-directional dependencies among the states to have a robust representation of activities and gestures from WiFi CSI values. 

%The details of this step is described in Section~\ref{sec:state-aware}. Note that, this step by itself improves the state-of-the-art of gesture modeling techniques, and can be used directly with a standard supervised classifier to recognize activities. However, to achieve the ultimate goal of this paper, we require to project this RF-domain representation of activities on the textual domain to enable classification of unseen activities.



\subsection{Rationale Behind Deep Neural Networks}

In \Sys, a \emph{Convolutional Neural Network} (CNN)~\cite{goodfellow2016deep} and a \emph{Recurrent Neural Network} (RNN)~\cite{goodfellow2016deep} are used in tandem to capture the local and the contextual features, respectively.  

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.45\textwidth]{images/rnn.pdf}
    \caption{CNNs learn local patterns that characterize each state, whereas RNNs (LSTMs) learn sequence of states.}
    \label{fig:cnn_rnn_justify}
\end{figure}

%A CNN is used to extract the local features from the spectrogram. 

The CSI spectrogram exhibits rich, informative, and distinguishable patterns for different states within an activity. It contains temporal information, for which, a CNN is the most suitable choice~\cite{goodfellow2016deep}. CNNs contain a hierarchy of filters, where each filter's job is to detect the presence of a particular pattern in a small region on the spectrogram. In Figure~\ref{fig:cnn_rnn_justify}, we use rectangular boxes on the spectrogram which are recognized by the different convolutional filters of the CNN shown on the left.

To model the sequential variation of states within an activity, we use an RNN. We choose an RNN over classical approaches such as a Hidden Markov Model (HMM) since unlike HMMs, RNNs do not require a strong Markovian assumption~\cite{delsole2000fundamental}. With RNNs, a model can learn long-term dependencies among the states. Furthermore, neural networks are in general better at learning complex patterns within the data than shallow models, and RNNs do not need fixed states like an HMM does. In Figure~\ref{fig:cnn_rnn_justify}, we use slices of a spectrogram to denote states and use arrows to illustrate the inherent dependencies between nearby states. 

To construct the RNN, we choose \emph{Long Short Term Memory} (LSTM) as the recurrent component since LSTMs are better at learning long-term dependencies between states~\cite{goodfellow2016deep}, which makes them suitable for capturing relationship between the past states with the recent states. To preserve contextual information from both the future and the past states, we use a bi-directional LSTM model. \bnote{A unidirectional forward LSTM only captures the state transition from past to recent states. But a bi-directional LSTM learns how future states influence past states as well. In many cases, it is important to bring information from the last few states to model an activity and bi-directional LSTMs have this feature.}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.4\textwidth]{images/lstm.pdf}
    \caption{Network architecture for state-aware representation.}
    \label{fig:conv_lstm}
	\vspace{-1.55em}

\end{figure}

\subsection{Detailed Algorithmic Steps} 

Figure~\ref{fig:conv_lstm} shows the integrated neural network architecture that takes CSI spectrogram as the input and produces the state-aware vector representation through a sequence of processing steps. 

$\bullet$ \emph{CSI Processing:} For a given CSI stream, $X$ that corresponds to an instance of an activity, we divide the CSI values into $n$ \bnote{equal} segments $\{X_1, X_2, \dots, X_n\}$. Here, $n$ is empirically determined, we used $n=5$ in all our experiments. For each segment $X_i$, we take the spectrogram~\cite{lu2009deconvolutive} to obtain $S_i$ as follows:
\[
\mathrm{S_i = STFT(X_i)} 
\]
where, STFT(.) denotes \textit{Short-Time Fourier Transform}~\cite{lu2009deconvolutive}, which estimates the short-term, time-localized frequency content of $X_i$.

$\bullet$ \emph{CNN Processing:} We use a three-layer CNN, $G_{\theta}$, where $\theta$ are the parameters of the network, which takes $S_i$ as the input and produces a $1,000$ dimension vector, $L_i$ that represents the local features of the input spectrogram:
\[
\mathrm{L_i = G_\theta(S_i)} 
\]

%$S_t$ is then fed to convolutional neural network $G(\theta)$. Here, $\theta$ are the parameters of the network. As the architecture of $G_{\theta}$, we use four layers of convolutional layers with max pooling and batch normalization. 

Each layer of the CNN extracts a feature map from the input data. As we go deeper into network, the deeper-layer filters extract more information. We empirically determine that three layers of convolutional operations extract adequate information for the later steps of \Sys. The filters have a size of $3 X 3$ and we increase the depth from $16$ to $64$ channels for the three layers.  We use \emph{Rectified Linear Units} (ReLu), $\sigma(a) = \max\{a, 0\}$ as the non-linear activation function for their robustness against the vanishing gradient problem~\cite{hochreiter1998vanishing}. The output of the third convolutional layer is fed into two \emph{dense} layers~\cite{goodfellow2016deep} with a ReLu activation layer in-between them. We keep $1,000$ neurons in the last dense layer, which is the dimension of the local feature vector. 

$\bullet$ \emph{RNN Processing:} For a total of $n$ segments, we obtain $n$ local feature maps $G_{\theta}(S_i)$ from the CNN. Each state's local feature is fed into a bi-directional LSTM (bi-LSTM) to model the contextual property of the states of an activity. The bi-LSTM network has two unidirectional LSTMs, i.e., a \emph{forward} and a \emph{backward} LSTM. For the forward LSTM, each hidden state $\overrightarrow{H_i}$ depends on the previous state $H_{i-1}$ and the input $S_i$. On the other hand, for the backward LSTM, each hidden state $\overleftarrow{H_i}$ depends on the future state $H_{i+1}$ and the input  $S_i$. By using a bi-directional LSTM, we obtain a representation of an activity that is aware of the transition of states which yields a strong model of the activities. We use 500 neurons in both the forward and the backward LSTMs. Each LSTM has a dropout layer to avoid overfitting.

$\bullet$ \emph{Representation:} The final  hidden representation of the bidirectional LSTM is the concatenation of $\overrightarrow{H_i}$  and $\overleftarrow{H_i}$.


==> Tamzeed_ArXIV%20(Copy)/tex/06B_CMP.tex <==

\section{Cross-modal Projections}
\label{sec:CMP}

In the previous section, we proposed a feature learning algorithm that learns to map CSI stream segments onto a feature space that  captures the contextual information of sequential states of each activity. This gives us a robust activity representation, which by itself can directly be used to train robust activity classifiers. However, that representation can not be used to perform zero-shot learning as it does not borrow knowledge from an external source. In this section, we describe the cross-modal projection step of \Sys which brings external knowledge from the text domain to enable classification of unseen activities. 

\subsection{The Need for Cross-Modal Projections}

\gnote{Existing CSI-based human activity recognition systems can recognize only a fixed set of activities for which the system has been trained for. When an unseen activity is presented to these systems, the best they can do is to find the class that is closest to the given activity. Due to their reliance on a single source of knowledge (i.e., only WiFi CSI-based training data), these systems by design cannot generate a new class label that describes the unseen example. By having additional sources (or \emph{modes}) of knowledge, e.g, the relationship among words and their attributes in the English text, we can enhance the ability of these systems to recognize previously unseen activities, and to generate class labels that come from the additional knowledge sources (i.e., the text domain).}         

The secret recipe behind \Sys's ability to classify unseen activities is the \emph{cross modal projection}. Through this step, we blur the difference between an activity's CSI stream and its corresponding English word embedding and attributes, and make them (almost) equal in their feature representations. In other words, if an English word (say, \mytt{run}) has a known vector representation (e.g., obtained using Google's Word-2-Vec~\cite{mikolov2013efficient} on a large dataset like Wikipedia) and a vector of attributes of the word (e.g., \emph{movement of legs} and \emph{motion of hands}, which is obtained from~\cite{zellers2017zero}), the goal of the cross-modal projection is to generate the exact same vectors when \Sys is presented with a CSI stream of that word (i.e., CSI of running). 
%\end{itemize}

%This is illustrated in Figure~\ref{fig:cm-pipeline} 
\begin{figure}[!thb]
    \centering
    \includegraphics[width=0.48\textwidth]{images/cross_modal_pipe.pdf}
    \caption{Cross-modal projections map a CSI stream to its corresponding label in the word and attribute embedding spaces.}
    \label{fig:cm-pipeline}
    \vspace{-1.0em}
\end{figure}




% ... WHY? Mention it combines or selects these two different representation. Provide an example where word is better and an example where activity-attribute is better.}

Figure~\ref{fig:cm-pipeline} illustrates cross-modal projection using \mytt{run} as the example activity, whose word embedding and attribute vectors are $X$ and $A$, respectively. In \Sys, the activity representation of \mytt{run} is passed through two cross-modal projection steps to obtain $Y_x$ and $Y_A$, corresponding to the word and the attribute spaces, respectively, and it is made sure that $Y_x \approx X$ and $Y_A \approx A$. In traditional feature representation, however, the projection is different (i.e., $Y \neq$ X and $Y \neq$ A), and hence, unlike \Sys, traditional features cannot guess the word label of an unseen activity.


\subsection{Rationale Behind Multiple Projections}

The benefits of cross-modal projection from CSI to two latent spaces, i.e., word and activity-attribute spaces, are as follows: 

%\begin{itemize}
    $\bullet$ \emph{Word Embedding Space:} There are over 150 thousand English words for which researchers in the natural language processing field have created semantically aware vector representations, called the \emph{Word Embedding}. Such an embedding preserves the contextual relationship among words and puts two words that are similar in meaning or are often used in the same context closer in the representation space. By projecting the activity representation to the word embedding space, \Sys is able to generate meaningful and context-aware representation of any CSI stream, irrespective of whether or not it has seen CSI of the same class before.
%\vspace{1em}

    $\bullet$  \emph{Activity-Attribute Space:} Human activities and bodily gestures comprise of movements by different body parts, i.e., arms, legs, head, and torso. Activities also involve external objects, e.g., an \mytt{eating} activity may involve the use of spoons and knives. These \emph{attributes} create nuances in different RF-based activity feature representations. Projecting CSI onto the activity-attribute space embeds this information into the projection, as CSI implicitly gets affected by moving different sorts of objects due to their reflections. Using this embedded contextual and attribute information from CSI, \Sys recognizes activities without any training examples.

\Sys uses both word embedding and activity-attribute spaces for cross-modal projections to combine the predictive power of both. Combining these two help each other in the final prediction step. For example, in the word embedding space (50 dimensional W2Vec), \mytt{run} is surprisingly closer to \mytt{pull} than \mytt{walk}, since they appear more with similar neighbouring words. However, \mytt{run} and \mytt{walk} are more similar in terms of activity properties. In the attribute space, however, \mytt{run} and \mytt{walk} are closer to each other. In such scenarios, where relying only on the contextual semantic information fails to figure the correct relationship between activities, the attribute information helps correct the misprediction. 

Likewise, in many cases, the attributes extracted for two activities are very similar. For example, \mytt{run} and \mytt{walk} have the exact same attribute (binary) vectors when the attributes are constructed from online dictionaries~\cite{zellers2017zero}. While we desire their vectors to be closer in the attribute space for these two activities, we do not want them to be exact. This is because if they are the same, the RF projections for these two activities will also be the same. Thus, \Sys will not be able to distinguish between \mytt{walk} and \mytt{run} if we only rely upon the attributes. In such scenarios, the word embedding helps correct the problem and \Sys is able to separate the activities in the joint feature space.  

\subsection{Detailed Algorithmic Steps}

%We propose an algorithm that integrates semantic knowledge from the text domain and attribute knowledge from activity definition to the state-aware activity representation. This is done by projecting the robust activity representation onto both text space and attribute space such that each activity representation is mapped to its corresponding label in the latent spaces namely: 

%. Therefore, in both spaces, the labels have fixed representations. Unlike words and attributes,

The goal of cross-modal projection is to map state-aware representation of WiFi CSI streams (Section~\ref{sec:state-aware}) to two latent spaces, i.e., the word embedding space and the activity-attribute space. The difficulty in this step is that although the class label corresponding to an activity has a fixed word embedding and a fixed attribute-vector, the CSI values corresponding to the same activity vary due to the diversity in human motion and physique. This makes the mapping from the CSI domain to the word-embedding and activity-attribute spaces a non-linear projection problem. In \Sys, we solve this problem by using a neural network to learn the projection from CSI to the latent spaces. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.45\textwidth]{images/double_cross_modal.pdf}
    \caption{State Aware Representation is projected into both Word-embedding and Attribute space which are then aggregated for a joint projection.}
    \label{fig:joint-cross}
     \vspace{-.75em}

\end{figure}


The projection operation is illustrated by Figure~\ref{fig:joint-cross}. The state-aware representation, i.e., the output of the LSTM from Figure~\ref{fig:conv_lstm}, is fed to two neural networks having fully connected layers. The first network projects the state-aware representation onto the activity attribute space, and the second network projects the representation onto the word embedding space. We refer to the last layer of the neural networks that perform attribute space projection and word embedding projection as $F_A$ and $F_W$, respectively. 


$\bullet$ \textit{Projecting onto Activity-Attribute Space.} From the attribute database provided by~\cite{zellers2017zero}, we obtain a set of binary attributes associated with each activity. Each activity, $a_i$ is represented as an $m$-dimension vector, $d_i \in \{1, 0\}^m$, where $m$ is the total number of attributes used to define an activity. Each element $d^{(k)}_i$ is a binary indicator of whether the $k^{th}$ attribute is true or false for that activity.  

%One branch of MLP coming out of state-aware representation is used for projecting the representation of CSI as close to as their corresponding activity's attribute vectors. This entails that the vector representation of the CSI's projection onto the attribute space will be very close to the activity's attribute vector.

%Formally, for each activity $a$, we have a $k$-dimensional vector $p_a$ for its attributes which is defined as following:

\begin{equation}
    d^{(k)}_{i}=
    \begin{cases}
      1, & \text{if attribute $k$ is true for activity $a_i$.}  \\
      0, & \text{otherwise}
    \end{cases}
\end{equation}

To get the likelihood of a CSI stream being predicted as an activity $a_i$, we project  $F_A$ to the attribute space. We take the dot product of the attribute vector $d_i$ and $F_A$. The dot product demonstrates the similarity between the projection $F_A$ with attribute vector 
$d_i$. For a CSI stream from activity $a_i$, our model's target is to increase the similarity between $d_i$ and $F_A$. The similarity which denotes the likelihood of $F_A$'s probability of belonging to activity $a_i$ in attribute space is calculated as a dot product:

\begin{equation}
    P^i_A = d_i \cdot F_A
    \label{eq:proj_a}
\end{equation}

% \st{To calculate the probability of an activity, the CSI stream's activity-attribute MLP's last layer $F_A$ is projected into attribute space and we take the softmax probability of the projections. To formally define for a an activity $a$ the probability of $F_A$ belonging to it is calculated as follows:}

% \begin{equation}
%     %\rnote{p(a|F_A)=softmax(\sum_i {p^i_{a}F_A})} \\
%     p() = \sum_i {p^{(i)}_{a} F_A}\\
%     \label{eq:proj_a}
% \end{equation}
% \rnote{Kept only the part that will be used later in step 3. (Unclear if the above eqn makes sense. What kind of multiplication and summing is happening? Dimensions match?)}



%This branch of MLP is responsible for projecting the state-aware representation into word embedding space. We aim to project an activity's CSI signature to be projected near to its class label's word embedding. 

$\bullet$ \textit{Projecting onto Word-Embedding Space.} For an activity, $a_i$ whose word embedding is $w_i$, we want to project the CSI-based state-aware representation as close as possible to $w_i$.  \bnote{Therefore, for a CSI stream of an activity $a_i$,  our target is to project  $F_W$  to be close to $w_i$ in vector space
} This results in a higher value of dot product between $F_W$  and $w_i$. Therefore, the similarity in word embedding space is defined as following: 
\begin{equation}
    %p(a|F_W)=softmax(w_aF_A) \\
    P^i_W = w_i \cdot F_W
    \label{eq:proj_w}
\end{equation}
%Therefore, we feed the dot product into a softmax layer to calculate the probability of a projection belonging to a class. The equation is as follows:


$\bullet$ \textit{Projecting onto the Joint Space.} To obtain a joint projection on both the attribute and the word embedding space, we employ an ensemble approach to combine the two projections from Equations~(\ref{eq:proj_a}) and~(\ref{eq:proj_w}) as follows: 
\begin{equation}
    P_i =P^i_A +P^i_W
\end{equation}
where, $P_i$ carries the confidence of a CSI segment's probability of belonging to class $a_i$. For |a| number of activities, given $F_A$ and $F_W$ extracted using state-aware representation for a CSI segment $X$ as described in Section~\ref{sec:state-aware}, the probability of $X\in a_i$ is calculated using the following softmax operation:
\begin{equation}
\label{eqn:softmax}
    p(a_i|F_A,F_W)=\frac{e^{P_i}}{\sum^{|a|}_{j=1} e^{P_j}}
\end{equation}



% \rnote{Discuss. This looks like summing up scalars and then softmax of a scaler!}


==> Tamzeed_ArXIV%20(Copy)/tex/06C_classify.tex <==
\section{Two Stage Classifier} 
\label{sec:classify}

%The \emph{seen} classes refer to those activity types for which \Sys has labeled CSI streams for training. The \emph{unseen} class, on the other hand, refers to activity types for which \Sys does not have any training CSI stream. For example, in the home activity monitoring scenario of Figure~\ref{fig:usecase}, \mytt{\{walking, drinking\}} are seen classes and \mytt{\{running, eating\}} are unseen classes. 

%There are two classes of activities that \Sys may encounter at runtime: \emph{seen} and \emph{unseen} classes. During the classification step, at first, \Sys employs a \emph{novelty detection} algorithm to determine whether the input CSI stream belongs to a seen class or an unseen class. After this determination, a \emph{nearest neighbor} classifier is used to find the most probable activity type for the input CSI stream. 

\Sys employs a two-stage classifier to infer the most likely activity type for an input CSI stream segment. The first-stage classifier determines whether the input CSI stream segment belongs to a \emph{seen} or an \emph{unseen} class. The second-stage classifier makes the final determination of the most probable activity type for the input CSI stream segment. 

%The use of a two-level classifier significantly improves the accuracy of \Sys, because we propose a holistic approach to classify both \emph{seen} and \emph{unseen} classes together. 

%The details of this two-level classifier is described in Section~\ref{sec:classify}. 

\subsection{The Need for Two-Stage Classifier}

Neural networks tend to memorize patterns in data from training. Thus, even for an unseen category, the network tries to project an input close to one of the seen classes in the state-aware representation space. While this serves our purpose of classifying an unseen activity, it affects the classification performance of a generalized system where the system may encounter examples from both seen and unseen classes. Since the unseen classes are projected too close to the seen classes, they will be classified as one of those seen classes. In Figure~\ref{fig:two-step-classifier}(a), we plot the first two principal components of our proposes state-aware activity representation for two activities: \mytt{run} and \mytt{walk}. Here, the state-aware representation is trained with samples from \mytt{walk}. We see that for these two activities, the projections are very close to each other with some overlaps. This results in errors in deciding the samples from \mytt{run} (an unseen category) and they get classified as \mytt{walk}. 


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.45\textwidth]{images/two_step.pdf}
    \caption{(a) State-aware activity representation projects samples of unseen class \emph{run} close to samples of seen class \emph{walk}  (b) Spectrogram level feature  projects the samples of unseen class \emph{run} far from the samples of seen class \emph{walk}.}
    \label{fig:two-step-classifier}
 	\vspace{-1.15em}

\end{figure}

To overcome the problem posed by neural network based state-aware representation in distinguishing seen vs. unseen categories, we employ a classifier which is based on the signal characteristics such as the time-frequency representation. To be more precise, while some activities such as \mytt{run} and \mytt{walk} have similarity in their attributes, they still have distinguishable signal characteristics that are embedded in WiFi CSI. Past works~\cite{wang2015understanding, wang2014eyes} have proven the distinguishable power of traditional signal-level features such as Short Time Fourier Transform (STFT) and Discrete Wavelet Transform(DWT). We use STFT to detect if a sample is from a seen or an unseen category. STFT gives us the changes in frequency components of the signal along the time axis.  

In Figure~\ref{fig:two-step-classifier}(b), we  plot the first two principal components of the STFT for the samples \mytt{run} and \mytt{walk}.  We see that they are well separated in the STFT representation, which allows us to determine if an example is from a seen or an unseen category. 

\subsection{Detailed Algorithmic Steps}

The two steps of the algorithm are as follows:

$\bullet$ \textit{Seen vs. Unseen Detection.} We devise a simple threshold-based decision algorithm to determine whether an input CSI stream segment belongs to an \emph{unseen} class. We use K-means~\cite{krishna1999genetic} clustering algorithm to cluster the STFT of the training samples of the seen category classes. This gives us $K$ cluster centers, ${C_1,C_2,\dots,C_K}$ for $K$ seen classes. For an input CSI stream segment, $u$, it belongs to an \emph{unseen} class if the following condition is true:
\begin{equation}
    \min_{s \in S} \| C_s - STFT(u) \| > \Omega
\end{equation}
% \rnote{change the symbols to make them consistent everywhere in the paper.}
where, $S$ is the set of \emph{seen} classes and $\Omega$ is an empirically determined threshold that maximizes the accuracy of \emph{seen} vs. \emph{unseen} class detection, and $\|.\|$ is the Euclidean norm. When this condition is false, $u$ belongs to a \emph{seen} class.


% \subsection{The Need for Two-Stage Classifier}

% The nature of neural network makes it to memorize patterns of data from training. Thus, even for unseen category the network will try to classify it as one of the seen category classes. However, due to variance in feature distribution for unseen class they are assigned with lower probabilities for seen category classes. For example, lets consider we have \emph{walking} as seen category and  \emph{running} as unseen category. In Figure~\ref{}, for a sample of \emph{walking} we see the probability for different classes in seen category. For the class \emph{walking} we have the maximum probability of $0.91$. In  Figure~\ref{}, we see that in the unseen category the maximum probability is $0.56$ for \emph{running} as  \emph{walking} and  \emph{running} are similar in terms of many attributes. 
% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.45\textwidth]{images/two_step_classifier_main.pdf}
%     \caption{Probability densities for seen and unseen samples. \rnote{labels needed. Why there are two densities?}}
%     \label{fig:two-step-classifier}

% \end{figure}

% Now, for a sample from unseen category \emph{running}, in  Figure~\ref{} we see that the maximum probability among seen classes is for \emph{walking} $(.68)$ which is less than the sample from \emph{walking}. For unheard category the maximum probability is for \emph{running} which is $(.65)$. This gives us the motivation for a two-stage classifier. \rnote{The example is quite confusing. And it was unclear how it motivates a two-stage classifier. Discuss.}


% %First, we get the probability  from the joint space projection for the seen category. If we find the probabilities are under an empirically determined threshold then we determine the sample as an unseen category and send it to the rest of the pipeline. We only consider the unseen category labels and choose the unseen class with maximum probability. On the other hand, if the probabilities are not below the threshold then we choose the activity with maximum probability as the assigned class for the sample.

% \subsection{Detailed Algorithmic Steps}

% The details of the two-stage classifier are presented as follows. 


% $\bullet$ \textit{Seen vs. Unseen Detection.} We devise a simple threshold-based decision algorithm to determine whether an input CSI stream segment belongs to an \emph{unseen} class. For an input CSI stream segment, $u$, it belongs to an \emph{unseen} class if the following condition is true:
% \begin{equation}
%     \min_{h \in H} \| E(h) - \rho(u) \| > \Pi
% \end{equation}
% \rnote{change the symbols to make them consistent everywhere in the paper.}
% where, $\rho(u)$ is the CSI stream segment embedding, $H$ is the set of \emph{seen} classes, $\Pi$ is an empirically determined threshold that maximizes the accuracy of \emph{seen} vs. \emph{unseen} class detection, and $\|.\|$ is the Euclidean norm. When this condition is false, $u$ belongs to a \emph{seen} class.    

%discriminative 

$\bullet$ \textit{Classification.} If the CSI segment is recognized as from a \emph{seen} category, only the labels from seen category are considered and the class label is obtained by applying the following equation:
\begin{equation}
    \argminB_{a_i} p(a_i|F_A, F_W)
    \label{eq:clabel}
\end{equation}
On the other hand, if the CSI segment is recognized as from an \emph{unseen} category, we exclude all the labels from the \emph{seen} category and only the labels from the \emph{unseen} category are considered and the class label is obtained by applying Equation~\ref{eq:clabel}.  

%choose the label from \emph{unseen} category that has the maximum probability as given by Equation~\ref{eqn:softmax}.



==> Tamzeed_ArXIV%20(Copy)/tex/07_implementation.tex <==
%\section{Implementation Notes}
\section{Experimental Setup}
\label{sec:impl}

\begin{figure}[!htb]%
\centering
	\includegraphics[width = 0.45\textwidth]{images/exp_setup.pdf}
	\caption{(a) Intel Nuc with Antennas. (b) Experimental Setup.}
	\label{fig:exp-setup}
	\vspace{-1.5em}
\end{figure}

\subsection{WiFi CSI Collection} 

We implement \Sys on an Intel NUC~\cite{nuc-pc} mini PC. The mini PC is interfaced with an Intel NIC 5300~\cite{nic-card} and three omni-directional antennas with 6 dBi gain. To extract CSI values from the NIC card, we use the tool developed by Halperin et. al~\cite{halperin2011tool}. This tool provides a modified firmware for NIC 5300 and an open source Linux driver with user space tools to collect CSI information of the received packets. We use a Netlink router as an access point (AP). The mini PC pings the AP periodically at a certain interval and the CSI is extracted from the packet that is received by the mini PC as an echo from the AP. The sampling rate of ping is set at 500 sample per second. The PC and AP are placed 12 feet apart from each other. Experiments are done in a student apartment and an office space.  Both rooms have typical furniture, e.g., two tables, multiple chairs, and cabinets. Activities are performed by four volunteers (1 female and 3 males). Figure~\ref{fig:exp-setup}(a) shows the mini PC Intel NUC connected to three antennas which we place on a stand during the experiments. Figure~\ref{fig:exp-setup}(b) shows the the two rooms with our experimental setup.

\subsection{Noise Reduction}

CSI data extracted from the NIC card suffer from dominant noise, which makes gesture recognition  difficult. To remove noise, we follow~\cite{wang2015understanding}'s PCA-based denoising technique. Since the Channel Frequency Response (CFR) for different subcarriers is a linear combinations of the same set of waveforms with different initial phases, when a gesture is performed, the changes of CFR value in different subcarriers are correlated. To extract the changes in CFR values caused by the movement in different subcarriers, we apply PCA on the CSI stream collected from 30 subcarriers for each TX-RX antenna pair. The ordered principal components give us the most variances experienced across all sub-carriers. We discard the first principal component stream as it contains dominant effect of noise. The second and the third components contain clear effect of gestures and less effect of noise. We choose the third stream as it has shown better noise immunity. Although the selected stream is less prone to noise, it still contains some effect of unwanted high-frequency noise. Hence, the stream is passed through a Butterworth filter~\cite{selesnick1998generalized} to remove static noise. We set a cut off frequency of 50Hz as human activity is usually  below 50Hz in frequency. Thus, we obtain a de-noised CSi stream from all sub-carriers.
 
%  \begin{figure}[!h]%

% \label{fig:Denoising}%
% \centering
% 	\includegraphics[width = 0.45\textwidth]{images/denoising.pdf}
% 	\caption{(a) Before denoising CSI stream has dominant noise. (b) After denoising all high frequency noise components are removed.}
% 	\label{fig:denoise}
% 	\vspace{-1.05em}
% \end{figure}

% Then, the 30 PCA streams are passed thorugh a low pass filter to remove static noises. We use a butterworth low pass filter. We set up a cut off frequency of 30Hz. ~\cite{CARM} suggests to discard the first PCA stream as it contains dominant noise and recommends to use the second and third stream. We use the third stream only as we found from our experiment it has lower noise level and we need only one stream per TX-RX antenna pair.  Thus, we get only one CSI stream for each TX-RX antenna pair.

\subsection{Gesture Segmentation}

In order to detect the start and the end of a gesture, we instruct the volunteers to perform gestures with a brief pause between them. As the peaks in a CSI stream depends on the initial position of the user, which is variable for different gestures, we cannot segment gestures by directly applying a threshold on the CSI values. Instead, we follow~\cite{virmani2017position} and take the first order difference of the stream which is stable during the pause and fluctuates during gestures. We apply a threshold-based peak detection technique on the first order different to detect gestures. The segments on the first order difference that are above a predefined threshold are detected as gestures. We refer~\cite{virmani2017position} to the readers for more details on pre-processing of CSI stream.







%  In Figure~\ref{fig:denoise}(a) we see the noisy raw CSI stream of a user performing a push gesture repetitively. After performing the denoising step we get a filtered CSI stream in Figure~\ref{fig:denoise}(b).
 
 
 \subsection{Data Augmentation} 
 
 To avoid overfitting and to make our model robust, we use a data augmentation technique to increase the user contributed data size by about 20 times. First,  we apply a geometric transformation to the time-frequency representation of the raw CSI signals. Specifically, we use translation to shift the spectrogram along the time axis. We exclude shifting along the frequency axis, as it does not reflect any physical world phenomenon. Shifting along the time axis reflects the effect of recording the same gesture at different timestamps. Second, We superimpose simulated noise on the signal to augment the dataset further. Each signal is superimposed with a Gaussian white noise~\cite{islam2017soundsifter}. The noise model is generated offline. Injecting noise captures environmental effect and makes the model resilient to noisy environment.

\subsection{Empirical Dataset} 

In this section, we describe our dataset collection method. \Sys leverages knowledge from the text domain using the activity names to classify activities without training examples. For that reason, we need \emph{named} activities that have semantic representation in English language. For example, \Sys is able to classify \emph{run} if it has seen training examples of \emph{walk} based on the semantic relationship between these two words. However, \Sys won't be able to classify activities without having semantic meaning in English or any other language.

Based on our study of named activities from~\cite{anguita2012human,anguita2013public,venkatnarayan2018multi}, we collect $20$ most common named activities for our empirical evaluation. To the best of our knowledge, this is the largest dataset in terms of the number of classes considered in WiFi-based activity recognition systems. Existing literature have used 6--8 types of gestures for supervised activity recognition from WiFi~\cite{virmani2017position, venkatnarayan2018multi, wang2014eyes, wang2015understanding}. Our dataset contains activities collected from four volunteers in two different rooms with different orientations and furniture. Our dataset is diverse and it stresses out the algorithmic components of \Sys. In Table~\ref{tab:act-list}, we provide the list of the $20$ activities clustered with major attributes. On average, each class have $100$ samples.

\begin{table}[!htb]
 \centering
\resizebox{.38\textwidth}{!}{
\begin{tabular}{r|l}

\textbf{Category}            & \textbf{Activities}  \\ \hline
Freehand Gestures   & Point, Raise, Rub, Scratch, Shake,\\ 
           & Toss, Circle, Arc.\\ 
Object-Human Interactions    & Drink, Eat, Push, Pull.\\ 
Upper/Lower-Body Gestures & Sit, Stand, Bow, Duck, Kick.\\ 
Mobility    & Jump, Walk, Run.\\ 
\end{tabular}
}
\caption{Twenty categories of activities are used in the experiments. Each category has 100 examples on average.}
\label{tab:act-list}
\vspace{-1.55em}

\end{table}

% We collect data for $10$ different classes of activities from our volunteers. The duration of each activity is 5--8 seconds. We augment the samples that are less than 8 seconds duration with trailing zeros to make each gesture 8 seconds long. While testing our algorithms, we divide the dataset so that all classes have the same number of testing samples to avoid any bias towards a particular class during the testing phase.

% \begin{table}[!htb]
% \resizebox{.48\textwidth}{!}{
% \begin{tabular}{r|llllllllll}
% \textbf{Activity} & Push & Pull & Circle & Arc & Walk & Run & Eat & Drink & Sit & Stand \\ \hline
% \textbf{Count}  & 250  & 250  & 225 & 225 & 225  & 225 & 225 & 225   & 225 & 225   \\ 
% \end{tabular}
% }
% \caption{List of Activities and Samples}
% \label{tab:dataset}
% \end{table}
 
% Table~\ref{tab:dataset} shows the activity names and the number of sampler per activity. Most of them have 225 samples and two have 250 samples.


 

==> Tamzeed_ArXIV%20(Copy)/tex/08_evaluation.tex <==
\section{Experimental Results}
\label{sec:eval}
\subsection{Accuracy of Unseen Class Detection} 

In this experiment, we report the accuracy of \Sys for \emph{unseen} classes. These are the classes for which \Sys did not have any training examples during training phase. As state-of-the-art systems are not capable of recognizing activities without prior training examples, we are unable to compare them with our solution (i.e., any existing algorithm will have an accuracy of random guess at best). Hence, we report \Sys's performance in this section by varying the number of unseen classes and compare it with two variants of our algorithm: (1) projecting State-Aware Representation (SAR) onto only word embedding (W2Vec) space, and (2) projecting State-Aware Representation (SAR) on only activity-attribute space. This comparison shows the performance boost due to joint space projection. Note that \Sys is able to correctly label an unseen activity only if it has learned the representation of classes that are semantically related to it in terms of movement of body parts and word-level embedding. Therefore, while selecting \emph{unseen} classes, we keep at least one class from the \emph{seen} classes which is close to it in word embedding and attribute space. For example, we select \emph{push} as an unseen class and keep \emph{pull} as a seen class which are semantically related. A \emph{push} is similar to a \emph{pull} in motion of the body parts, e.g., both require movement of hand(s) but legs remain unmoved.  Furthermore, the two English words \emph{push} and \emph{pull} are closer in the word embedding space as they appear in similar contexts.

\begin{figure}[!htb]
	\centering
	\includegraphics[width = 0.45\textwidth]{plot/unseen.pdf}
	\caption{\Sys's accuracy for unseen activity classification.}
	\label{fig:zsl}
	\vspace{-1.05em}
\end{figure}


In Figure~\ref{fig:zsl} we report the accuracy of \Sys in recognizing the unseen classes of activities when 2--6 types of activities are from unseen classes. We evaluate with different combinations of \emph{seen} and \emph{unseen} activities and present the mean accuracy and variance in the plot. In Figure~\ref{fig:zsl}, we see that for two unseen classes, we achieve a classification accuracy of around $90\%$. With only word embedding and attribute space projection, the accuracy is $87\%$ and $88\%$, respectively. For three unseen activities, we get an accuracy near $83\%$ with \Sys. With only word embedding projection the accuracy is around $80\%$, but with attribute space projection the accuracy drops to $60\%$. This is due to the similarity of activities in attribute space, which results in very similar attribute vectors. Therefore, projecting only on attribute space makes the classification harder. As the number of unseen classes increase to 4, 5, and 6, the accuracy becomes to $73\%$ , $67\%$ and and $62\%$, respectively. In all the cases, joint space projection boosts the performance in comparison with single space projection. As the number of unseen classes increase, the problem becomes harder since the model has to differentiate between more classes without training data. We report up to six unseen classes in the plot, however, for seven unseen classes, our accuracy is around $53\%$. With random selection, the accuracy for seven unseen class is $14.28\%$, so \Sys is still better by almost $40\%$.

\subsection{Accuracy of Seen Class Detection} 
\label{sec:eval_seen}

In this experiment, we evaluate \Sys's \emph{seen} class detection performance by keeping \rnote{all} the classes in seen category. We compare \Sys with other baseline classification algorithms. Recent works~\cite{yue2018extracting,jiang2018towards} have demonstrated the efficiency of using Convolutional Neural Network(CNN)-based classifiers for WiFI based activity recognition. Following these works, we compare \Sys with a CNN classifier optimized for our dataset with five convolutional layers along with batch normalization and dropout layers. As mentioned earlier, state-aware representation (SAR) by itself can be used as a feature for supervised classification. Therefore, we also report the performance of state-aware representation (SAR) integrated with a softmax layer. In addition, we also show the performance of projecting state-aware representation only to word embedding space and attribute space. We use five-fold cross-validation by randomly selecting training and testing examples each time. We also report the classification performance of a shallow classifier with a traditional handcrafted feature (i.e., STFT). We report the mean and variance of classification accuracy.
\begin{figure}[!htb]
	\centering
	\includegraphics[width = 0.45\textwidth]{plot/seen.pdf}
	\caption{\Sys's accuracy is higher than baseline algorithms in seen class detection.}
	\label{fig:osl}
	\vspace{-.60em}
\end{figure}

In Figure~\ref{fig:osl}, we find that \Sys achieves a mean accuracy of $82\%$. On the other hand, state-aware representation (SAR) along with softmax layer is able to achieve  around $80\%$ mean accuracy. The performance boost of \Sys is due to the fact that from joint space projection, our model is able to classify activities by integrating knowledge from both word embedding and attribute domain. Projecting state-aware representation onto only word embedding and attribute space yields accuracy of $78\%$ and $76\%$, respectively. With CNN, we have an accuracy of $74\%$. Therefore, the proposed state-aware Representation improves the accuracy for seen class detection by $8\%$ than CNN model. This improvement is achieved since the state-aware representation learns the temporal relationship among the states in an activity. With an SVM, we see the accuracy is around $62\%$. Therefore, it is evident that \Sys is able to achieve better accuracy than other classifiers in seen class detection. Note that \Sys's architecture is modular and generic. We can also integrate other representation to \Sys if necessary.

\subsection{Accuracy of Seen vs Unseen Class Detection} 

In this section, we present the accuracy of our threshold based Seen vs. Unseen detection's performance. The accuracy is threshold dependent. In Figure~\ref{fig:threshold}, we plot the accuracy for $\Omega \in [4.0-5.25]$. We observe that setting a high threshold fails to detect many class as \emph{unseen} and the accuracy drops for the \emph{unseen} classes. With high threshold, the unseen class samples have to be very far apart from any cluster center of the seen class clusters. On the other hand, setting the threshold too small leads to poor results for \emph{seen} classes as it determines majority CSI stream sample as \emph{unseen}. Hence, there is a trade-off between the \emph{seen} and \emph{unseen} class detection accuracy. The optimum threshold is $4.75$, for which, the classification accuracy of the \emph{seen} and \emph{unseen} classes are around $80\%$.
\begin{figure}[!htb]
	\centering
	\includegraphics[width = 0.45\textwidth]{plot/threshold.pdf}
	\caption{The accuracy of \emph{seen} and \emph{unseen} class detection depends on the threshold  $\Omega$'s value. }
	\label{fig:threshold}
	\vspace{-1.95em}
\end{figure}


\subsection{End to End Evaluation}

 \begin{figure*}[!thb]
    % \label{fig:loss_effect}
    \centering
    \subfloat[]{{\includegraphics[width=.33\textwidth]{plot/unseen2.pdf}}}%
    \subfloat[]{{\includegraphics[width=.32\textwidth]{plot/unseen5.pdf} }}%
    \subfloat[]{{\includegraphics[width=.33\textwidth]{plot/unseen8.pdf} }}%
    \caption{ \Sys performs better than baseline algorithms for all cases. a)When 8 out of 10 classes are in seen category, \Sys has almost $80\%$ accuracy for all cases. On the other hand, baseline algorithms' accuracy drops below $20\%$ for cases when unseen category dominate in test samples. b) For 5 out of 10 classes in seen category \Sys outperforms all baseline algorithms for different cases. c)  When 2 out of 10 classes are in seen class, for $.25$ fraction of test samples coming from seen category \Sys's performance drops below $40\%$ which is still 1.5 times better than baselines' performance.  }
    %\vspace{-0.15in}
    \label{fig:whole}%
    \vspace{-.5em}
\end{figure*}

To quantify \Sys's end-to-end performance, we report its classification accuracy for an application scenario. We monitor a user's home activity for ten different classes: \mytt{\{push, pull, run, sit, rub, walk, stand, eat, scratch, drink\}}. We consider three different training scenarios. First, we consider that the user provides 8 out of 10 activity classes' examples to \Sys during training, i.e., the number of classes in seen and unseen categories are 8 and 2, respectively. Second, we consider the case where 5 out of 10 activity  classes' examples are given to \Sys during training. The last and the hardest test case is a scenario where \Sys has only 2 activity classes' samples during training, i.e., 8 out 10 classes are unseen. 

In Figure~\ref{fig:whole}, we report the performance of \Sys along with two baseline algorithms: a convolutional neural network (CNN) and a random forest classifier for all three aforementioned scenarios. For each scenario, we consider three cases where we vary the ratio  between  samples from seen and unseen classes in the test dataset in the following ways: a) $\frac{\#seen}{\#unseen}=25\%$, b) $\frac{\#seen}{\#unseen}=50\%$ and c) $\frac{\#seen}{\#unseen}=75\%$. Here, $\#$ denotes number of samples.



In Scenario 1 (Figure~\ref{fig:whole}(a)), where only 2 classes are in the unseen category, \Sys shows an accuracy around $80\%$ for all the cases, whereas the baseline algorithms' accuracy drops below $20\%$ when most of the samples are coming from the unseen category. Note that the unseen classes are chosen by keeping one of their closest neighbours in the word embedding and attribute space in the seen category. 

In scenario 2 (Figure~\ref{fig:whole}(b)), \Sys achieves an accuracy of $84\%$ for case 3 with majority of the samples in test cases coming from the seen classes. However, when the ratio of seen classes in the test data gets decreased in case 1, the accuracy drops to $73\%$. Yet, \Sys's performance is better than both baselines by a margin of greater than $40\%$. 

In scenario 3 (Figure~\ref{fig:whole}(c)),  where only two classes are in the seen category, the accuracy for the case where $75\%$ of test samples are from seen classes reaches up to $72\%$ for \Sys. However, for case 1, the accuracy drops to $36\%$ where $75\%$ of the test samples are from the unseen categories. This drop is due to the fact that most of the classes are now in unseen category and \Sys has very few classes to learn the mapping function from RF to text domain. For this case, baselines achieve a maximum accuracy of only $24\%$. Therefore, it is evident that \Sys's performance is better than traditional classification algorithms in all the cases.

\subsection{Execution Time} Although only a few WiFi chipsets support CSI information extraction, we believe that in the future, with new tools and chipsets, \Sys will be runnable completely on a variety of platforms including smartphones. In this experiment, we report the execution time of the proposed algorithms for a computer (Macbook Pro). Data are read from the file system of the device. In Table~\ref{tab:exec}, we list the execution times for inference of the two models. We see that the state-aware representation (SAR), which has  convolutional and recurrent layers, takes 12ms on average for inference on a Macbook. On the other hand, the execution time for cross-modal projection, which has two fully connected layers, is around 2ms on a Macbook.

\begin{table}[!htb]
\centering
\resizebox{.25\textwidth}{!}{
    \begin{tabular}{r|l}
        \textbf{Network} & \textbf{Macbook Pro} \\
        \hline
        State-Aware Representation & 12ms  \\
        Cross-Modal Projection  & 2ms \\
    \end{tabular}
}


 \caption{Inference time of deep networks.}
 \label{tab:exec}
 	\vspace{-1.5em}
\end{table}


==> Tamzeed_ArXIV%20(Copy)/tex/09_literature.tex <==
\section{Related Work}
\label{sec:literature}


\subsection{Device-free Sensing} 

$\bullet$ \textit{RSSI based}: WiFi based sensing have opened the doorway for device-free activity monitoring in the last couple of years. Researchers have used wifi signal characteristics such as signal strength (RSSI) and channel state information(CSI) for activity recognition~\cite{kwapisz2011activity}. RSSI based activity recognitions have been proposed in~\cite{abdelnasser2015wigest, sigg2014rf, sigg2014telepathic, kosba2012rasid, sigg2013rf}. However, RSSI based gesture recognition system have limitations in detecting fine-grained gestures. Moreover, all of these works require training examples to detect a particular activity class.~\cite{abdelnasser2015wigest,sigg2014telepathic} uses pattern matching algorithm to find the best match between the target gesture with pre-defined gestures. Our target in this paper, is classifying activities and gestures without training examples and our framework can be ported to RSSI based systems. 

$\bullet$ \textit{Special Device based}: There have been several works in gesture and activity recognition using specialized devices and radars.~\cite{malysa2016hidden, yue2018extracting, zhao2016emotion} use FMCW~\cite{ramasubramanian2017using, adib2015smart} radio to monitor user activity.~\cite{yue2018extracting} trains a CNN classfier to detect human motion.~\cite{malysa2016hidden} trains a hidden markov model using time-velocity feature for activity recognition. \cite{pu2013whole} uses a 5-antenna receiver and a single-antenna transmitter to perform gesture classification, in the presence of three other users performing random gestures. 
They use doppler shifts to match with pre-defined gestures for an incoming test data. It is evident that none of these specialized device based sensing system deals with ctivity recognition without prior examples. They all require labelled training examples for activity recognition. 

$\bullet$ \textit{CSI based}: With the availability of CSI from network interface cards, multiple works~\cite{wang2017wifall, wang2016we, xi2014electronic, li2016wifinger} have emerged which exploit CSI information for gesture and activity recognition. \cite{wang2014eyes} proposes a signal profile matching technique to detect loosely defined daily activities that involve a series of body movements over a certain period of time.~\cite{wang2015understanding} proposes correlation  between CSI amplitude value and gesture speed to build model for gesture recognition.  ~\cite{wang2016gait} uses variations in the Channel State Information (CSI) to classify gaits of humans. ~\cite{virmani2017position} uses translation based data augmentation technique to make gesture classification models robust to user orientation.~\cite{venkatnarayan2018multi} proposed multi-person gesture recognition system by generating virtual gesture samples and combining them to create an exhaustive template matching algorithm. Recent works such as ~\cite{chen2018wifi, wang2018spatial, ma2016survey} use deep learning based techniques such  Convolutional Neural Networks to recognize activities from CSI.~\cite{zou2018deepsense, chen2018wifi} proposes recurrent neural network based activity classifier , however ours is the first work to model the micro-activity or state transition which constitute an activity.~\cite{zou2018deepsense}  predicts label for each segment of the CSI stream. On the other hand, we need only one label for the whole CSI stream which makes our model to learn the entire sequence of states to make a decision about the activity. Besides, we learn the local and transitional feature in an end to end manner with bi-directional recurrent neural network, which makes our model stronger. Ours  SAR is the first model to incorporate local feature of states and their transition in a bi-directional fashion. ~\cite{jiang2018towards} proposed an adversarial network to learn environment independent signal characteristics from gestures. In this work, the authors used unlabelled data to improve their model's performance. But their proposed system is not able to infer an activity without having any training example. Very recent work~\cite{zero_effort} proposed velocity profiles as environment independent feature to solve the problem of environmental effect on CSI. All of these works rely on provided training examples to classify a particular class of activity. \Sys deals with classification of activity from WiFi CSI data without any training examples. This is significantly different from current state of the arts.

\subsection{Zero Shot Learning}
In image domain, learning from limited or no data has been explored recently.~\cite{koch2015siamese, vinyals2016matching, duan2017one} focus on learning suitable image representation to classify images from very few or only one examples. These works are totally different from ours as we want to recognize activities from WiFi without any training data.
The other branch of learning with limited data focuses on zero shot learning for image classification.
The  earlier practices of zero shot learning~\cite{lampert2014attribute,norouzi2013zero, kodirov2015unsupervised} for image classification problem infer the labels of unseen classes using a two step algorithm. First, the attributes of the sample is inferred and then the class label is predicted from an attribute database, which has most similar attributes with the image. Recent works~\cite{xian2016latent, socher2013zero, akata2016label} have explored the mapping between image features and semantic space by projecting image features into word embedding space. Similar line of works~\cite{palatucci2009zero,frome2013devise, zhang2015zero,kodirov2017semantic} project image feature into semantic space then searches the nearest class label embedding using ranking loss. Although these papers propose zero shot learning method for images, none of them addresses the problem for RF domain and activity recognition. ~\cite{zellers2017zero, xu2017transductive,liu2017generalized, madapana2017semantical} do activity recognition using zero shot learning for RGBD data.~\cite{islam2019soundsemantics} proposes zero shot learning for audio event recognition. But, the sequential nature of activity and need for external attribute knowledge makes our problem more challenging. ~\cite{cheng2013towards} proposes zero shot learning for body-worn IMU based activity recognition. However, our work is the first paper to propose a zero shot learning method for WiFi based activity classification where we overcome the challenges for cross-modal learning between text and RF domain.  These works on zero shot activity detection use an attribute database of the gestures to recognize unseen types. Our contextual word-embedding based approach does not require the attributes of the unknown gestures or activities beforehand. To the best of our knowledge, we present the first system with capabilities of inferring activities from RF signal without training examples. We propose the first work to integrate textual domain with RF. We also present novel feature representation for RF based activity monitoring. 



==> Tamzeed_ArXIV%20(Copy)/tex/10_discussion.tex <==
\section{Discussion}
\label{sec:disc}

$\bullet$ \textit{Synergey Between Seen and Unseen Class}
 For an unseen activity, \Sys is able to detect it with high accuracy if there is a seen class with similar class label property, i.e., similar word embedding and attribute vectors. \Sys assumes that activity classes with similar properties have semantically similar class labels. We use this assumption to learn the non-linear mapping function to project WiFi signals onto the word embedding and attribute spaces. Without semantically similar training examples corresponding to an unseen class, a zero-shot learner fails to recognize examples from that unseen class. However, in a large dataset, the chances that there is no semantically similar training example to an unseen class is relatively low.  To demonstrate this, we conduct an experiment. We keep \mytt{pull} as an unseen class and exclusively put the following classes in the seen category in a round-robin fashion: \mytt{\{push, throw, point, kick\}}. In Figure~\ref{fig:disc}, on the X-axis, we put these classes with their corresponding distances in the joint word embedding and attribute space with \mytt{pull}. We see that, as the distance increases from the unseen category, the accuracy of unseen class recognition drops. When \mytt{push} is in seen category, the classification accuracy for \mytt{pull} is more than $90\%$. As \mytt{push} and \mytt{pull} are close in word embedding and attribute spaces, the presence of \mytt{push} in training data helps recognize the samples from \mytt{pull}. As we go further away from \mytt{pull} in the word embedding and attribute space, the accuracy drops even more. For \mytt{kick}, which is the farthest from \mytt{pull}, we see that the classification accuracy for \emph{pull} is around $60\%$.
\begin{figure}[!htb]
	\centering
	\includegraphics[width = 0.45\textwidth]{plot/discussion.pdf}
% 	\vspace{-.5em}

	\caption{\Sys's performance in unseen activity recognition is dependent on its relationship with classes in seen category.}
	\label{fig:disc}
	\vspace{-1.0em}
\end{figure}

$\bullet$ \textit{Necessity of User-Provided Tag-List.} The user-provided additional labels do not have any influence on the training phase. They are only used in the classification step after the training has been completed. If we do not have these additional labels, then the search space becomes too large (i.e., as big as having all the words in our database for a language) in the classification stage. Therefore, the user provided labels for unseen class is important in getting better accuracy for unseen activities.

$\bullet$ \textit{Environmental Effect.} Our main objective in this paper is to propose the first cross-modal RF to text projection to enable zero-shot activity classification. The proposed representation learning algorithm does not consider environment  or multi-person effect. Recent works~\cite{jiang2018towards,venkatnarayan2018multi} have showed promising results on solving these issues. Both State-Aware Representation and Cross modal projections are modular and generic. We can port these solutions to \Sys to handle these artifacts.




==> Tamzeed_ArXIV%20(Copy)/tex/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion} 
In this paper, we present the first WiFi-based device-free activity recognition system that does not require training examples for all activities. We propose a robust state-aware representation of RF signature associated with activities to preserve their contextual information. We propose a novel way to embed contextual information from the text domain to the RF domain by projecting RF data onto the word embedding and attribute space. We use this cross-modal RF embedding and propose a general classifier to recognize both \emph{seen} and \emph{unseen} activities. We collect WiFi data for 20 different activities from four volunteers and show that \Sys is capable of inferring activities from WiFi without training examples with $62\%-90\%$ accuracy for 2--6 unseen classes. 
\newpage
